ezCoref: Towards Unifying Annotation Guidelines for Coreference Resolution

Large-scale, high-quality corpora are critical for advancing research in coreference resolution. However, existing datasets vary in their definition of coreferences and have been collected via complex and lengthy guidelines that are curated for linguistic experts. These concerns have sparked a growing interest among researchers to curate a unified set of guidelines suitable for annotators with various backgrounds. In this work, we develop a crowdsourcing-friendly coreference annotation methodology, ezCoref, consisting of an annotation tool and an interactive tutorial. We use ezCoref to re-annotate 240 passages from seven existing English coreference datasets (spanning fiction, news, and multiple other domains) while teaching annotators only cases that are treated similarly across these datasets. Surprisingly, we find that reasonable quality annotations were already achievable (>90% agreement between the crowd and expert annotations) even without extensive training. On carefully analyzing the remaining disagreements, we identify the presence of linguistic cases that our annotators unanimously agree upon but lack unified treatments (e.g., generic pronouns, appositives) in existing datasets. We propose the research community should revisit these phenomena when curating future unified annotation guidelines.

==> EMNLP 2022/emnlp_sections/abstract_v1.tex <==
\begin{abstract}
%\agcomment{WIP} 
Large-scale high-quality corpora are critical for advancing research in coreference resolution. However, existing datasets vary widely in their definition of coreference (expressed through annotation guidelines), making it unclear which guidelines to employ when collecting a corpus in a new language or domain. Furthermore, because these guidelines contain lengthy explanations of complex linguistic phenomena, they are best suited for expert annotators (e.g., linguists) rather than untrained crowd workers. In this work, we investigate whether it is feasible to crowdsource coreference annotations by providing \emph{minimal} guidelines to non-expert annotators, thereby reducing time and effort on the part of both annotators and researchers. We develop a crowdsourced coreference annotation platform called \ezcoref\ and use it to re-annotate 240 passages from seven existing English coreference datasets. 
We find annotators agree (>90$\%$ B3) with expert annotations (e.g., those in OntoNotes) even without extensive training, signifying that high-quality data can be obtained via crowdsourcing with minimalistic guidelines. Additionally, we observe deviations between crowd annotators and existing guidelines on linguistic phenomena such as general pronouns, appositives, and copulae, which can help inform guideline creation for future coreference annotation efforts.

% \mkcomment{I think the focus is off in the abstract -- basically seems like we braging that we got good annots with no guidelines, so 'easy things are easy' -- my least fav review, ugh!}

% [Shortened version of the above] Large-scale high-quality corpora are critical for advancing research in coreference resolution. However, existing datasets vary widely in their definitions of coreference, expressed through annotation guidelines. Furthermore, these guidelines contain lengthy explanations of complex linguistic phenomena and are most suited for expert annotators (e.g. linguists). In this work, we propose to crowdsource coreference annotations by providing \emph{minimal} guidelines to non-expert annotators, therefore reducing time and effort on the part of both annotators and researchers. We develop a crowdsourced coreference annotation platform called \ezcoref\ and use it to annotate 240 passages from seven existing English coreference datasets. We find that without extensive training, crowd workers provide annotations that mostly agree with expert annotations (e.g., those in OntoNotes). This signifies that high-quality data can be obtained via crowdsourcing with minimal guidelines. Additionally, we analyze deviations between crowd annotators on linguistic phenomena such as cataphora, appositives, and copulae, to inform guideline creation for future coreference annotation in new languages and domains.

% In particular, we observe a high agreement among annotators in the fiction domain and that annotating cataphora is challenging for crowd annotators. We also find that appositives and copulae have been treated similarly by existing guidelines, but non-expert annotators naturally mark them differently and would require clarification in guidelines if expected otherwise. 

% This paper is the first to compare the quality of crowdsourced coreference annotations against those of experts, and to identify where their behavior differs to facilitate future annotation efforts.

% To address these challenges,
% we develop and release \ezcoref, an easy-to-use coreference annotation tool and annotation methodology
% that facilitates crowdsourced data collection across multiple domains, currently in English.

% Instead of teaching crowdworkers how to handle non-trivial cases (e.g., near-identity coreferences), \ezcoref\ provides only a minimal set of guidelines sufficient for understanding the basics of the task. To validate this decision, we deploy \ezcoref on Mechanical Turk to re-annotate 240 passages from seven existing English coreference datasets across seven domains, achieving an average rate of 2530 tokens per hour, for one annotator. 

\ignore{Large-scale high-quality corpora are critical for advancing research in coreference resolution. 
Coreference annotation is typically time-consuming and expensive, since
researchers generally hire expert annotators %(e.g., trained linguists) 
and train them
with an extensive set of guidelines.
% This process is expensive and time-consuming, which motivates cheaper and quicker 
Crowdsourcing is a promising alternative,
but coreference includes complex semantic phenomena 
difficult to explain to untrained crowdworkers,
and the clustering structure is difficult to manipulate in a user interface. \agcomment{mentioning clustering structure here is too detailed}
% With the advent of deep learning, a large annotated corpus is crucial for advancing the development of coreference systems. %However, coreference annotations have traditionally been arduous and time-consuming, with a small number of trained linguists providing extensive annotations. 
% One way to quickly collect a large-scale coreference corpus is to use crowdsourcing (CITE) but this approach requires an intuitive annotation tool and simplified guidelines. 
% In this paper, we propose a new, more human-friendly paradigm to collect crowdsourced coreference annotations. 
To address these challenges,
we develop and release \ezcoref, an easy-to-use coreference annotation tool and annotation methodology
that facilitates crowdsourced data collection across multiple domains, currently in English.
% \ezcoref\ can facilitate the annotation process across multiple domains and languages\kkcomment{did we do expts on other languages? Not sure if we should say this if no expts} \mkcomment{no, we didn't but I think it's a strong aspect of the tool and can't see how it would break at least for languages that use the same alphabet, or am i missing sth?\micomment{since we didn't do an exps, we shouldnt mention this in the abstract. maybe in future work} }, 
%% BTO: auto detection assumes English, so our current software could NOT be applied to nonEnglish.
%and received positive feedback from the crowd workers. \mkcomment{well, actually that was about the tutorial, but it's probably ok} \agcomment{we collected feedback for  main task as well, though not many annotators responded. The small number of feedback was positive/neutral.}
% \mkcomment{yeah, I hope we will be able to get more from the survey}
Instead of teaching crowdworkers how to handle non-trivial cases (e.g., near-identity coreferences), \ezcoref\ provides only a minimal set of guidelines sufficient for understanding the basics of the task. To validate this decision, we deploy \ezcoref on Mechanical Turk to re-annotate 240 passages from seven existing English coreference datasets across seven domains, achieving an average rate of 2530 tokens per hour, for one annotator. \agcomment{why is this rate important to mention here?}
%
\agcomment{the following line is the main crux of the paper}\textbf{This paper is the first to compare the quality of crowdsourced coreference annotations against those of experts, and to identify where their behavior differs to facilitate future annotation efforts.}
We show that it is possible to collect coreference annotations of a reasonable quality in a fraction of time it would traditionally require.
%We provide the crowd workers with minimal annotation guidelines and identify what they intuitively mark as coreference. We utilize this data and provide suggestions for future annotation efforts.  


%Further, we study the differences in annotations for each dataset and compare them against crowdsourced annotations. This paper is the first to gather and categorize these inconsistencies and provide suggestions for future annotation efforts and evaluation decisions. Despite increased attention on crowdsourcing annotations for coreference resolution, there are still many open problems, which we highlight in this paper.


%ORIGINAL:
% With the advent of deep learning, large annotated corpora are crucial for advancing the development of models for coreference resolution. The need to collect large-scale corpora with reduced costs \mkcomment{time?} and efforts has motivated interest in developing annotation platforms to collect crowdsourced annotations for this task. However, there is still a need for an easy-to-use and intuitive platform which can facilitate the annotation process across multiple domains and languages. In this paper, we present an easy-to-use and intuitive annotation platform to collect coreference annotations. Using this platform, we collect crowdsourced annotations for seven existing datasets, covering a range of genres and annotation procedures. We examine the challenges while collecting annotations using crowdsourcing.
% Further, we study the differences in annotations for each dataset and compare them against crowdsourced annotations. This paper is the first to gather and categorize these inconsistencies and provide suggestions for future annotation efforts and evaluation decisions. Despite increased attention on crowdsourcing annotations for coreference resolution, there are still many open problems, which we highlight in this paper.
}


\end{abstract}

==> EMNLP 2022/emnlp_sections/abstract_v2.tex <==
\begin{abstract}
% Large scale high quality corpora are critical for advancing research in coreference resolution. However, existing datasets vary in their definition of coreferences (expressed via annotation guidelines), making it unclear which guidelines should be employed when collecting annotations in a new domain or language. Furthermore, these guidelines are often curated with experts (e.g. linguists) in mind, containing lengthy explanations of complex linguistic phenomena, and thus are not suitable for untrained crowd annotators. Owing to these concerns, there has been a growing interest in curating a unified set of guidelines which can also be utilized in crowdsourcing setups, thereby reducing effort on part of both annotator and researcher. In this paper, we investigate crowdsourcing coreference with the use of minimal guidelines, consisting of cases that are similarly treated across all existing datasets, thus serving as the starting point towards guidelines unification. To collect the crowd annotations under these guidelines, we develop a crowdsource-friendly coreference annotation platform called ezCoref and use it to re-annotate 240 passages from seven existing English coreference datasets, spanning multiple domains. On comparing our crowdsourced annotations with the expert annotations, we obtain high agreement (>90$\%$ B3), signifying that reasonable annotations are achievable via crowdsourcing with minimalistic guidelines. We further identify that fiction domain is most suitable for crowdsourcing coreference owing to high inter-annotator agreement in this domain. Finally, we identify linguistic cases where annotators unanimously agree, yet these cases either lack unified treatment across existing datasets (e.g., appositives) or have been resolved differently (e.g., generic pronouns), thus highlighting complex coreference cases which should be revisited by the research community while curating a future annotation guidelines.

% Large-scale, high-quality corpora are critical for advancing research in coreference resolution. However, existing datasets vary in their definition of coreferences (expressed via annotation guidelines), making it unclear which guidelines to employ when collecting annotations in a new domain or language. Furthermore, these guidelines contain lengthy explanations of complex linguistic phenomena, as they are often curated with experts (e.g., linguists) in mind. These concerns have sparked a growing interest among researchers in curating a unified set of guidelines suitable for annotators with various backgrounds. In this work, we develop a crowdsource-friendly coreference annotation methodology, \ezcoref, consisting of an annotation tool and an interactive tutorial. We use \ezcoref\ to re-annotate 240 passages from seven existing English coreference datasets (spanning multiple domains) while teaching annotators only those few cases that are treated similarly across these datasets. Surprisingly, we find that reasonable quality annotations were already achievable (>90$\%$) agreement between the crowd and expert annotations) even without extensive training. On carefully analyzing the remaining disagreements, we identify the presence of linguistic cases that our annotators unanimously agree upon but lack unified treatments (e.g., appositives, generic pronouns) in the existing datasets, thus suggesting coreference cases to be revisited by the research community while curating unified annotation guidelines. Finally, upon analyzing the inter-annotator agreement among crowd annotators, we find fiction domain to be particularly suitable for crowdsourcing coreferences.
 
Large-scale, high-quality corpora are critical for advancing research in coreference resolution. 
However, existing datasets vary in their definition of coreferences and have been collected via complex and lengthy guidelines that are curated for linguistic experts.
% However,
% existing datasets vary in their definition of coreferences,
% % (expressed via annotation guidelines), 
% making it unclear which guidelines to employ when collecting annotations in a new domain or language. Furthermore, these guidelines contain lengthy explanations of complex linguistic phenomena, as they are often curated for linguistic experts. 
These concerns have sparked a growing interest among researchers to curate a unified set of guidelines suitable for annotators with various backgrounds. In this work, we develop a crowdsourcing-friendly coreference annotation methodology, \ezcoref, consisting of an annotation tool and an interactive tutorial. We use \ezcoref\ to re-annotate 240 passages from seven existing English coreference datasets (spanning fiction, news, and multiple other domains) while teaching annotators only cases that are treated similarly across these datasets.\footnote{All resources accompanying this project will be added to our project page: \url{https://github.com/gnkitaa/ezCoref}} Surprisingly, we find that reasonable quality annotations were already achievable (>90$\%$ agreement between the crowd and expert annotations) even without extensive training. On carefully analyzing the remaining disagreements, we identify the presence of linguistic cases that our annotators unanimously agree upon but lack unified treatments (e.g., generic pronouns, appositives) in existing datasets. 
% \mkcomment{for me this doesn't connet in the middle well without "which" -- that is: "...agree upon but WHICH lack..." it's not incorrect now, it's just hard to read}
We propose the research community should revisit these phenomena when curating future unified annotation guidelines.

% \mkcomment{make stronger? maybe even simply: "The research community should revisit/reevaluate..." or "Our findings suggest that these phenomena have to be ...."}
\end{abstract}

% PLAINTEXT for arXiv
% Large-scale, high-quality corpora are critical for advancing research in coreference resolution. However, existing datasets vary in their definition of coreferences and have been collected via complex and lengthy guidelines that are curated for linguistic experts. These concerns have sparked a growing interest among researchers to curate a unified set of guidelines suitable for annotators with various backgrounds. In this work, we develop a crowdsourcing-friendly coreference annotation methodology, ezCoref, consisting of an annotation tool and an interactive tutorial. We use ezCoref to re-annotate 240 passages from seven existing English coreference datasets (spanning fiction, news, and multiple other domains) while teaching annotators only cases that are treated similarly across these datasets. Surprisingly, we find that reasonable quality annotations were already achievable (>90% agreement between the crowd and expert annotations) even without extensive training. On carefully analyzing the remaining disagreements, we identify the presence of linguistic cases that our annotators unanimously agree upon but lack unified treatments (e.g., generic pronouns, appositives) in existing datasets. We propose the research community should revisit these phenomena when curating future unified annotation guidelines.

==> EMNLP 2022/emnlp_sections/acknowledgments.tex <==
\section*{Acknowledgements}

% BTO notes, funding
% - NSF CCRI
% - NSF SubjKB


% We are very grateful to the freelancers on Upwork
% and volunteers who helped us evaluate generated
% text. We thank Xavier Garcia and the T5X team for
% helping us with technical issues related to the T5X
% library. 
We are very grateful to the crowd annotators on AMT
for participating in our annotation tasks and providing positive reviews. We are grateful to Kavya Jeganathan, Abe Handler, Neha Kennard, Timothy O'Gorman, Nishant Yadav, Anna Rogers, and the UMass NLP group for several useful discussions during the course of the project. We also thank Massimo Poesio for sharing the GNOME portion of ARRAU dataset. 
This material is based upon work supported by National Science Foundation awards 1925548, 1814955, and 1845576, and a Google PhD Fellowship awarded to KK. %awarded in 2021.



==> EMNLP 2022/emnlp_sections/analysis.tex <==
\section{Analysis}
\label{sec:data_analysis}
In this section, we perform quantitative and qualitative analyses of our crowdsourced coreference annotations. First, we evaluate the performance of our mention detection algorithm, comparing it to gold mentions across seven datasets. Next, we measure the quality of our annotations (via inter-annotator agreement between our crowdworkers) and their agreement with other datasets. Finally, we discuss interesting qualitative results.  
\subsection{Mention Detector Evaluation}
% As a first step to collect crowdsourced annotations, we must identify mentions in documents from each dataset. Existing datasets use very different methods to identify such mentions, ranging from manual, semi-automatic, to fully automatic procedures. Furthermore, they also use very different criteria to identify these mentions. As a result, mentions provided with these datasets cannot be directly used to compare the inter annotator agreement of crowd annotations across different domains.
% Thus, we use a simple and automated method to identify mentions with high recall with these datasets. 
% \mkcomment{I think this should be in the mention detection section. Here we can start with one intro sentece and move to the analysis}

% \btocomment{this needs to talk about head words---briefly define and motivate the procedure. it underlies all comparisons between our workers and gold std.}
% \agcomment{
% Due to different approaches followed by datasets for mention identification, mentions identified by our algorithm, and the mentions provided with existing datasets can have different boundaries for the same mention. Thus, we use a head-word-based comparison between two mentions to fairly compare our annotations with gold annotations. In particular, we find the headword of a mention span by identifying the most-shared ancestor (in the dependency tree) of all tokens within the mention span. We consider two mention spans as the same if their respective headwords match.}
Datasets differ in the way they define their mention boundaries. Hence, the boundaries for the same mention may differ. To fairly compare our mentions with the gold standards, we employ a headword-based comparison. We find the head of the given phrase by identifying, in the dependency tree, the most-shared ancestor of all tokens within the given mention. Two mentions are considered same if their respective headwords match.

\autoref{table:mention_detection_algo} compares our mention detector to the gold mentions in existing datasets. Our method obtains high recall across most datasets ($>$\num{0.90}), which shows that most of the mentions annotated in existing datasets are correctly identified and allows a direct comparison of crowd annotations with expert annotations.
% suggesting that our mention detection algorithm identifies most of the mentions provided in respective datasets. This setup allows us to collect crowdsourced coreference annotations on these mentions and compare them with the expert annotations supplied in their respective datasets
It has the lowest recall with ARRAU  (\num{0.84}) and PreCo (\num{0.88}), which is to be expected as ARRAU marks all referring premodifiers (identified manually) and PreCo allows common noun modifiers, while we identify only the premodifiers which are proper nouns.\footnote{We made this decision as identifying automatically all premodifiers would result in many singletons and lead to more arduous annotation effort.}
% ARRAU has the lowest recall (\num{0.84}) as they manually identify all premodifiers as mentions (when they are referring) in addition to noun phrases. \mkcomment{I think there are two aspects: 1) they mannually identify mentions in general is should be better than auto in terms of quality (like NP vs VP can be leading to some algo mistakes - and I saw some in qual, even the river "Fog up the river" - "fog" is not being detected as it's probably identified as vp; and 2) they identify all premods as mentions, this includes common nouns which we exclude (this is regardless of whether that's done auto or manual). Maybe sth like "We observe that our algorithm has the lowest recall with ARRAU (\num{0.84}). This is to be expected as ARRAU marks all referring premodifiers, while we identify only the premodifiers which are proper nouns. We made this decision as identifying automatically all premodifiers would result in many singletons and lead to a greater annotation efforts." (added things from sentences below, the important thing is that in auto way we cannot just identify the refering ones and identifying all would be a mess.) }
% However, marking all possible premodifiers algorithmically can significantly increase the number of mentions (mostly singletons) thereby increasing annotation time and effort. Thus, our mention detection algorithm includes only those premodifiers which are proper nouns. Similarly, PreCo also allows more premodifiers (common nouns), as mentions, resulting in a slight drop in the recall, although it has a better recall than ARRAU. 
% \mkcomment{Similarly, PreCo allows common noun premodifiers which is likely one of the reasons for the slightly lower recall.}
For most datasets, the precision is $>$\num{0.80}, suggesting that the algorithm identifies most of the relevant mentions. 
We observe a substantially lower score for OntoNotes, LitBank, and QuizBowl as these datasets restrict their mention types to limited entities (refer to \autoref{table:motivation}). However, low precision on these datasets is expected and does not affect our analysis since an algorithm with high precision on LitBank or OntoNotes would miss a huge percentage of relevant mentions and entities on other datasets (constraining our analysis) and when annotating new texts and domains. 
Moreover, our algorithm identifies more mentions than in the original datasets, which also allows us to discover new entities. 
% Comparing precision, we observe a substantially lower score for OntoNotes, LitBank, and QuizBowl as these datasets restrict their mention types to limited entities (refer to \autoref{table:motivation}). As a result, our algorithm identifies more mentions than in the original datasets, which also allows us to discover new entities. For the remaining datasets, the precision is $>$\num{0.80}, suggesting that the algorithm identifies most of the relevant mentions.
% \agcomment{also say why this high Precision/Recall of mention detection algorithm is important? What does it mean to have good performance? How does it help us in overall objective of this paper?}
% \kkcomment{Arguing about precision seems tricky --- on one hand low precision is good because you will have more coverage / new entities. On the other hand (like you previously mentioned, too many mentions will significantly increase annotator effort. Seems like there's a sweet spot here for precision} 
Finally, the mention density (number of mentions per token) from our detector 
% between our detector and existing datasets, and find that while gold mention density varies considerably across the seven datasets due to their differing mention criteria (\autoref{table:motivation}),  it 
remains roughly consistent across all datasets when using our method, allowing us to fairly compare statistics (e.g., agreement rates) across datasets.

\begin{table}[]
\centering \scriptsize
\begin{tabular}{lcccc}
\toprule \addlinespace[0.1cm]
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Dataset}}} &
  \multirow{2}{*}{\textbf{Recall}} &
  \multirow{2}{*}{\textbf{Precision}} &
  \multicolumn{2}{c}{\textbf{Mentions / Tokens}} \\ \addlinespace[0.1cm] \cline{4-5} \addlinespace[0.1cm]
\multicolumn{1}{c}{}       &                      &                      & \textbf{Gold}        & \textbf{This Work}      \\ \hline \addlinespace[0.1cm]
OntoNotes                  & 0.957 & 0.376 & 0.112 & 0.286 \\
LitBank                    & 0.962                & 0.415                & 0.121                & 0.280                \\
QuizBowl                   & 0.956                & 0.543                & 0.188                & 0.318                \\
PD (Gold)   & 0.953                & 0.803                & 0.259                & 0.273                \\
PD (Silver) & 0.938                & 0.791                & 0.265                & 0.274                \\
GUM                        & 0.906                & 0.848                & 0.269                & 0.287                \\
PreCo                      & 0.881                & 0.883                & 0.287                & 0.287                \\
ARRAU                      & 0.840 & 0.870 & 0.289 & 0.279 \\

\bottomrule
\end{tabular}
\vspace{-0.05in}
\caption{Comparison of mentions identified by our mention detection algorithm with the gold mentions annotated in the respective datasets. We use head-word based comparison to compare mentions of different lengths.}
\vspace{-0.1in}
\label{table:mention_detection_algo}
\end{table} 


% \mkcomment{"On the other hand, mention density of our algorithm remains roughly consistent across all datasets." not sure about the other part, I wouldn't say "syntactic and semantic phenomena"}


% Different coreference datasets annotate different kinds of mentions. Furthermore, the procedure to identify these mentions also varies across these datasets. OntoNotes, for example, considers all noun phrases identified via its treebank data as mentions while they excluding singletons (i.e., mentions that do not refer to anything), severely restricting the number of mentions in this dataset. Other mention types such as possessive nouns, proper noun premodifiers, and verb phrases (when coreferent with an NP) are manually identified by annotators. Datasets such as LitBank and QuizBowl allow singletons. However, they limit their mention sets to certain types of entities, ACE-style-entities for LitBank and authors, characters, works for QuizBowl \footnote{QuizBowl allows other types of mention only when this mention is an answer to a question}. Consequently, as shown in Table~\ref{table:mention_detection_algo}, all these datasets have low mention density. 

% The remaining datasets, including PreCo, Phrase Detectives, ARRAU, and GUM, consider a wider variety of mentions, including all noun phrases, singletons, and generic mentions. In addition, Phrase Detectives and ARRAU also mark expletives and split antecedent mentions. Phrase Detectives relies on a semi-automatic procedure using Berkeley Parser~\cite{petrov-klein-2007-improved} to identify mentions followed by manual verification. ARRAU and GUM identify their mentions manually based on a single expert annotation and annotations collected by students as part of a linguistics course, respectively. PreCo also seems to rely on its annotators to identify mentions\agcomment{I can't seem to find in their paper how do they identify mentions}. Overall, these datasets have a higher mention density, comparable to mention density obtained by using our mention detection algorithm, as shown in Table~\ref{table:mention_detection_algo}. 

% However, a simple and automated method is required to identify mentions supporting large-scale crowdsourcing of coreferences. We use our developed mention detection algorithm to identify mentions for documents in all the seven existing datasets. Comparing the extracted mentions with the mentions provided in the respective datasets\footnote{We use head-word based comparison to accommodate comparison of mentions with different lengths.}, we obtain a high recall across all the datasets (> 0.90 for most) suggesting that our mention detection algorithm identifies most of the mentions provided in respective datasets. This setup allows us to collect crowdsourced coreference annotations on these mentions and compare them with the expert annotations supplied in their respective datasets. In ARRAU, all premodifiers are marked as mentions (including adjectival, numerical and adverbial modifiers) in addition to the noun phrase they modify, unlike our mention detection algorithm which merges premodifiers with the noun phrase to construct a compound noun phrase as mention. Furthermore, ARRAU also considers verb phrases as mentions to support event anaphora. These factors explain a drop in recall for ARRAU. Verb phrases are currently not supported by our mention detection algorithm, but can be easily incorporated. Similarly, PreCo considers common noun and proper noun modifiers as mentions, but does not allow adjective modifiers. Thus, PreCo has has a slight drop in recall, although it has better recall compared to ARRAU. 

% In addition to recall, we also analyze precision between algorithmically identified mentions and mentions provided with datasets. The precision is substantially lower for OntoNotes, LitBank, and QuizBowl since these datasets allow only limited types of mentions. Our algorithm identifies many more mentions than originally annotated in these datasets, allowing the discovery of potentially new entities. For the remaining datasets, the precision is > 0.80, suggesting the algorithm identifies most of the relevant mentions. 


% Points to discuss - AG

% ARRAU - A [Taiwaneese] Company - adjectival modifier as mention - $arrau\_wsjarrau\_0606\_0\_0$

% 1. While calculating recall, we use the head word based matching of mentions. Mention density is number of mentions/ number of tokens. e calculate these statistics for entire data including training, validation and testing splits wherever applicable. 


% 2. OntoNotes has only singletons and LitBank has only ACE entities, resulting in low gold mention density for both datasets.Our MD algo identifies lot more mentions compared to gold data, thus precision is low. However, recall is high implying MD algo identifies most of the gold mentions and identifies additional mentions.

% 3. QuizBowl marks singletons, 
% Gold mentions are identified by annotators (user highlights a phrase and then assigns it to a group). Users are asked to annotate all authors, characters, works, and the answer to the question (even if the answer is not one of the previously specified types of entities). Users are asked to
% consider appositives as separate coreferences to
% the same entity. Thus, The Japanese poet Basho
% has two phrases to be marked, The Japanese poet
% and Basho, which both refer to the same group. Split antecedents not marked. 

% 3. PD gold and silver includes non-referring expressions. 

% 4. PD, GUM, PreCo and ARRAU have comparable mention densities. The mention densities are also close to mention densities obtained by using our MD Algo. 

% In ARRAU, for example, singletons and expletives are annotated as well, as are split antecedent plurals, generic coreference, discourse deixis, and bridging references. The ARRAU corpus is relatively small in terms of tokens (350K), but has a higher markable density than ONTONOTES (0.29 markable/token).

% In PreCo, 3000 most common English words appear in the
% documents. Singleton mentions and generic coreference are annotated, event anaphora is not, and
% predicative NPs are annotated as co-referring with
% their argument.

% In PD, split antecedent are marked, expletives, predicative NPs.
% In the
% Phrase Detectives corpus predication and coreference are clearly distinguished, as in ONTONOTES
% and ARRAU but unlike in PRECO.  Singletons
% are considered markables. Expletives and split
% antecedent plurals are marked, unlike in either
% ONTONOTES or PRECO.  Each document would first
% be processed by a pipeline combining off-the-shelf
% tools (sentence splitting and tokenization using the
% OpenNLP pipeline3
% and parsing using the Berkeley Parser (Petrov and Klein, 2007)) and custom
% preprocessing and post-processing heuristic steps
% to correct the output. (See (Poesio et al., 2013)
% for more details about the pipeline and its performance.) Then one of the administrators would
% carry out a quick check of the document removing the most obvious mistakes before uploading
% it. After the document was uploaded, participants
% could report markable errors, which would then be
% corrected by hand


%\agcomment{to myself: consistent sigdigs}
%\agcomment{Reminder to myself: PreCo and ARRAU have lower recall, some mentions in gold are not detected by system. need to check, what kind of mentions are extra in gold? adverbial noun modifiers in PreCo, events in gerund form in PreCo, Event Anaphora in ARRAU, ON. GUM has event mentions, it is unclear whether they mark coreferences for events.}




% \subsection{Variation of Agreement across Domains/
% , an annotator must know that Kitty is a nickname of Ekaterina in the novel, and Levin failed in his courtship of Ekaterina before marrying her to resolve coreferences. This requirement of factual knowledge in a complicated cataphoric structure (thereby a lot more incoherent than fiction) makes the task a lot harder for crowdsourcing setups. Factual knowledge is required sometimes for news domain as well, (e.g., in Table~\ref{table:iaa_examples}, example (d), one must know that Pravda is former official newspaper of the Communist Party of the Soviet Union.)

% We examine the inter-annotator agreement to analyze how crowd annotator behaviour varies across all the domains. We use B3 metric to compute inter-annotator agreement scores for each domain, as shown in Figure~\ref{fig:IAA_domainwise_exclude_singletons}. Annotators have highest agreement on fiction domain (72.45 $\%$), possibly due to large number of pronominal mentions present in literary texts. Annotators on crowdsourcing platforms usually perform well on pronominal mentions, also suggested by our qualitative analysis (\S\ref{sec:qualitative}). The opinion domain consists of magazines discussing the political, economic, social, and cultural evolution of Taiwan during 1996-1998 $\&$ 2000-2001. This text is also rich with pronominal mentions, often discussing about Taiwaneese leadership. Annotators have least agreement on Quizes (59.73$\%$), due to the unique structure of the QuizBowl dataset. This text is rich in cataphoric conferences, a category of coreferences found difficult for annotators on crowdsourcing platforms to resolve. Also, these quizes and the news domain sometimes require world knowledge to identify conferences, making the task harder for annotators. 
% \agcomment{WIP: talk to Marzena, if some arguments from qualitative analysis can support the observations.}



% \begin{figure}[t]
%     \centering
%   %\hspace{-3mm}
%   \includegraphics[width=0.5\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/IAA_domainwise_exclude_singletons_PreCoDivided.pdf}
%   \caption{Inter Annotator Agreement across different domains. B3 scores are computed in accordance with the CoNLL script~\cite{pradhan-etal-2014-scoring}, excluding singletons. Bio (Biographies); Wiki (Wikipedia). \btocomment{could convert to two-row tabular to save space}
%   %\jmcomment{what do the authors of e.g. OntoNotes, Litbank report as their interannotator agreement? Reviewers might not know how good/bad 72.6\% is.} \mkcomment{I agree though it's not that easy as they (if even reported) report different coeficients (\%, B3, alpha, kappa, F1 etc.). Also  it's not on the common set of mentions (right?) so these agreements will mean sth different, and I'm not sure whether all but ON include singletons (I think they do) in their caluculations. That being said I wonder if there is any rule of thumb for IAA measured by B3.} \mkcomment{NOTE: planning to add IAA with singletons - the pattern we see here is gone as the agreeemnt substantially improves with singletons - and matches this in the existing lit. (which includes sing for more of these datasets}
%   }
%   \label{fig:IAA_domainwise_exclude_singletons}
% \end{figure}

% QuizBowl and news domain requires world knowledge.


% News Domain requires world knowledge to resolve some mentions.
% According to OntoNotes, 
% $nw\_wsj\_0290\_0\_0.json$
% Maybe [ he ]e21 did n't start [ it ]e15 , but [ Mohandas Gandhi ]e21 certainly provided a recognizable beginning to [ non-violent civil disobedience as we know [ it ]e15 today ]e15 .

% [ The Mahatma , or `` great souled one , '' ]e21 instigated several campaigns of passive resistance against [ the British government in [ India ]e28 ]e0 

% However, only 2/5 annotators could identify link between Mohandas Gandhi and  The Mahatma , or `` great souled one , ''


% ARRAU news example
% $arrau\_wsjarrau\_0609\_0\_6$

% [ Proponents ]e31 maintain that [ a president ]e24 would choose to use [ a line-item veto ]e9 more judiciously than [ that ]e163 .

% But [ there ]e164 may be [ another problem with [ the device ]e9 ]e165 : Despite [ all the political angst [ it ]e9 would cause ]e166 , [ it ]e9 might n't be effective in cutting [ the deficit ]e27 .

% Annotators disagree over ``a line-item veto" and ``the device". 

% $arrau\_wsjarrau\_0606\_0\_1$, the project and the plant


% Weblogs: vague antecedents.
% $on\_wb\_eng\_0002\_0\_2$

% [ This shift ]e6 is driven by the combination of -LRB- a -RRB- escalating world consumption of petroleum , especially in rapidly developing economies like China and India , and -LRB- b -RRB- the peaking of global oil production capacity , the increasing expense of exploiting the remote and isolated oil reserves that remain , and terrorist / political instability in oil - producing countries .
% S23
% [ This ]e6 is not the oil companies ' fault .
% S24
% [ This ]e6 is not Dick Cheney 's fault .
% S25
% [ This ]e6 is not the auto industries ' fault .
% S26
% [ It ]e6 is not the environmentalists ' fault .
% S27
% [ It ]e6 's the reality of geology and geopolitics .


% Fiction ($lb\_11\_alices\_adventures\_in\_wonderland\_brat\_0\_3$)

% lot of pronoun mentions referring to characters in the story. Agreement high on these mentions.

% agreement on ``you".
% high agreement on resolving pronouns.

% Please , Ma’am , is [ this [ New Zealand ]e22 or [ Australia ]e22 ]e22 ? ’

% ( and [ she ]e0 tried to curtsey as [ she ]e0 spoke -- fancy CURTSEYING as [ you ]e23 ’re falling through [ the air ]e24 !
% S7
% Do [ you ]e23 think [ you ]e23 could manage [ it ]e26 ? )


% $GUM\_fiction\_moon\_0\_0.json$
% Annotators agree on ``the moon" cluster with several [it] mentions. Another cluster is ``I". 

% cases of disagreement in LitBank
% ‘ And [ what ]e28 [ an ignorant little girl ]e0 [ she ]e29 ’ll think [ me ]e0 for asking !

%\vspace{-0.2cm}
\subsection{Agreement with Existing Datasets} 
% Having established relatively good agreement amongst our workers on most domains, we now turn to a different question:
How well do annotations from \ezcoref agree with annotations from existing datasets? 
% To answer this question, we compare the crowd-sourced annotations with the existing annotations provided with respective datasets. 
% \btocomment{maybe mention recent computational F1 scores on ontonotes}
\paragraph{Aggregating annotations:}
To compare crowdsourced annotations with gold annotations, we first require an aggregation method that can combine annotations from multiple crowdworkers to infer coreference clusters. We use a simple aggregation method that determines whether a pair of mentions is coreferent by counting the number of annotators who marked the two mentions in the same cluster.\footnote{Future data collection efforts interested in creating large resources can utilize more advanced aggregation methods~\cite{poesio2019crowdsourced}.} Two mentions are considered as coreferent when the number of annotators linking them together is greater than a threshold ($\tau$). After inferring these pairs of mentions, we construct an undirected graph where nodes are mentions and edges represent coreference links. Finally, we find connected components in the graph to obtain coreference clusters.\footnote{This method resolves to majority voting-based aggregation when the $\tau$ is set so that more than half of annotators should agree. For $\tau=N$, this method is very conservative, adding a link between two mentions only when all annotators agree unanimously. Conversely, for $\tau=1$, only a single vote is required to add a link between two mentions.} We compare aggregated annotations from \ezcoref with gold annotations across the seven datasets using B3 scores (precision, recall, and F1), as illustrated in Figure~\ref{fig:agreement_with_gold_data}. 
% \agcomment{a comment about future work can explore weighted aggregations to improve annotations quality.}
\paragraph{High agreement with OntoNotes, GUM, LitBank, ARRAU:} Our annotators achieve the highest precision with OntoNotes, suggesting that most of the entities identified by crowdworkers are correct for this dataset. In terms of F1 scores, the datasets which are closest to crowd annotations are GUM, LitBank, and ARRAU, all of which are annotated by experts. This result confirms that high-quality annotations can be obtained from non-experts using \ezcoref\ with minimal training.

\begin{figure}[]
    \centering
   %\hspace{-3mm}
   \includegraphics[width=0.5\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/AgreementWithGoldDataWiseScatter.pdf}
  \caption{Agreement with gold annotations across datasets. B3 (F1) scores shown in parentheses are computed with singletons included.
%   \btocomment{is this info a strict subset of fig3? make styling consistent. do we need both?}
%   \agcomment{changed styling. It is a strict subset of Fig 3, although its better to keep it, this information will be very hard to read from Figure 3 due to overlapping curves.}
  %% BTO: ok. the point is to explain to reader.
  }
  \vspace{-0.1in}
  \label{fig:agreement_with_gold_data}
\end{figure}

% \textcolor{red}{This result shows that \ezcoref\ facilitates high quality annotations from untrained crowdworkers.} \agcomment{This result shows that high quality annotations can be obtained from untrained crowdworkers under minimal training.}


% - gold entity density versus our entity density ($\#$entities/$\#$tokens)

% - histogram of chain length ($\#$chains versus chain length) 
% implying that crowd annotators miss many links when compared to gold annotations. During qualitative analysis, we observe that QuizBowl contains multiple cataphoric constructions, which often require factual knowledge in order to correctly annotated (See Table~\ref{table:iaa_examples}, examples (c) and (e)). This is being supported by the low IAA between our annotators.
\paragraph{Low precision with Phrase Detectives and PreCo, low recall with Quiz Bowl:}
We observe that Phrase Detectives has a very low precision compared to all other datasets, implying that crowdworkers add more links compared to gold annotations. Our qualitative analysis reveals that PD annotators miss some valid links, splitting entities which are correctly linked together by our annotators (see \autoref{table:split_entities}). Another dataset with lower precision is PreCo, which also contains many missing links. In general, we observe more actual mistakes in PreCo and PD than in the other datasets, which is not surprising as they were not annotated by experts.\footnote{That said, both PreCo and PD were additionally validated by multiple non-expert annotators.} This result is further validated by our agreement analysis of the fiction domain (\autoref{table:agreement_domain_data}), in which \ezcoref\ annotations agree far more closely with expert annotations (GUM, LitBank) than PreCo and PD. Finally, Quiz Bowl has by far the lowest recall with \ezcoref\ annotations, which is expected given the difficulty with cataphora and factual knowledge (examples (c) and (e) in Table~\ref{table:iaa_examples}).
% \btocomment{can shorten}


\begin{table}[]
\tiny
\begin{tabular}{ll}
PD & \begin{tabular}[c]{@{}l@{}}Not long after \color{teal}{[}a suitor{]}\color{black} \; appeared, and as \color{teal}{[}he{]}\color{black} \; appeared to be very rich and \\the miller could see nothing in \color{teal}{[}him{]}\color{black} \; with which to find fault, he betrothed \\his daughter to \color{teal}{[}him{]}\color{black} \;. But the girl did not care for \color{teal}{[}the man{]}\color{black} \;(...). She did not \\feel that she could trust \color{brown}{[}him{]}\color{black} \;, and she could not look at \color{brown}{[}him{]}\color{black} \; nor think of \\\color{brown}{[}him{]}\color{black} \;without an inward shudder.\end{tabular} \\ \addlinespace[0.2cm]
PreCo & \begin{tabular}[c]{@{}l@{}}When I listened to the weather report, I was afraid to see
\color{violet}{[}the advertisements{]}\color{black} \;.\\ 
\color{magenta}{[}Those colorful advertisements{]}\color{black} \;always made me crazy.\end{tabular}
\end{tabular}
\vspace{-0.05in}
\caption{Cases of split entities (missing links) in annotations provided with Phrase Detectives and PreCo. Instead, our crowd annotators mark all mentions as referring to the same entity in each of these examples.}
\vspace{-0.1in}
\label{table:split_entities}
\end{table}

\begin{table}[h]
\centering \scriptsize
\begin{tabular}{llrrr}
\toprule
\multirow{2}{*}{\textbf{Domain}} & \multirow{2}{*}{\textbf{Dataset}} & \multicolumn{3}{c}{\textbf{B3}} \\ \cline{3-5} \addlinespace[0.05cm]
 &  & \textbf{Precision} & \textbf{Recall} & \textbf{F1} \\  \addlinespace[0.05cm] \hline \addlinespace[0.05cm]
\multirow{4}{*}{Fiction} & GUM & 0.982 & 0.921 & 0.950 \\ \addlinespace[0.05cm]
 & LitBank & 0.959 & 0.927 & 0.943 \\
 & PreCo & 0.805 & 0.963 & 0.877 \\
 & Phrase Detectives & 0.784 & 0.775 & 0.780 \\ \addlinespace[0.1cm]
 \bottomrule 
\end{tabular}
\vspace{-0.05in}
\caption{Agreement with existing datasets for fiction.}
\vspace{-0.1in}
\label{table:agreement_domain_data}
\end{table}


% The annotations from PD dataset seem to also include cases of near-identity as coreferences, given that the guidelines provided for this dataset were minimal in a gamified crowdsourcing setup.

% On the contrary to the above datasets,  OntoNotes has a very high precision suggesting that most of the entities identified by crowd annotators are correct for this dataset. Finally, the datasets which are closest to crowd annotations are GUM, LitBank, and ARRAU. 

% \paragraph{Domain effects:}
% Table~\ref{table:agreement_domain_data} presents the agreement scores for the fiction domain,\kkcomment{again, some kind of baseline (upper or lower bound) will be good for Table 3 and Figure 2. Possible ideas are annotating with a pretrained model, annotating with experts (like us)} further categorized by datasets. For the fiction domain, crowd annotators have lower precision with Phrase Detectives and PreCo, implying annotators add more links (find new entities) on top of gold annotations. However, crowd annotators have high precision and recall with LitBank and GUM datasets, implying that the semantic annotation criteria of these datasets are closest to the crowd's perspective.

\begin{table*}[th]
\centering \tiny
\begin{tabular}{lll}
\toprule
Phenomena & \begin{tabular}[c]{@{}l@{}}Dataset \\ (Domain)\end{tabular} & Example \\ \midrule
 & \begin{tabular}[c]{@{}l@{}}LitBank\\ (Fiction)\end{tabular} & (a) {\color[HTML]{000000} \begin{tabular}[c]{@{}l@{}}A Wolf had been gorging on an animal \color{teal}{[}he{]}\color{black} \; had killed, when suddenly a small bone in the meat stuck in \color{teal}{[}his{]}\color{black} \; throat and \color{teal}{[}he{]}\color{black} \; could not swallow \color{brown}{[}it{]}\color{black}.\\ \color{teal}{[}He{]}\color{black} \; soon felt a terrible pain in \color{teal}{[}his{]}\color{black} \; throat (...) \color{teal}{[}He{]}\color{black} \; tried to induce everyone \color{teal}{[}he{]}\color{black} \; met to remove the bone. "\color{teal}{[}I{]}\color{black} \; would give anything, " said \color{teal}{[}he{]}\color{black} \;, " \\ if \color{purple}{[}you{]}\color{black} \; would take \color{brown}{[}it{]}\color{black} \; out. "\end{tabular}} \\ \addlinespace[0.1cm]
 
\multirow{-3}{*}{Pronouns} & \begin{tabular}[c]{@{}l@{}}GUM\\ (Biographies)\end{tabular} & (b) \begin{tabular}[c]{@{}l@{}}Despite Daniel's attempts at reconciliation, \color{violet}{[}his{]}\color{black} \; father carried the grudge until \color{violet}{[}his{]}\color{black} \; death. Around schooling age, \color{violet}{[}his{]}\color{black} \; father, Johann, encouraged \\ \color{violet}{[}him{]}\color{black} \; to study business (...). However, Daniel refused because \color{violet}{[}he{]}\color{black} \; wanted to study mathematics. \color{violet}{[}He{]}\color{black} \; later gave in to \color{violet}{[}his{]}\color{black} \; father's wish and studied\\ business. \color{violet}{[}His{]}\color{black} \; father then asked \color{violet}{[}him{]}\color{black} \; to study in medicine.\end{tabular} \\ \addlinespace[0.2cm]
Cataphora & \begin{tabular}[c]{@{}l@{}}QuizBowl\\

(Quizzes)\end{tabular} & (c) \begin{tabular}[c]{@{}l@{}}\color{magenta}{[}One character in this work{]}\color{black} \; is forgiven by \color{brown}{[}magenta{]}\color{black} \; wife for an affair with a governess before beginning one with a ballerina. \color{teal}{[}Another character in \\\color{teal} this work {]}\color{black} \; is a sickly, thin man who eventually starts dating a reformed prostitute, Marya Nikolaevna. In addition to \color{magenta}{[}Stiva{]}\color{black} \; and \color{teal}{[}Nikolai{]}\color{black} \;, \color{brown}{[}another \\ \color{brown} character in this work{]}\color{black} \; (...) had earlier failed in \color{brown}{[}his{]}\color{black} \;courtship of Ekaterina Shcherbatskaya.\end{tabular} \\ \addlinespace[0.2cm]

 & \begin{tabular}[c]{@{}l@{}}OntoNotes\\ (News)\end{tabular} & (d) \begin{tabular}[c]{@{}l@{}}The Soviet Union's jobless rate is soaring (...), \color{teal}{[}Pravda{]}\color{black} \; said. Unemployment has reached 27.6 \% in Azerbaijan, (...) and 16.3\% in Kirgizia, \\ \color{teal}{[}the Communist Party newspaper {]}\color{black}\;said.\end{tabular} \\ \addlinespace[0.1cm]
\multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}Factual \\ Knowledge\end{tabular}} & \begin{tabular}[c]{@{}l@{}}QuizBowl\\ (Quizes) \end{tabular} & (e) \begin{tabular}[c]{@{}l@{}}(...) \color{brown}{[} another character in this work {]}\color{black} \; (...) had earlier failed in \color{brown}{[}his{]}\color{black} \;  courtship of \color{magenta}{[}Ekaterina Shcherbatskaya{]}\color{black}. Another character in this work rejects \\ \color{magenta}{[}Ekaterina{]}\color{black} \;  before (...) moving to St. Petersburg. For 10 points name this work in which \color{brown}{[}Levin{]}\color{black} \;  marries \color{magenta}{[}Kitty{]}\color{black} \; , (...) a novel by Leo Tolstoy.\end{tabular} \\ \bottomrule
\end{tabular}
\vspace{-0.1in}
\caption{Representative examples showing unique phenomena in each dataset (coreferences are color coded).}
\vspace{-0.1in}
\label{table:iaa_examples}
\end{table*}
%\vspace{-0.1in}
\paragraph{Varying the aggregation threshold $\tau$:} What is the effect of varying the aggregation threshold ($\tau$)  on precision and recall with gold annotations? Figure~\ref{fig:agreement_with_gold_votingthres} shows that the Quiz Bowl dataset has the highest drop in recall (36\% absolute drop) when increasing $\tau$ from 1 to 5.\footnote{We analyze variations in recall since it is more interpretable than precision, given that the denominator is fixed in recall with a variable number of annotators.}  This indicates that the number of unanimous clusters ($\tau=\num{5}$) is considerably lower than the total number of clusters found individually by all annotators ($\tau=\num{1}$); as such, our annotators heavily disagree about gold clusters in the QuizBowl dataset. 
% Individual annotators identify very different clusters, indicating a higher disagreement not only with gold annotations but also among themselves. 
We observe a similar trend in OntoNotes (26\% drop in recall), whereas Phrase Detectives has the lowest drop in recall (\num{0.07}) with the increase in the number of annotators, 
% suggesting that the number of unanimous clusters ($\tau=\num{5}$) is almost similar to the total number of clusters found individually by all annotators. Thus, annotators agree on many gold clusters in the original dataset,
which is expected since Phrase Detectives is crowdsourced. 

%\agcomment{to myself, discussion points for graphs}

% In Figure~\ref{fig:agreement_with_gold_data}

% QBZ and ON: Low Recall, Annotators miss many links compared to gold.

% PreCo: Low Precision, Annotators add more links compared to gold.

% GUM: FROM Paper: In gold data, annotators were more likely to disregard or not notice a relation than to connect
% entities against the guidelines’ instructions.1

%In Figure~\ref{fig:agreement_with_gold_domain}

% Quiz and Opinion: Annotators miss many links compared to gold, thus missing some potential entities. However, most of the entities discovered by annotators are relevant. 

% Tests: Annotators add more links compared to gold. Annotators retrieve most of the relevant entities according to gold annotations. However, annotators sometimes merge two entities into a common entity. 


% \begin{figure}[t]
%     \centering
%   %\hspace{-3mm}
%   \includegraphics[width=0.5\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/AgreementWithGoldDataWise.pdf}
%   \caption{Agreement with gold annotations across datasets. B3 scores are computed with singletons included.}
%   \label{fig:agreement_with_gold_data}
% \end{figure}

% \begin{figure}[t]
%     \centering
%   %\hspace{-3mm}
%   \includegraphics[width=0.5\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/AgreementWithGoldDataWiseScatter.pdf}
%   \caption{Agreement with gold annotations across datasets. B3 (F1) scores shown in parentheses are computed with singletons included.
% %   \btocomment{is this info a strict subset of fig3? make styling consistent. do we need both?}
% %   \agcomment{changed styling. It is a strict subset of Fig 3, although its better to keep it, this information will be very hard to read from Figure 3 due to overlapping curves.}
%   %% BTO: ok. the point is to explain to reader.
%   }
%   \label{fig:agreement_with_gold_data}
% \end{figure}


% \begin{figure}[t]
%     \centering
%   %\hspace{-3mm}
%   \includegraphics[width=0.5\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/AgreementWithGoldDomainDataWiseScatter.pdf}
%   \caption{Agreement with gold annotations across datasets and domains. B3 scores shown in brackets are computed with singletons included.}
%   \label{fig:agreement_with_gold_domain}
% \end{figure}



% \multirow{3}{*}{News} & ARRAU & 0.946 & 0.943 & 0.944 \\
%  & PreCo & 0.949 & 0.928 & 0.938 \\
%  & OntoNotes & 0.964 & 0.850 & 0.903 \\ \addlinespace[0.05cm]




% In Figure~\ref{fig:agreement_with_gold_votingthres}, 

% Using Recall,
% PD: recall (TP) almost same. correct clusters found are not varying alot with number of annotators -> annotators agree alot on these correct clusters. Can do with less number of annotators.
% QBZ: recall (TP) varies alot. correct clusters found are varying alot with number of annotators -> annotators do not agree alot on these correct clusters. There is high variance in finding correct clusters. Need a lot of annotators for higher confidence. 

% \begin{figure*}[t]
%     \centering
%   %\hspace{-3mm}
%   \includegraphics[width=\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/AgreementWithGoldMajorityVotingThresholdDomainWise.pdf}
%   \caption{Agreement with gold annotations for different domains with varying majority voting threshold ($\tau$). B3 scores are computed with singletons included.}
%   \label{fig:agreement_with_gold_votingthres_domain}
% \end{figure*}

% In Figure~\ref{fig:agreement_with_gold_votingthres_domain}, 

% Using Recall,
% Fiction, Wikipedia and Tests: recall (TP) almost same. correct clusters found are not varying alot with number of annotators -> annotators agree alot on these correct clusters. Can do with less number of annotators.

% Quiz, Opinion, Web, News: recall (TP) varies alot. correct clusters found are varying alot with number of annotators -> annotators do not agree alot on these correct clusters. There is high variance in finding correct clusters. Need a lot of annotators for higher confidence.

% \subsection{Compare Alice in wonderland in LB and PD}
% \agcomment{WIP}
% On common sentences, mentions will vary
% Entities discovered will vary, PD should have more entities
% PD Silver is CS+guidelines
% Ours is CS+minimal guidelines

% To Do:

% 1.IAA on just this file on common sentences.

% 2.Agreement between Our and LB

% 3.Agreement between Our and PD

% 4.Agreement between PD and LB

% \subsection{Compare WSJ in ON and ARRAU}

\subsection{What domains are most suitable for crowdsourcing coreference?}
% \micomment{why is this section before 5.3? it seems much less interesting. perhaps it could be merged somehow}
Which domains yield the highest inter-annotator agreement (IAA) between our crowdworkers? 

\begin{table}[h]
\centering \scriptsize
\begin{tabular}{lllllll}
\toprule
\textbf{Fiction} & \textbf{Bio} & \textbf{Opinion} & \textbf{Web} & \textbf{News} & \textbf{Wiki} & \textbf{Quiz} \\ \midrule
 72.6             & 72.4         & 69.5             & 65.9         & 62.3          & 61.8          & 59.7          \\ \bottomrule
\end{tabular}
%\vspace{-0.05in}
 \caption{Inter Annotator Agreement (B3 \%) across different domains. B3 scores are computed in accordance with the CoNLL script~\cite{pradhan-etal-2014-scoring}, excluding singletons. Bio (Biographies); Wiki (Wikipedia).}
\vspace{-0.1in}
 \label{table:iaa_agreement}
\end{table}
% Are there any domains which are more suitable for crowdsourcing? We measure the inter-annotator agreement (IAA) to answer this question and analyze how crowd behavior varies across domains. 
% \mkcomment{Or: "In order to investigate, which domains are/can potentially be more suitable for crowdsourcing we measure the inter-annotator agreement (IAA) of our annotators.}
We use the B3 metric\footnote{We also computed Krippendorff's $\alpha$ for inter-annotator agreement and obtained similar results.} \cite{bagga-1998-algorithms} to compute IAA for each domain, excluding singletons\footnote{The agreement including singletons is substantially higher. The exact numbers are provided in Appendix \ref{sec:iaa_appendix_singletons}.} (see Table~\ref{table:iaa_agreement}).
We obtain the highest agreement on fiction (72.6$\%$) and biographies (72.4$\%$). This is because both domains contain a high frequency of pronouns (see examples \emph{a} and \emph{b} in Table~\ref{table:iaa_examples}), which our annotators found easier to annotate.
% Furthermore, both domains offer a coherent narrative, which is likely to facilitate the annotation. 
We also observe that the fiction domain contains many well-known children stories (e.g., Little Red Riding Hood) that are likely familiar to our annotators, which may have made them easier to annotate.
Annotators have the least agreement on Quiz Bowl coreference (59.73$\%$), as this dataset is rich in challenging cataphoras (example \emph{c} in Table~\ref{table:iaa_examples}) and often require world knowledge about books, characters, and authors to identify coreferences (example \emph{e} in Table~\ref{table:iaa_examples}).

\begin{figure}[]
    \centering
   %\hspace{-3mm}
   \includegraphics[width=0.48\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/agreement_prec_recall_vary_tau}
    \vspace{-0.1in}
  \caption{Agreement with gold annotations with varying voting threshold $\tau$. $\tau=3$ is majority voting (Figure~\ref{fig:agreement_with_gold_data}). B3 scores computed with singletons included.  
%   \btocomment{use same tick mark spacing (same numbers, thus diff visual spacing) on both axes, as it looks like fig2 now has}
%   \btocomment{note it's voting but not MAJORITY voting if tau is anything other than 3.}
  }
  \vspace{-0.1in}
  \label{fig:agreement_with_gold_votingthres}
\end{figure}


\subsection{Qualitative analysis}
\label{sec:qualitative}

% \begin{table}[]
% \centering \tiny
% \begin{tabular}{lrr} 
% \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Mistakes (our)}} & \multirow{2}{*}{\textbf{Mistakes (gold)}} \\
%                      &    &    \\
% \textbf{PD (silver)} & 22 & 76 \\
% \textbf{PreCo}       & 12 & 33 \\
% \textbf{GUM}         & 48 & 25 \\
% \textbf{OntoNotes}   & 81 & 49 \\
% \textbf{ARRAU}       & 33 & 16 \\
% \textbf{LitBank}     & 21 & 13 \\
% \textbf{QuizBowl}    & 67 & 10
% \end{tabular}
% \caption{Number of mistakes in annotations by our crowd workers and gold annotations provided with respective datasets.}
% \label{table:mistakes}
% \end{table}

% \btocomment{first 3 paras are quantitative. last 3 are examples. examples are more important. cut quant analysis to be very short and high level summary - are we better or worse?, be honest, and dont bother enumerating every one - esp since table in appendix}
% \btocomment{Table 10 appears in appendix for me. If that's intentional, say it's in appendix and drastically cut down discussion here.}
To better understand the differences in annotation quality, we conduct a manual analysis\footnote{Conducted by a linguist who studied annotation guidelines of all datasets.} of all 240 passages in our experiment, comparing our \ezcoref\ annotations to gold annotations from each dataset. Specifically, we look at each link that was annotated by our workers but not in the gold data, or vice versa. For each link, we determine whether crowd or the gold annotations contained a mistake, or whether the discrepancy is reasonable under specific guidelines. We find that \ezcoref\ annotations contain fewer mistakes than non-expert annotated datasets such as PreCo and PD, but there are almost twice as many mistakes as those of expert datasets such as OntoNotes and GUM, and seven times as many mistakes as those in the esoteric Quiz Bowl dataset (\autoref{table:mistakes} in Appendix).

%\vspace{-0.05in}
% Table~\ref{table:mistakes} shows
% a
% nd those of existing datasets, w that we re-annotated using 
% We further manually analyze all 240 passages annotated by our annotators and compare them against the same 240 passages with gold annotations. We annotate each link added and deleted by our annotators as compared with the gold data. We also annotated mistakes in the gold data using their guidelines, whenever applicable. Each link added or missed by our annotators is then further categorized into: \btocomment{no explanation needed for first 3. dont use bullets to save space?} (1) clear mistakes, (2) parser errors, (3) clear improvements, (4) reasonable links: valid links that are sometimes not considered as coreferring in the other datasets, such as copula, appositives, generic mentions, and occasionally near-identity items as defined in \citet{recasens-etal-2010-typology}.


% \btocomment{we need to concede that our entire SYSTEM gives worse data than most of the prev collected datasets. the table is hard to read.  it took me a while to realize you have to sum columns 1+2, versus 3+4, to get worse-vs-better-or-equal.}
% Overall, we find that our annotators add more improvements and reasonable links than they make mistakes, as compared to the original annotations (Table~\ref{table:qual_figures}). The biggest improvement we observe over Phrase Detectives, PreCo, and LitBank, where only a little less than 11\% of added (or deleted) links are undeniable mistakes of our annotators. On the other hand, QuizBowl is the dataset where the largest percentage of links added (or deleted) by our annotators constitutes as a clear mistake (over 47\% links). These results confirm that this QuizBowl is a very challenging dataset requiring either domain knowledge or/and familiarity with the QuizBowl question structure. 

% Furthermore, we observe that our annotators perform better than annotators of Phrase Detectives (silver) and PreCo making three times fewer mistakes than observed in the exact same passages of the original data\footnote{For all gold data we annotate only instances which are clear mistakes as per their guidelines, which are sometimes very limited.}. Our annotators also make slightly fewer mistakes than observed in the same subset of OntoNotes original files. However, they make twice as many mistakes as observed in the same subsets of GUM, ARRAU, and LitBank, and finally almost seven times as many mistakes as in QuizBowl.  \mkcomment{Ankita, do we want to have another table with our mistakes vs gold mistakes in these files? I couldn't make myself to write that we make half of the onto mistakes, though it's true...} We also look more closely at some phenomena, which we observe in our annotations.
\paragraph{Qualitative examples of disagreements and deviations from expert guidelines:}
As in~\citet{Poesio2005AnnotatingA}, we identify cases of genuine ambiguity, where a mention can refer to two different antecedents. The first row of Table~\ref{table:fog_you_examples} shows an example from Dickens' \emph{Bleak House}, where the pronoun ``it'' could reasonably refer to either the ``fog'' or the ``river.'' Our annotators have high disagreement on this link, which is understandable given the literary analysis of~\citet{szakolczai2016novels} who interprets the ambiguity of this pronoun as Dickens' way to show indeterminacy attributed to elements in the scene.\footnote{In LitBank, the source of this passage, the pronoun ``it'' is annotated as referring to the ``river'' as only ``river'' is a potential markable per entity restriction (selects ACE entities only).}

We observe that generic mentions, especially generic pronouns, are almost always annotated as coreferring by our annotators. The second row of Table~\ref{table:fog_you_examples} shows one example of such a case, where annotators unanimously connected all instances of generic ``you.'' While generic pronouns are usually regarded as non-referring \cite{huddleston2002the_you_nonrefering}, they retain something of their specific quality as personal pronouns \cite{quirk1985a_you_retained}.
Furthermore, \citet{Orvell2020} demonstrate that the use of generic ``you'' promotes the resonance between people and ideas. By using the same linguistic form (``you''), often used to refer to the addressee, one invites the addressee to consider how the situation refers to them, and in this sense, the generic ``you'' is being perceived as referring to the same entity, the reader, or, in our case, the annotator. 
Finally, while datasets tend to treat copulae and appositive constructions identically and annotate them in a similar way, our annotators intuitively annotate them differently. 
Although they almost always mark noun phrases in appositive constructions as coreferents, the noun phrases in copulae are linked by majority vote only in $\sim$ 35\% of cases.

% Unsurprisingly, our annotators do not agree on what the pronoun ``it'' refers to, which leads to merging these two entities when less than five annotations are employed. However, upon obtaining five annotations, the majority vote annotates pronoun ``it'' as the antecedent of ``fog.''
% On the other hand, in LitBank, where this passage came from, the pronoun ``it'' is annotated as referring to the ``river'' as only ``river'' is a potential markable per entity restriction (selected ACE entities only).

\begin{table}[]
\tiny
\begin{tabular}{ll}

Ambiguity & \begin{tabular}[c]{@{}l@{}}\color{teal}{[}Fog{]}\color{black} \; everywhere. \color{teal}{[}Fog{]}\color{black}  \; up \color{brown}{[}the river{]}\color{black} \;, where \color{blue}{[}it{]}\color{black} \; flows among green \\ aits and meadows; \color{teal}{[}fog{]}\color{black}  \;  down \color{brown}{[}the river{]}\color{black} \;, where \color{blue}{[}it{]}\color{black} \; rolls defiled  among \\the tiers of shipping and the waterside pollutions of a great (and dirty) city. \\ -  Charles Dickens, \textit{Bleak House} \end{tabular}\\ \addlinespace[0.2cm]

Generic & \begin{tabular}[c]{@{}l@{}}Please , Ma’am , is this New Zealand or Australia? ( and she tried to \\ curtsey as she spoke -- fancy CURTSEYING as \color{violet}{[}you{]}\color{black} \;’re falling \\ through the air! Do \color{violet}{[}you{]}\color{black} \; think \color{violet}{[}you{]}\color{black} \; could manage it?) \\
- Lewis Carroll, \textit{Alice in Wonderland} \end{tabular}

\end{tabular}
\vspace{-0.1in}
\caption{Examples of genuine ambiguity and generic ``you'' observed in our data.}
\vspace{-0.1in}
\label{table:fog_you_examples}
\end{table}
 %\mkcomment{we have the iaa (krip alpha) for copula which is lowe 0.157, sadly we don't have it for appos so I can either skip this or add in footnote}


% Discuss:

% (1) in literature the for/river example, litbank assigns "it" to "river" as in their guidelines "fog" is not a markable

% (2) generic "you" are being assigned to the same cluster; you as the reader -> https://www.pnas.org/content/117/49/31038; example from lb\_11\_alices\_adventures\_in\_wonderland\_brat\_0\_3

% (3) world knowledge

% (1) OntoNotes- definitively better unless world knowledge is needed, splitting  into passages didn't seem to affect the annot

% (2) LitBank - great annotations, sometimes links difficult cause of passage split (rare cases)
% adding a lot of valid links due to the lb restrictions (ACE)

% lb has weird annot style, in appos such as "a, b" they annot BOTH a and b with different numbers (entities)(but also link them?), in copula they do same "a is b" (a and b different entities) - this is different from onto which for appos mark them together [a, b] and for copula mark only the  most specific one "[a] is b". 


% Alice in Wonderland has a weird case where The White Rabbit is treated as a person (and annotated) but when it's being referred to as "it" this is not added to the chain (probably intentionally) -oh wait... they exclude PRO!!!!

% fog/river/it is now resolved with more annotators marking it as part of the fog chain

% (3) qb - very difficult to identify cataphoras (only 1 cata in other sets so far, maybe), need world knowledge and/or structure 

% (4) arrau - wsj - also did good job, arrau sometimes annotates relative pronouns, I'm not sure whether that's intended (looks like it) or by accident but they don't say they do

% (5) pd -our > pd

% (6) Preco -  The dataset seems to have some essays/opinionated articles, fiction, bio, news... Some sentences are missing. Our majorvote doesn't look too well.



% - mistakes

% - newly detected links 

% - examples


% I think we have few major cases to discuss:
% (1) copular expressions - they are being treated in a simplified way as for now, it's inconsistent , and not showing the whole picture. For instance in ONTO they don't mark the NPs in copular expressions as coref, if there is a reference to this entity later ONLY the more detailed of two NPs is chosen and marked but consider this example:
% Jane is a florist. This is her profession. Each day she wakes up early to...
% "Jane" is more specific than "a florist" so she will be marked as coref to "her" and later "she" but "a florist" cannot be marked as a coref to "Jane" and I think also "this" just by this limitation.

% now if "Jane" and "a florist" can be corefs and then "a florist" and "thit" can also be corefs that's also problematic


% There are definitely test cases we can come up for both marking and not marking elements of copular expressions

% and maybe the answer should not be that straightforward anyway

% \textbf{[1] Bare Copular: }A is the B. (He is the culprit)

% Pereltsvaig (2001)  treats: "A is the B" as corefs ("bare" copular). " they are coindexed in syntax, hence coreferential."


% Fiengo and May (1994) treats "A is the B" as coreferential but not coindexed

% \textbf{[2] Equative Copular:} A is B. (The Morning Star is the Evening Star.)

% Heycock and Kroch (1999) - each of the two noun phrases in an equative copular sentence can be modified by a nonrestrictive relative clause hence both NPs are
% referential


% \textbf{Identificational copular}: demonstrative as subj

% Higgins (1979): That (man) is Robert.
% Demonstrative must be understood as having deictic, not anaphoric, reference (Higgins 1979: 220, 224, 245). A is referential while B is Identificational.


% (2) near-ident as defined by R.

% (3) ambiguous as understood by arrau

% (4) generic you/we

% (5) generic mentions

==> EMNLP 2022/emnlp_sections/conclusion.tex <==
\section{Conclusion}
We investigate whether it is feasible to crowdsource coreference annotations by providing \emph{minimal} guidelines to non-expert annotators, thereby saving annotator and researcher efforts. Concretely, we develop a crowdsourced coreference platform called \ezcoref and use it to re-annotate 240 passages from seven existing English coreference datasets. Our crowd workers agree with expert annotations even without extensive training, signifying that high-quality data can be obtained via crowdsourcing with minimalistic guidelines. We also observe crowd deviations from expert guidelines on linguistic phenomena such as general pronouns, appositives, and copulae. 
% Furthermore, we observe high agreement among annotators on familiar texts (e.g., fiction) and low agreement on text rich in cataphoras. 
We hope our observations will inform guideline creation for future coreference annotation efforts.
% In this work, we present \ezcoref, an intuitive and easy-to-use annotation tool to collect crowdsourced annotations for coreference resolution. Using \ezcoref, we re-annotate a subset of documents from seven different English coreference datasets, each of which was created using a different set of complex linguistic guidelines. In contrast, our \ezcoref\ re-annotation aims to collect collect high-quality coreference data with a \emph{minimal} set of guidelines. Our results show that crowdworkers obtain high agreement with many expert annotations (e.g., GUM, ARRAU) and that our annotation quality is better than previous crowdsourced efforts (e.g., Phrase Detectives). 
% % We observe that our annotators (lacking gu almost always mark generic pronouns as coreferring, noun phrases in appositive constructions as coreferents, and disagree over linking noun phrases in copulae constructions.
% We hope our \ezcoref\ tool and observations will inform future research into coreference platform development and guideline construction.
% \agcomment{To myself, add somewhere "Although, we conducted our analysis using AMT, we believe our findings should be equally applicable to both crowdsourcing paradigms, microstasks via AMT and GWAPs."}
% With any data analysis study, our study also has some limitations. Our conclusions can be further strengthened by extending the scale of our experiments, i.e., by collecting more passages across datasets and domains. In order to make the task easier for crowdsourcing, we chose to divide documents into smaller passages, which can potentially miss some coreference links. However, we can address this by cross-document coreference and entity linking. 

==> EMNLP 2022/emnlp_sections/data_collection.tex <==
\section{Using \ezcoref\ to Re-annotate Existing Coreference Datasets}
\label{sec:data_collection}
% To study the behavior of annotators in our setup, we deploy \ezcoref\ on the AMT crowdsourcing platform to re-annotate 240 passages from seven existing datasets, covering seven unique domains. We compare our workers' annotations to each other across domains, compare them to the previous gold standard annotations, and conduct our own qualitative analysis. In total, we collect annotations for 12,200 mentions and 42,108 tokens.

We deploy \ezcoref\ on the AMT crowdsourcing platform to re-annotate 240 passages from seven existing datasets, covering seven unique domains. In total, we collect annotations for 12,200 mentions and 42,108 tokens. We compare our workers' annotations both quantitatively and qualitatively to each other and to existing expert annotations. 


% \agcomment{The goal of this study is to determine the default behavior of crowd annotators. Are there instances where annotators would intuitively annotate certain mentions as coreference versus cases where they disagree? Owing to these observed patterns of agreement (or disagreement), are there certain domains which are more suitable for crowdsourcing coreferences? Finally, out of many existing yet varied annotation criteria and guidelines, which criteria seem more natural to adopt in crowdsourcing setups? To answer these questions, we collect annotations for 12,200 mentions and 42,108 tokens.} 

%\subsection{Experimental Setup}

% \begin{table}[]
% \centering \scriptsize
% \begin{tabular}{llllll}
% \hline
% \textbf{Datasets} & \textbf{Domains} & \textbf{Docs} & \textbf{Passages} & \textbf{Tokens} & \textbf{Mentions} \\ \hline
% \multicolumn{1}{r}{7} & \multicolumn{1}{r}{7} & \multicolumn{1}{r}{83} & \multicolumn{1}{r}{240} & \multicolumn{1}{r}{42108} & \multicolumn{1}{r}{12200} \\ \hline
% \end{tabular}
% \end{table}

% We first describe the data preparation process, then move to the procedure employed during the data collection.

\paragraph{Datasets:}  
We collect coreference annotations for the seven existing datasets described in Table~\ref{table:motivation}: OntoNotes~\cite{hovy-etal-2006-ontonotes}, LitBank~\cite{bamman-etal-2020-annotated}, PreCo\footnote{The PreCo dataset is interestingly large but seems difficult to access. In November 2018 and October 2021 we filled out the data request form at the URL provided by the paper,
and attempted to contact the PreCo official email directly,
%\btocomment{ is that correct? all authors?} \mkcomment{I sent an email to preco@yitu-inc.com on 10/29/2021}  BTO: ok so you did NOT email all coauthors.  one of them may review the paper and get mad that we didn't contact them.  note it has long-time Johns Hopkins researchers who presumably are more responsible than fly-by-night chinese startup people.
but did not receive a response. To enable a precise research comparison, we scraped all documents from PreCo's public demo in November 2018 (no longer available as of 2021); its statistics match their paper and our experiments use this version of the data.
PreCo further suffers from data curation issues \cite{gebru_documentation, Jo2020}; it uses text from English reading comprehension tests collected from several websites,
but the original document sources and copyright statuses
are undocumented. When reading through PreCo documents, we found many domains including opinion, fiction, biographies, and news (\autoref{table:datasets-description-detailed} in Appendix); we use our manual categories for domain analysis. \label{fn:preco}}~\cite{chen-etal-2018-preco}, ARRAU~\cite{Uryupina2019}, GUM~\cite{zeldes-2017-gum}, Phrase Detectives~\cite{chamberlain-etal-2016-phrase}, and QuizBowl~\cite{guha-etal-2015-removing}. The sample covers seven domains: news, opinionated magazines, weblogs, fiction, biographies, Wikipedia articles, and trivia questions from Quiz Bowl. 
% To keep the annotation task simple, we ask workers to annotate passages from documents (on average 175 tokens long, consisting of complete sentences) instead of complete documents.
For each dataset with multiple domains, we manually select domain(s) to re-annotate so that we cover a broad range of domains. From each domain in each dataset, we then select documents and divide them into shorter passages (on average 175 tokens each), creating 20 such passages per dataset. For datasets with multiple domains, we choose 20 such passages per domain (see Appendix~\ref{sec:crowd_data} for detail). Overall, we collect annotations for 240 passages with 5 annotations per passage to measure inter-annotator agreement. 
% \btocomment{Lots of this is wrong or is using sloppy terminology due to domains. We manually selected domains within each dataset. How did we select them? I thought it was to get a broad range of domains. We never randomly sample docs within a dataset, as the last sentence says. We do NOT use all domains from ontonotes, but the above paragraph implies that. Please read it over carefully.}
% \mkcomment{tried to reword it a bit}


% For each dataset, we randomly select and chunk documents, resulting in 20 passages\footnote{As OntoNotes and ARRAU annotate the same documents from Wall Street Journal, and LitBank and Phrase Detectives annotate the same parts of Alice in Wonderland, we additionally choose 10 passages for each of these texts in order to compare the annotations between these datasets.} per domain (see APPENDIX X for detail).
% We ensure that each passage is at least 150 token long (mean=\num{175.45}, std=\num{26.26}), and contains complete sentences only. This approach minimizes the mental fatigue of the annotators, potentially improving the quality of annotations in the local context. However, it can also lead to missing links in the context of the entire document. 
% \agcomment{reworded it}
% %We provide a baseline framework to reconstruct such missing links.
% % \mkcomment{do we?} \agcomment{we can say its future work, or can say that this problem can be formulated as cross-document entity coreference which has been widely researched and neural models exist for same.}
% \mkcomment{thanks for changing it, usually this is something you would say at the end, like this work has these limitations, but that can be addressed in this way. I will leave it here for now with this comment, I think we may wanna move it to the end later if everyone agrees}


% For each dataset, we randomly select and chunk documents, resulting in 20 passages per domain (see APPENDIX X for detail). We ensure that each passage is at least 150 token long (mean=\num{175.45}, std=\num{26.26}), and contains complete sentences only.  \agcomment{keep this sentence if including this analysis} Overall, we annotate 240 passages, collecting five annotations per passage. 

\paragraph{Procedure:}
We first launch an annotation tutorial (paid \$4.50) and recruit the annotators on the AMT platform.\footnote{We allow only workers with a >= 99\% approval rate and at least 10,000 approved tasks who are from the US, Canada, Australia, New Zealand, or the UK.} At the end of the tutorial, each annotator is asked to annotate a short passage (around 150 words). %containing easily identifiable links. 
Only annotators with a B3 score~\cite{bagga-1998-algorithms} of \num{0.90} or higher are then invited to participate in the annotation task. 

\paragraph{Training Annotators with Minimal Guidelines using \ezcoref:}
\begin{figure}[th]
\centering
\includegraphics[width=0.4\textwidth, scale=0.5,clip,trim=0 0 0 0mm]{figs/ezcoref_simplified_efforts.pdf}
\caption{
% Trade-off between effort of annotators and researchers, interested in collecting new coreference datasets.
Existing expert annotated datasets entail high annotator effort (e.g., OntoNotes, ARRAU). Existing crowdsourced coreference datasets (e.g., Phrase Detectives) entail significant researcher effort. In this work, we explore the minimum effort scenario for both annotators (by providing them minimal guidelines) and researchers (by open-sourcing \ezcoref).} 
% \agcomment{this diagram is rough, i still have to carefully think which dataset to place where, and beautify it.}}
% \mkcomment{PreCo-should be a bit higher on the researcher effort and a bit further on annot effort than ezCoref (because of the need to go through and first develop simplified (less than ours) guidelines; they are the most similar but also have a bit more detailed guidelines resulting in annot/researcher efforts going up just a bit; QuizBowl and PD I would assume have similar guidelines as PreCp (can be a bit closer to us cause maybe they are simpler?); the research effort in PD is definitely sky-high; why is it so for QB? need to get experts? GUM has maybe higher researcher efforsts cause they literary spend a semester teaching ppl how to annot? (ragardless of whether that's needed of not, since it's part of the class) LB I would say maybe has less annot effort as the entities are restricted? I don't remember whether they automatically identify them}
\label{figure:motivation_efforts}
%\vspace{-0.1in}
\end{figure}
As the goal of our study is to understand what crowdworkers perceive as coreference and to identify instances of genuine ambiguity, we train our annotators with minimal guidelines. We carefully draft our training examples to include only cases which are considered as coreference by all the existing datasets. The objective is to teach crowdworkers the broad definition of coreference while leaving space for different interpretations of ambiguous cases or those resolved differently across the existing datasets. Note that a comparable experiment with more complex guidelines is infeasible since it is unclear which guidelines to choose, and also providing complex linguistic guidelines to crowdworkers remains an open challenge.
% Overall, \ezcoref\ is aimed to minimize both researcher and annotator effort for new efforts in coreference data collection compared to prior work (\autoref{figure:motivation_efforts}).
Overall, \ezcoref\ is aimed to minimize both researcher and annotator effort for new coreference data collection, in comparison to prior work (\autoref{figure:motivation_efforts}).

% Our setup also helps us explore the feasibility of crowdsourcing coreference annotations with minimal annotator and researcher efforts. In particular, our annotators are trained on simple cases and do not need to refer to lengthy linguistic guidelines used in expert annotated datasets (e.g., OntoNotes), thereby reducing annotator efforts. While GWAPs have made progress in teaching complex guidelines to crowdworkers thereby reducing annotator efforts, they still require higher researcher efforts. In contrast, .\micomment{this is very redundant!}

% \agcomment{here say why other minimal guidelines not needed. Note that an experiment with complex guidelines is not feasible since it is unclear which guidelines to choose from among the varied existing guidelines. Furthermore, teaching these complex linguistic guidelines to crowd annotators still remains challenging, one of the issues raised in this paper}
% At the end of the tutorial, each annotator is asked to annotate a short passage (around 150 words). %containing easily identifiable links. 
% Only annotators with a B3 score~\cite{bagga-1998-algorithms} of \num{0.90} or higher are then invited to participate in the annotation task. 

\paragraph{Worker details:}
Overall, 73 annotators (including 44 males, 20 females, and one non-binary person)\footnote{We did not collect demographic data for the remaining eight individuals, from an earlier pilot experiment.} completed the tutorial task, which took 19.4 minutes on average (sd=11.2 minutes). They were aged between 21 and 69 years (mean=38.9, sd=11.3) and identified themselves as native English speakers. 
Most of the annotators had at least a college degree (47 vs 18). 89.0$\%$ of annotators, who did the tutorial, received a B3 score of 0.90 or higher for the final screening example, and were invited to the annotation task. 50.7$\%$ of the invited annotators returned to participate in the main annotation task, and 29.2\% of them annotated five or more passages. Annotation of one passage took, on average, 4.15 minutes,
a rate of 2530 tokens per hour. 
%\btocomment{report tokens per time speed. i attempted to calculcate. fix if wrong.}
% \btocomment{This number contradicts 600 tok/hr claimed in Related Work earlier tonight (which I now deleted). 175 tok/4.15 min = 2530 tok/hr.}
% \agcomment{600 mentions per hour, not tokens. mentions/tokens = 0.28 approx for our md algo}
% \agcomment{Our speed = 600 mentions per hour. Avg time per passage=4.15 min, average mentions per passage=49, using mentions/tokens for our MD algo is ~0.28 (so 175*0.28=49) approx 40 minutes for 400 mentions. Can say 1.5 times faster than \texttt{CoRefi}}
%and differed greatly depending on the domain
The total cost of the tutorial was \$460.70. We paid \$1 per passage for the main annotation task, resulting in a total cost of \$1440.\footnote{All reported costs include 20$\%$ AMT fee.}




% \section{Data Collection}
% \label{sec:data_collection}
% \subsection{Experimental Setup}
% To gain a crowdsourced perspective of coreference resolution, we use \ezcoref to re-annotate 260 passages from seven existing passages covering nine different domains. We perform a data collection study on Amazon Mechanical Turk (AMT), which also helps us assess \ezcoref's effectiveness in a crowdsourcing environment. We do not limit the number of people who may participate in the study, unlike previous attempts at crowdsourcing coreferences. \mkcomment{citation, citation, citation :), also we do limit the numbers by how many tutorials we launch, what exactly did you mean here?}

% Our goal is to understand how people perceive the concept of coreference resolution and identify instances of genuine ambiguity. Thus, we do not provide any detailed guidelines to our annotators. Instead, we train our annotators minimally by providing only examples of basic coreferences (e.g., pronouns). The objective here is to teach them the broad definition of conference resolution while leaving the space for different interpretations of text, surfacing genuine disagreements among the annotators. Minimal guidelines also ensure that annotators understand the concept of coreference resolution without being overwhelmed with linguistic details and are motivated to annotate a reasonable number of passages.
% \mkcomment{hmm, this is a bit like saying that any more guidelines and they would be NOT willing to do it so kind of saying that this won't work}

% Prior to the ....
% Before participating in our study, we requested every annotator to provide their consent. The annotators were informed about the purpose of this research study, any risks associated with it, and the qualifications necessary to participate. The consent form also elaborated on task details describing what they will be asked to do and how long it will take. The participants were informed that they could choose as many documents as they would like to annotate (by accepting new Human Intelligence Tasks at AMT) subject to availability, and they may drop out at any time. Annotators were informed that they would be compensated in the standard manner through the Amazon Mechanical Turk crowdsourcing platform, with the amount specified in the Amazon Mechanical Turk interface. As part of this study, we also collected demographic information, including their age, gender, native language, education level, and proficiency in the English language. We ensured our annotators that the collected personal information would remain confidential in the consent form.

% In order to identify annotators, who are genuinely interested in our task and weed out spammers, we employ a quality control strategy. \ezcoref allows incorporating a final test example at the end of the tutorial where annotators are asked to annotate a single passage (~150 words) \mkcomment{it's not restricted, right? this number was our choice} without any guidance. They are encouraged to use the concepts they learned during the tutorial to annotate the test example. We use the final test example scores to identify high-performing annotators, whom we then invite to participate in our annotation study. We used the B3 metric~\cite{bagga-1998-algorithms}, a standard evaluation metric used in the coreference literature, to calculate final test example scores. Overall, we launched eight rounds of the tutorial task, where each round consisted of nine invitations. \mkcomment{I don't think we need the number of rounds, we need the number of annot who took the tutorial, how many fialed etc., don't worry with explaining why we launched the tutorials many times} We launched tutorial tasks in multiple rounds because .....\agcomment{i couldnt formulate a good way to say that we did it to avoid paying higher AMT service fee and also space out selection of annotators} The total cost of tutorial tasks was $\sim$ $\$$390, including 20$\%$ AMT service fees \mkcomment{don't need to specify the 20percent, if you want to add it since 390 seems like a lot, then you can add it in the footnote, also this is not the final number as we are paying bonuses etc. I would put a placeholder for now.}. To pass the final test example, an annotator was required to achieve a B3 score of more than 90$\%$. Approximately 90$\%$ of annotators passed the final task, and 55$\%$ of participants who passed returned to participate in the main annotation task. Furthermore, 53$\%$ of these returned annotators submitted annotations for more than five passages. Forty-five annotators self-identified as male, nineteen as female, and one as non-binary. Forty-seven annotators had a college degree, five had graduate school degrees, twelve had secondary education, and one had primary education. All annotators identified English as their native language and considered themselves proficient in English. Most of the annotators are aged between 30-55 years.  Most of the female annotators are aged between 30-45 years, and most male annotators are aged between 35-55 years.
% \agcomment{need to add details about time taken}

% We collect coreference annotations for seven existing datasets, namely OntoNotes, LitBank, PreCo, ARRAU, GUM, QuizBowl, and Phrase Detectives. These datasets cover nine domains, including news, opinionated magazines, weblogs, fiction, English language assessment tests, text from Wikipedia, and quiz questions from a trivia game named Quiz bowl. \agcomment{need to check with Marzena} \mkcomment{will write the domains}

% There are, however, some lengthy documents in these datasets, and having one annotator mark an entire document is not ideal for crowdsourcing platforms since most people prefer short and simple tasks that minimize mental fatigue~\cite{finnerty-etal-2013-keep}. Thus, we utilized a partial annotation framework in which annotators mark only a portion of the entire document. While this approach makes tasks more manageable, it may result in missing coreference links in these partially labeled documents. We provide a baseline framework to reconstruct such missing links. \mkcomment{you don't give up, huh :P}

% For each domain, we select 20 passages with atleast 150 words and atmost 300 words. If a domain exists in more than one dataset, we select 20 passages for this domain from each of the datasets. Passages from domains that appear in multiple datasets allow us to compare their coreference annotations according to varied guidelines. Overall, we collect coreference annotations for 260 passages with median xx words. Further, we use our mention detection heuristics to identify mentions for each of these passages. Finally, for each passage, we collect five annotations. \mkcomment{how were the passages selected? randomly? randomly select file and cut?}

% Annotations were collected on the Amazon Mechanical Turk platform. In order to ensure high-quality annotations, we required annotators to have more than 10,000 HITs approved on the AMT platform and a HIT approval rate of 99$\%$ and above. Annotators were also limited to English-speaking countries, including the United States of America, Canada, New Zealand, Australia, and Great Britain. Annotators were paid $\$$4.5 for the tutorial task, which took a median of XX minutes (mean YY minutes) to complete. We launched each passage as a separate HIT for the main annotation task, where annotators were paid $\$$1 for each HIT. Annotators could decide how many passages they want to annotate. Annotator speeds varied by multiple orders of magnitude (). The total cost of collecting 260 passages with five annotations per passage was $\$$1560, including 20$\%$ AMT service fees. 

% \agcomment{need to add time it took for us to collect data}

% \textbf{Rough Notes}

% Interface/Software Details
%     1. choice of examples in tutorial/ minimal guidelines
%     2. quality control strategy 
%     3. chunking of passages

% Annotations/Data Collection

%     1. experiment choices: num of anno, number of passages, stats

% - randomly choose 20 excerpts from each dataset with regard to the domain, each of about 150-180 token length (mean? std?).
    
%     2. pilot study and main study, cost of annotation, time taken for collecting data, demographics, payment
    
%     - run pilot tutorial, collect feedback
%     - collect data for the main task with 5 annotations per passage
    
%     -list of passages in appendix (original source, how many passages, source corpus...)

%     - intructions for annotators
%     \agcomment{not sure what details are needed?}
    
%     - also MTURK - how filtered, how much paid...
    
    
% \mkcomment{Need to think about the flow... to make this as clear as possible. Maybe subsections like: DATA, ANNOTATORS TRAINING?}

==> EMNLP 2022/emnlp_sections/ethics.tex <==
\section{Ethics Statement}
\label{sec:ethics}

The data collection protocol was approved by the coauthors' institutional review board. All annotators were presented with a consent form (mentioned below) prior to the annotation. They were also informed that only satisfactory performance on the screening example will allow them to take part in the annotation task. All data collected during the tutorial and annotations (including annotators` feedback and demographics) will be released anonymized. 
We also ensure that the annotators receive at least \$13.50 per hour. Since base compensation is per unit of work, not by time (the standard practice on Amazon Mechanical Turk), we add bonuses for workers whose speed caused them to fall below that hourly rate.

\paragraph{Consent}
Before participating in our study, we requested every annotator to provide their consent. The annotators were informed about the purpose of this research study, any risks associated with it, and the qualifications necessary to participate. The consent form also elaborated on task details describing what they will be asked to do and how long it will take. The participants were informed that they could choose as many documents as they would like to annotate (by accepting new Human Intelligence Tasks at AMT) subject to availability, and they may drop out at any time. Annotators were informed that they would be compensated in the standard manner through the Amazon Mechanical Turk crowdsourcing platform, with the amount specified in the Amazon Mechanical Turk interface. As part of this study, we also collected demographic information, including their age, gender, native language, education level, and proficiency in the English language. We ensured our annotators that the collected personal information would remain confidential in the consent form.

==> EMNLP 2022/emnlp_sections/introductionv1.tex <==
% \section{Introduction Skeleton}
% \label{sec:intro}

% \begin{itemize}
%     \item Training coreference systems require lots of data. Several expert annotated and crowdsourced datasets have been collected to this end.

%   \item However, these datasets use different guidelines and annotation standards, making it hard to translate progress in one domain/language to other domains/languages~\cite{universal-anaphora}. Even within the same language and domain (e.g., English fiction), these datasets adopt very different annotation schema and guidelines. \mkcomment{just a comment, but its not like we solve this problem}

%   \item In order to collect data for any new domain/language, one faces an evident challenge, what guidelines and annotation standards to choose from among the existing ones or how to combine them together? \mkcomment{again, here too, we don't solve this problem either; not saying to get rid of it, just pay attention when writing? (how you phrase it)}
  

%   \item it is very expensive to iterate over guidelines/ annotation schema for a new domain, especially since many existing guidelines are extensive (e.g. ontonotes manual is X pages). 
  
%   \item Gamified approaches try to address this problem by XX which is good, but suffers from ... 
  
%   \item In this paper, we examine how well non-expert crowd workers agree with existing guidelines given only minimal training. 

% Our main contributions are:

% \item To collect these annotations, we propose a methodology, including an annotation tool supported with an interactive tutorial which focuses on step-by-step learning via progression, allowing us to teach annotators the broad phenomena of coreference.

% \item We collect annotations for documents from 7 different existing datasets, allowing us to examine the details of conference phenomena as perceived by human annotators without extensive training. 

% \item Using these collected annotations, we investigate several interesting questions such as: 
% \begin{enumerate}
%     \item  Which domains are most suitable for crowdsourcing coreferences? We find that fiction domain is easy.
%     or for which domains where can we expect good quality/good agreement/reasonable annotations?
    
%     \item which types of coref is difficult to annotate in crowdsourcing setups? we find annotators struggle with cataphora.
    
%     \item To what extent do crowd annotators agree with expert annotators? We find annotators agree with expert annotations even without extensive training, signifying that high quality data can be obtained via crowdsourcing with minimalistic guidelines. 
%     \mkcomment{this sounds nice, but not sure (don't remember the numbers) where it's not too strong? }
    
%     \agcomment{i re-read results section today. I think we can say this, perhaps hedge it a bit.}
%     \mkcomment{awesome}
    
%     \item On which linguistic phenomena do annotators agree with experts? We find that appositives and copulae have been annotated similarly by existing guidelines, but annotators naturally mark them differently. We provide qualitative analysis of such cases and highlight cases with genuine ambiguity.
% \end{enumerate}
    
% \item We hope our observations can inform future annotation efforts and guidelines construction.

% \end{itemize}

\section{Introduction}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity
in a given document. Coreference systems are an integral component of the preprocessing pipeline for many downstream tasks, such as summarization~\cite{azzam-etal-1999-using, steinberger-etal-2007-two}, question answering \cite{ vicedo-ferrandez-2000-importance, dhingra-etal-2018-neural}, and machine translation~\cite{hardmeier-2012-discourse, bawden-etal-2018-evaluating}. 

State-of-the-art coreference systems~\citep[e.g., ][]{
% lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert} are trained on large expert-annotated datasets such as OntoNotes~\citep{weischedel-etal-2013-ontonotes}. Collection of such datasets have traditionally involved linguists trained in lengthy guidelines~\citep[e.g.,][]{ontonotes-guidelines} that explain in detail what should and should not be considered coreference (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). 

While many datasets have been curated, these existing coreference datasets vary widely in their annotation guidelines, resulting in inconsistent annotations across languages and domains
% , with challenging cross-lingual and cross-domain issues
~\cite{universal-anaphora}, and even sometimes within the same language and domain (e.g., English news in Figure~\ref{figure:data_guidelines}).


% and PreCo~\citep{chen-etal-2018-preco} .



\begin{table}[]
\centering
\tiny
\begin{tabular}{ll}
\hline
Dataset     & Example                                                                                                                                                                                                                                                                     \\ \hline \addlinespace[0.1cm]
OntoNotes   & \begin{tabular}[c]{@{}l@{}}Maybe we need a \color{teal}{[}CIA{]}\color{black}\;version of the Miranda warning : \\ You have the right to conceal your coup intentions, \\ because we may rat on you .\end{tabular}                                                                                 \\ \addlinespace[0.2cm]

ARRAU       & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the Miranda warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right to conceal \color{magenta}{[}your{]}\color{black}\; {[}coup{]}e16 intentions{]}eS{]}eS, \\ because {[}we{]}eS may rat on \color{red}{[}you{]}\color{black}\;.\end{tabular} \\ \addlinespace[0.2cm]

Crowd (this work) & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the {[}Miranda{]}eS warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right{]}eS to conceal \color{blue}{[}your{]}\color{black}\; coup intentions{]}eS, \\ because \color{brown}{[}we{]}\color{black}\; may rat on \color{blue}{[}you{]}\color{black}\;\end{tabular}    \\ \hline
\end{tabular}
\captionof{figure}{A sentence annotated according to different guidelines. \agcomment{WIP}}
\label{figure:data_guidelines}
\end{table}

% \agcomment{OntoNotes and ARRAU have such detailed guidelines, is coreference underspecified then?}
\agcomment{Crux of para: coref is hard to specify, thus collected by experts taught with lengthy guidelines. But these guidelines differ alot}
Coreference is a complex phenomenon that is difficult to specify to annotators. 
\mkcomment{Yet, all people on the planet do it every day in order to communicate... This doesn't make much sense as it is right now. I know what you want to say but for that I believe this has to be reworded. Also can it even be explained if ppl perceive it differently as it's not a binary IS/IS NOT problem?}
As such, collecting coreference datasets has traditionally involved linguists trained in lengthy guidelines~\citep[e.g.,][]{ontonotes-guidelines} that explain in detail what should and should not be considered coreference (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). Existing coreference datasets vary widely in their annotation guidelines, resulting in inconsistent annotations across languages and domains
% , with challenging cross-lingual and cross-domain issues
~\cite{universal-anaphora}, and even sometimes within the same language and domain (e.g., English news in Figure~\ref{figure:data_guidelines}).
\mkcomment{This sounds much better than before!!!! :)}
% , these datasets~\cite{ontonotes-guidelines, Uryupina2019} adopt very different annotation guidelines (Figure~\ref{figure:data_guidelines} and \autoref{table:motivation}). 
% \citep[e.g., ][]{hovy-etal-2006-ontonotes, poesio-artstein-2008-anaphoric, Uryupina2019}. Datasets such as OntoNotes explain in detail to their annotators what should and should not be considered coreference

% These lengthy guidelines contain complex instructions clarifying how to handle specific linguistic phenomena .

% \mkcomment{I don't think "expertly-collected" sounds good (expertly == skillfully https://www.merriam-webster.com/thesaurus/expertly). I offered a rewrite to this paragraph (connecting it with the following one) but cannot find this comment now. Was that deleted? Maybe sth like this: For instance, datasets, such as OntoNotes, collected by experts, explain what should and should not be considered coreference via legthy guidelines~\cite{ontonotes-guidelines} which contain complex instructions about lingustic paradigms (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). }

% Acquiring these datasets has traditionally been difficult, expensive, and time-consuming, requiring linguists trained in fine-grained annotation schemas \citep[e.g., ][]{hovy-etal-2006-ontonotes, poesio-artstein-2008-anaphoric, Uryupina2019}. For instance, expertly-collected datasets such as OntoNotes explain what should and should not be considered coreference via a lengthy set of guidelines~\cite{ontonotes-guidelines} 
% that covers many complex linguistic details (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). 
% \mkcomment{For instance, datasets, such as OntoNotes, collected by experts, explain in details what should and should not be considered coreference~\cite{ontonotes-guidelines}. The lengthy guidelines contain complex instructions clarifying how to handle specific linguistic phenomena (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). } 
% Furthermore, these datasets differ widely in their annotation guidelines, resulting in inconsistent annotations across languages and domains, with challenging cross-lingual and cross-domain issues \cite{universal-anaphora}.
% \mkcomment{These annotation guidelines vary greatly across datasets, resulting in inconsistent annotations across languages and domains, with challenging cross-lingual and cross-domain issues \cite{universal-anaphora}.}


% \mkcomment{These datasets differ widely in their annotation standards, resulting in inconsistent annotations across languages and domains}
% \mkcomment{"with challenging cross-lingual and cross-domain issues" this is too vague; the next sentence repeats kind of the first sentences. The flow of this paragraph now is: The guidelines are difference (in general)--> this leads to different annot across langs --> within lang still different }


% In order to collect data for any new domain or language, one faces an evident challenge: what guidelines and annotation standards to choose from among the existing ones or how to combine them together? 
\agcomment{Crux of para: coming up with guidelines for a new domain/language is not easy because of these differences in existing guidelines}
In order to collect data for new languages or domains, one has to decide which guidelines to employ.
% Since existing coreference datasets differ widely in terms of what is considered as a mention and what types of links should be annotated (\citet{universal-anaphora} and \autoref{table:motivation}), it is not straightforward to combine these guidelines.
This is not a straightforward task, as the differences in existing guidelines can be significant not only in terms of what can and cannot corefer, but also in what is even considered to be a mention. 
\mkcomment{The above just repeats what's in line 44.}
% (<<== writing again they differ widely in guidelines is a bit too much; btw my rewrite is also poor; I don't like both)} 
Furthermore, it is expensive and time-consuming to iterate over candidate guidelines, requiring expert understanding to resolve differences in choice of mentions and coreference links (e.g., whether mentions related via copulae verb should corefer or should they be treated as a separate special link, requiring expert knowledge of what are copulae and the implications of treating them as coreference versus a special link; \autoref{table:motivation}).

\mkcomment{half of this also repeats what was said before}


% inconsistencies.
\agcomment{reworded}
\micomment{what kind of inconsistencies? why do they require expert understanding?} 
%\mkcomment{this is also a bit awkward}
For instance,~\citet{uryupina2020annotating} iteratively refined their guidelines over approximately 10 years to maximize intercoder agreement when collecting the ARRAU dataset.
%spanning approximately 10 years 
% \mkcomment{here it's not clear what does this mean, this is about PD (crowdsourcing) and they did adjust their guidelines for the GWAP}\agcomment{reworded. Is this clearer?}


To reduce annotation costs, more recent efforts have moved towards crowdsourcing coreference datasets with non-expert workers~\cite{chamberlain-etal-2016-phrase, chen-2018-preco, kicikoglu2019wormingo, madge2019crowdsourcing},
% \mkcomment{Xu, Chamberlain is about correcting errors not corefs per say, though they discuss PD} 
which suffer even more from the lack of standardized guidelines compared to expert data collection.\micomment{suffer in what way?}
\agcomment{not only the choice of guidelines is important, moreover they have to be simple and easy to understand}
\mkcomment{To reduce annotation costs, more recent efforts have moved towards crowdsourcing coreference datasets with non-expert workers~\cite{chamberlain-etal-2016-phrase, chen-2018-preco, kicikoglu2019wormingo, madge2019crowdsourcing}. <--- end sentence here, and maybe write in next that the guidelines for experts are not applicable cause XYZ; need simplified guidelines but this is also hard cause the expert ones are so different to begin with -- just so to not repeat too much (not say again that they different widely)}
% \mkcomment{more than what?}
The crowd annotators are often working on many competing tasks in very short time, mandating concise and easy-to-comprehend guidelines. To address this challenge of  teaching complex linguistic concepts to crowd annotators,  \textit{game with a purpose} (GWAP) methods incorporating a notion of progression have been proposed~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, whereby the annotators start with simpler tasks, and then they are progressively taught more complex tasks. However, developing GWAPs and collecting annotations takes much longer and requires maintaining constant high visibility for it~\cite{poesio2013phrase}.  
\mkcomment{(e.g., it took over 10 years to ...} \micomment{this GWAP stuff is not integrated into the rest of the introduction. you need to break down the different types of crowdsourcing settings (not just GWAP) and then say that we're examining MTurk because you can obtain annotations on it much more rapidly with bigger worker population. and this para should be concise, so don't cite so much stuff and cut details}


\begin{table*}[]
\centering 
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{lccccclcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Domains\\ $\#$(doc, ment, tok)\end{tabular}}} & \multirow{2}{*}{\textbf{Annotators}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{2}{c}{\textbf{Mention Types}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Coreference Links}} &  \\ \cline{5-6} \cline{8-11} \addlinespace[0.05cm]
 &  &  &  & \textbf{Singletons} & \textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}} & \multicolumn{1}{c}{} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} & \textbf{Ambiguity} \\\midrule
 
\textbf{\begin{tabular}[c]{@{}l@{}}ARRAU\\ \cite{Uryupina2019}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (552, 99K, 350K)\end{tabular}  & Single Expert & Manual & Yes & None &  & Special Link & No Link & Yes & Explicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}Phrase Detectives (PD)\\ \cite{chamberlain-etal-2016-phrase}\end{tabular}}& \begin{tabular}[c]{@{}c@{}}Multiple\\ (542, 100K, 400K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Crowd (gamified) +\\ 2 Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semi\\ Automatic\end{tabular} & Yes & None &  & Special Link & Special Link & Yes & Implicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}GUM\\\cite{zeldes-2017-gum}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (25, 6K, 20K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Experts \\ (Linguistics Students)\end{tabular} & Manual & Yes & None &  & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Types)  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Type)  \end{tabular} & Yes & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}PreCo \\ \cite{chen-etal-2018-preco}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple***\\ (38K, 3.58M, 12.5M)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Non-Expert, \\ Non-Native \end{tabular}& Manual** & Yes & None &  & Coref & Coref & Yes & None \\ \addlinespace[0.1cm]

\textbf{\begin{tabular}[c]{@{}l@{}}OntoNotes\\ \cite{hovy-etal-2006-ontonotes}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (1.6K, 94K, 950K)\end{tabular}  & Experts & Mixed & No & None &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}LitBank\\ \cite{bamman-etal-2020-annotated}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (100, 29K, 210K)\end{tabular}  & Experts & Manual & Yes & ACE (selected) &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}QuizBowl\\ \cite{guha-etal-2015-removing}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (400, 9.4K, 50K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Manual\\ \& CRF*\end{tabular} & Yes & \begin{tabular}[c]{@{}c@{}}Characters,\\ Books,\\  Authors*\end{tabular} &  & Coref & Coref & If Applicable & None \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}ezCoref Pilot Dataset 
\\ (this work)\end{tabular}} & Multiple & Crowd (paid) & \begin{tabular}[c]{@{}c@{}}Fully\\ Automatic\end{tabular} & Yes & None &  & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & Implicit \\ \bottomrule
\end{tabular}
\end{adjustbox}

\caption{Summary of seven datasets analyzed in this work,
which 
differ in domain, size, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. }\scriptsize{***See Footnote \ref{fn:preco}.}} 

% \agcomment{ezCoref is not a dataset, should not call last row as ezCoref}\btocomment{changed. i think `ours' sounds bad.}
\label{table:motivation}
\end{table*}

% This work aims at identifying the default behavior of crowd annotators, presented only with minimal guidelines explaining the broad phenomena of coreference. For instance, we explore what are the linguistic phenomena where annotators have disagreements and hence require clarification in the annotation guidelines. What are the cases where annotators most often agree unanimously and should be included in guidelines only if downstream applications expect otherwise? Finally, which cases entail high agreement among annotators but have been resolved differently in existing guidelines? To answer the above questions, we re-annotate a subset of documents from seven different English coreference datasets, encompassing a diverse mix of domains and different set of guidelines. 

In this paper, we examine how well non-expert annotators agree with existing guidelines given only minimal training.\micomment{why are we doing this? currently the motivation for these experiments is not clear} In particular, we re-annotate a subset of documents from seven different English coreference datasets (Table~\autoref{table:motivation}), encompassing a diverse mix of domains and different set of guidelines. To collect these annotations, we teach crowd annotators only the broad concept of coreference, including cases where most of the existing guidelines agree. We explore what are the cases where annotators disagree, and hence require further clarification in the annotation guidelines. Furthermore, we identify cases which most crowd annotators mark a certain way but have been resolved differently in the existing guidelines.\micomment{honestly i think this para is redundant given the contributions list that follows. the intro needs to be shorter anyway so maybe you can cut this}
\agcomment{agreed}
% , and what are the cases which most annotators naturally mark as coreferent, and therefore should be included in the guidelines only if the downstream application expect otherwise.

% we explore what are the linguistic phenomena where annotators disagree on, and hence require further clarification in the annotation guidelines, and what are the cases where annotators show high agreement, and therefore should be included in the guidelines only if the downstream application expect different behavior. Furthermore, we identify cases with high agreement among the crowd annotators that have been resolved differently in the existing guidelines. 
% In order to do so, we re-annotate a subset of documents from seven different English coreference datasets, encompassing a diverse mix of domains and different set of guidelines.


% Consequently, a natural question arises when planning any future coreference data collection efforts: what is a simplified set of guidelines that can be reliably used?
% Should we adopt one of the existing guidelines, or should we combine all the existing guidelines? Since existing coreference datasets differ widely in terms of what is considered as a mention and what types of links should be annotated (\citet{universal-anaphora} and \autoref{table:motivation}), it is not straightforward to combine these guidelines, especially resolving cases that are handled differently by each guideline. These challenges are further exacerbated in crowdsource settings, where annotators are eager to maximize their monetary returns by completing many tasks in a short duration, further mandating short and easy-to-comprehend guidelines.
% \mkcomment{I think that sure "This rises a question" but I would rather approach this from a psycholinguistic perspective. So people consider coreference, when given no guidelines. We didn;t really experiment with simplified guidelines as in what works and what does not, we just "let people do what they want" could potentially connect it to some of these papers about using all annots, etc. as in there is noise but there is also a gunuine disagreeent. TLDR: I think we should do psycholinguistic approach, we investigate what people do when not being forced into any system.}
% \mkcomment{just to bring back Poesio's comment today: ""especially ppl whom you haven't trained to death to agree with you" -- maybe this is the way to frame it}

Following are the main contributions of our work:
\begin{enumerate}
\setlength{\itemsep}{2pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
    % \item We explore whether we can collect high-quality coreference data with a \emph{minimal} set of guidelines, only illustrating basic phenomena like pronoun resolution (\autoref{table:tutorial_example}). \mkcomment{what does it mean high quality}
    
    \item We examine how well non-expert annotators agree with existing guidelines given minimal training, only illustrating basic phenomena like pronoun resolution (\autoref{table:tutorial_example}). 

    \item To collect coreference annotations, we propose a methodology, including an intuitive, easy to use for crowdworkers and open-sourced annotation tool---\texttt{ezCoref}\footnote{Our platform's code and collected data is available in supplementary materials, and will be released publicly after blind review.}---supported with a short, effective, crowd-oriented interactive tutorial\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}"} that features step-by-step learning via progression, allowing us to teach annotators the broad concept of coreference.
    
    \item We re-annotate a subset of documents from seven different English coreference datasets, encompassing a diverse mix of domains and different set of guidelines. Our analysis demonstrate that the crowd annotators obtain high agreement with most of the expert annotations, and the quality of our annotations is higher than that of previous crowdsourced efforts.
    \item Using these collected annotations, we answer several interesting questions such as: 
    \begin{enumerate*}
        \item Which domains are most suitable for crowdsourcing coreferences? We observe highest agreement among crowd annotators for the fiction domain. 

        \item Which types of coreference is difficult to annotate in crowdsourcing setups? We find annotators struggle with cataphora.
        
        % \item To what extent do crowd annotators agree with expert annotators? We find annotators agree with expert annotations even without extensive training, signifying that high quality data can be obtained via crowdsourcing with minimalistic guidelines. 

        \item On which linguistic phenomena do annotators agree with experts? We find that appositives and copulae have been annotated similarly by existing guidelines, but annotators naturally mark them differently.
    \end{enumerate*}
    \item  We conclude with a qualitative analysis of such cases and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and inform coreference platform development.
\end{enumerate}

% Coreference resolution is the task of identifying all textual expressions
% that refer to the same discourse entity
% in a given document, and thus grouping such coreferent expressions (mentions) into clusters (entities). Systems trained to solve this task are often an integral component of the preprocessing pipeline for many downstream tasks, such as summarization~\cite{azzam-etal-1999-using, steinberger-etal-2007-two}, question answering \cite{ vicedo-ferrandez-2000-importance, dhingra-etal-2018-neural}, and machine translation~\cite{hardmeier-2012-discourse, bawden-etal-2018-evaluating}.
% % such as summarization~\cite{azzam-etal-1999-using, steinberger-etal-2007-two}, question answering \cite{morton-1999-using, vicedo-ferrandez-2000-importance, dhingra-etal-2018-neural}, relation extraction \cite{zelenko-etal-2004-coreference, verga-etal-2018-simultaneously}, machine translation \cite{hardmeier-2012-discourse, miculicich-werlen-popescu-belis-2017-using, bawden-etal-2018-evaluating}, and sentiment analysis~\cite{jakob-gurevych-2010-using}.
% Modern coreference systems are implemented via data-hungry neural network models~\citep[e.g., ][]{ lee-etal-2017-end, moosavi-strube-2018-using, joshi-etal-2019-bert} trained on large-scale expert-annotated datasets such as OntoNotes~\citep{weischedel-etal-2013-ontonotes}.
% % and PreCo~\citep{chen-etal-2018-preco}. 

% \begin{figure}[t]
%     \centering
%   %\hspace{-3mm}
%   \includegraphics[width=0.48\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/Interface.pdf}
%   \caption{Part of the \ezcoref interface (\S\ref{sec:software})}
%   \label{figure:interface}
% \end{figure}

% ~\cite{wiseman-etal-2015-learning, clark-manning-2016-deep, lee-etal-2017-end, moosavi-strube-2018-using,  kantor-globerson-2019-coreference, fei-etal-2019-end, joshi-etal-2019-bert},  and various/a number of  datasets~\cite{pradhan-etal-2012-conll, weischedel-etal-2013-ontonotes, poesio-etal-2013-phrase,  cybulska-vossen-2014-using, guha-etal-2015-removing, zeldes-2017-gum, webster-etal-2018-mind, chen-etal-2018-preco, bamman-etal-2020-annotated}. 
% \kkcomment{Can probably move lots of these cites to the related work, currently intro is pretty long and it takes a while until it gets to contributions of work (ezCoref)}

% \agcomment{The OntoNotes and PreCo examples are for language but we are talking about domains too. Also it seems weird to cite so many datasets in previous line and then say that there are only few language or domains} 
% \mkcomment{What's weird is that they keep on making datasets mostly for English and mostly news/informatives, maybe lit.  Anyway I don't think we need these citations in this way. Was that note about datasets always there? somehow remember it saying models but not datasets, seems like we need to clarify that? I mean we are saying there is a lot of datasets then saying we need one. Was it always saying "DIVERSE" datasets? this seems like there are many with many domains etc.}
% \agcomment{yes, we had written models and several datasets and then added citations for both model and datasets}
% \mkcomment{then now it stands out more, "diverse" suggest there are many, and they cover a lot (are very different from each other), changed "diverse" to "various/number of", delete these comments if you agree}





% \begin{table*}[t]
% \centering \scriptsize
% \begin{tabular}{llllcccccc}
% \toprule
% \textbf{Dataset} & \textbf{Domains} & \textbf{Annotators} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{3}{c}{\textbf{Mention Types}} & \multicolumn{3}{c}{\textbf{Coreference Links}} \\ \cmidrule(lr){5-7} \cmidrule(lr){8-10}
%  &  &  &  & \textbf{Singletons} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Entire \\ Appositive\\ Span\end{tabular}}} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} \\ 
%  \midrule
% \textbf{ARRAU} & Multiple & Single expert & Manual & Yes & None & Yes & Special& No Link & Yes \\ \addlinespace[0.2cm]
% \textbf{PD} & Multiple & \begin{tabular}[c]{@{}l@{}}Crowd +\\ 2 experts\end{tabular} & \begin{tabular}[c]{@{}l@{}}Semi\\ automatic\end{tabular} & Yes & None & Yes & Special& Special Link & Yes \\ \addlinespace[0.2cm]
% \textbf{GUM} & Multiple & \begin{tabular}[c]{@{}l@{}}University\\ students with \\ Linguistics\\ background\end{tabular} & Manual & Yes & None & No & Coref (Cop) & Special Link & Yes \\ \addlinespace[0.2cm]
% \textbf{PreCo} & Multiple* & ESL Crowd & Manual** & Yes & None & Yes & Coref & Coref & Yes \\ \addlinespace[0.2cm]
% \textbf{ON} & Multiple & Experts & Mixed & No & None & Yes & Special& Special Link & \begin{tabular}[c]{@{}l@{}}Only with\\ Pronominals\end{tabular} \\ \addlinespace[0.2cm]
% \textbf{LB} & Single & Experts & Manual & Yes & ACE & No & Special& Special Link & \begin{tabular}[c]{@{}l@{}}Only with\\ Pronominals\end{tabular} \\ \addlinespace[0.2cm]
% \textbf{QBZ} & Single & \begin{tabular}[c]{@{}l@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}l@{}}Manual\\ \& CRF\end{tabular} & Yes & \begin{tabular}[c]{@{}l@{}}Characters,\\ Books,\\ Authors*\end{tabular} & No & Coref & Coref & Unspecified \\ \addlinespace[0.2cm]
% \textbf{\ezcoref} & Multiple & Crowd & \begin{tabular}[c]{@{}l@{}}Fully\\ Automatic\end{tabular} & Yes & None & No  &  &  &  \\
% \bottomrule
% \end{tabular}
% \caption{Summary of seven datasets analyzed in this work (abbreviations defined in \S\ref{TODO} \btocomment{cur this is sec2 or sec4.1?? somewhere we need to show/define the boldfaced abbrevs we use in this table and in other tables, along with full names and citations for the datasets.}),
% which differ in domain, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. } \mkcomment{Checking the table for consistancy}}
% \label{table:motivation}
% \end{table*}

% Acquiring these datasets has traditionally been difficult, expensive and time-consuming, requiring linguists trained in fine-grained annotation schemas \citep[e.g., ][]{hovy-etal-2006-ontonotes, poesio-artstein-2008-anaphoric, Uryupina2019}. As such, coreference datasets exist only for a small set of  languages (mostly English) and even then only for limited domains (mainly news and fiction). 
% % \btocomment{is `mainly' a fair summary?} \mkcomment{yes, but should add fiction there}
% Furthermore, these datasets differ widely in their annotation guidelines, resulting in inconsistent annotations across languages and domains,
% with challenging cross-lingual and cross-domain issues \cite{universal-anaphora}.
% %Consider the following sentence that was annotated by both OntoNotes and ARRAU:


%While OntoNotes has only three mentions, ARRAU annotates five mentions, 

% \noindent
% Is it possible to use crowdsourcing and non-expert annotators to generate high-quality coreference data?  As in other types of linguistic annotations, crowdsourcing could reduce costs \cite{snow-etal-2008-cheap}, allowing for larger scale datasets.  Furthermore, by using a standard platform like Amazon Mechanical Turk, this approach is accessible to a wider range of researchers, who may wish to collect new data for different corpora or even languages.


% To this end, we develop \texttt{ezCoref}, a crowdsourced coreference annotation platform that is intuitive and easy to use for crowdworkers, and open-source for other researchers to utilize.\footnote{Our platform's code and collected data is available in supplementary materials, and will be released publicly after blind review.}
% % \ezcoref\ facilitates fast annotations at scale with reduced costs. 
% % \agcomment{need to check this claim, are we reducing costs} \mkcomment{yeah, i think this will always ddepend on how much you are willing to pay (both crowdworkers and linguists... I changed it to possible cost reduction}
% Unlike existing crowdsourced coreference efforts~\cite{chamberlain-etal-2016-phrase, bornstein-2020-corefi, li-etal-2020-active-learning}, \ezcoref\ simplifies the annotation task for workers by using automatically detected mention boundaries\footnote{The syntax-based mention detector is our system's only English-specific component.}, is easily integrable with platforms like Amazon Mechanical Turk, and offers a short, effective, crowd-oriented interactive tutorial\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}"
%  }. %\micomment{add 1-2 more takeaways of the differences} \mkcomment{ankita, we need to look at this when doing final check over zoom}

% In order to train the annotators, we provide a customizable tutorial where annotators are introduced to the annotation task in a fun and interactive manner. Our experiments demonstrate that this tutorial also helps identify annotators genuinely interested in the task.


%  crowdsourcing, which has been demonstrated as a successful approach for several NLP tasks~\cite{snow-2008-cheap, bowman-etal-2015-large, rajpurkar-etal-2016-squad}. 
% This success has led to the development of few annotation
%However, these advances have been hampered, as coreference resolution is a complex linguistic task, which requires not only annotation platform but also simplified yet informative annotation guidelines compatible with crowdsourcing scenario.

%\mkcomment{SIMPLIFY: However, coreference resolution is a complex linguistic task, which requires not only suitable annotation platform but also simplified yet informative annotation guidelines compatible with crowdsourcing scenario /// However, coreference resolution is a complex linguistic task. As such, it requires not only intuitive annotation platform but also simplified yet informative annotation guidelines compatible with crowdsourcing scenario. }

%Standard training procedures used by the existing coreference datasets typically employ lengthy and detailed linguistic guidelines. As such, they are not suitable for crowdsourcing platforms that require task descriptions to be as concise as possible.
% These existing platforms either require annotators to annotate mention pairs~\citep[e.g., ][]{hladka-etal-2009-play, chamberlain-etal-2016-phrase, li-etal-2020-active-learning, ravenscroft-etal-2021-cd},\micomment{what does mention pairs mean? you haven't explained the terminology yet. rewrite into something more intuitive} making the task time-consuming, and therefore less appealing to the crowd workers, or use multiple keyboard key combinations and/or non-intuitive interface \citep[e.g., ][]{bornstein-2020-corefi}, which may be challenging especially for non-experts~\cite{wang-etal-2013-perspectives}.
% \micomment{this paragraph feels out of place. we don't directly compare ezcoref to any of these interfaces, so we can't really claim to be better than them. i think we should just reference them as exsiting work and move onto the main experiments (reannotating existing datasets)}

% \agcomment{will we be offending corefi authors by this statement?}
% \mkcomment{@Ankita: changed the complicated language to multiple keyboard key combinations}

% \agcomment{following two para should be emphasized more}
% With this new interface, we turn to the question of how to define coreference to untrained crowdworkers.
% Expertly-collected datasets such as OntoNotes explain what should and should not be considered coreference via a lengthy set of guidelines~\cite{ontonotes-guidelines} that covers many complex linguistic details (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions).
% %\agcomment{(e.g., how to identify appositive heads and copular structures, some of which should not corefer, which premodifiers can or cannot be linked, etc.)}
% %\micomment{give example in parentheses}\mkcomment{example added} 
% Even if it was feasible to teach such guidelines to crowdworkers, existing coreference datasets differ widely in terms of what is considered as a mention and what types of links should be annotated (\citet{universal-anaphora} and \autoref{table:motivation}), so it is unclear what standards ought to be used.

% Furthermore, crowdsourcing requires concise yet informative guidelines, especially given a complex linguistic task such as coreference resolution.
% Yet, existing annotation guidelines are typically lengthy and cover many linguistic details, some of which may be unnecessary %and can be simplified/omitted/shortened 
% as the annotators would intuitively annotate these types of cases/mentions as coreference.
%they include exhaustive instructions on cases crowd annotators would intuitively annotate as coreferring. 
%details/instructions on cases categories, examples, items, details on annotations crowd workers would do by default, as they include detailed instructions on cases crowd annotator would annotate as corefs by default
%are reflecting the default behavior of the crowd annotators.%As such, they are not suitable for crowdsourcing platforms that require task descriptions to be as concise as possible.
% \mkcomment{this is written as if the system is the main contribution, for now I will leave it as it is as this flow is a bit more coherent}
% \agcomment{we can possibly change the flow in conjunction with the experiments section, since our main arguments for data analysis part are WIP}
% \agcomment{the detailed guidelines are "reflecting the default behavior of the crowd annotators"? I didn't follow this at first. }
% \mkcomment{rewrote it}
% \agcomment{I wonder why this is an issue, or worth mentioning? Traditionally, annotation guidelines must incorporate corner cases where there may be ambiguity, or cases where the task provider wants a specific behaviour from annotators}

%\mkcomment{There is something missing here. You can make an argument "well, but if you simplify, what information do you get out of it". Need to make an argument that: it's even unclear if the lengthy descriptions are needed in the first place, maybe we can get more with less}

% This problem is exacerbated by the fact that the annotation guidelines of the existing datasets differ widely from each other in terms of what is considered as a mention, and what types of links should be annotated~\cite{universal-anaphora} (see FIGURE). Thus, it is unclear which guidelines to employ and how to simplify them so that they will be accessible not only to trained linguists but also to crowd annotators. \jmcomment{Does ezCoref solve this problem or does it introduce another mention detection algo? At this point it's not clear that ezCoref uses its own algorithm or why it's better than existing mention detection criteria. Maybe a one sentence mention that ezCoref uses something better and point to the mention algo section.} \kkcomment{+1 to JM, it's not really clear to me from the intro what exactly ezCoref does that makes it easy for crowdworkers, focusing on mention detection algo + intuitive UI with figure will be helpful}

%the process of familiarizing the annotators with the concept of coreference itself poses a great challenge, requiring deeper analysis. %require more research  

%1existing datasets have different and complicated guidelines
%2if used that than a lot of study
%3hence not feasible for crowdsourcing (also which one to choose anyway)
%4hence we study this

% For instance, consider an example sentence shown in~\ref{fig:motivating_example}, which has been annotated according to seven different annotation guidelines, corresponding to seven coreference datasets drawn from diverse genres and annotation styles. \agcomment{need to fill this up based on example}
% \agcomment{why is this an issue? why having different annotation guidelines a problem?}
% \mkcomment{as to why this is an issue, see my previous comments. need to rewrite this paragraph to make it stronger, dont address reader directly - not to myself}

%Another challenge has been the lack of software that can be easily integrated with crowdsourcing platforms. While there is a number of coreference annotation software designed with crowdsourcing in mind~\cite{chamberlain-etal-2016-phrase, bornstein-2020-corefi, li-etal-2020-active-learning}, they are either time-consuming to set up by the researchers or have a complicated user interface which may pose a challenge for crowd annotators~\cite{wang-etal-2013-perspectives}.
%\mkcomment{Now we are repeating it but I think this should be said earlier where I moved it. (where we first mention the software.}
% \agcomment{I felt like there is a disconnect while moving to this para, can ignore for now}

% Instead, we explore whether we can collect
% high-quality coreference data with a \emph{minimal} set of guidelines, 
% only illustrating basic phenomena like pronoun resolution
% (\autoref{table:tutorial_example}).
% \micomment{add parenthetical about what these guidelines include e.g., pronoun reoslution} \mkcomment{can change to pronoun resolution etc. but I feel like all we give them is what all datasets agree on, and that's strong point, we also list that in a table which we can refer to here} 
% We use \ezcoref\ to re-annotate a subset of documents from seven different English coreference datasets. \agcomment{why? what is the purpose of using so many datasets?} Our crowdworkers
% , each of which uses a different set of guidelines. \mkcomment{that's the third time we mention different set of guidelines, I wonder if we have to have it here?} 
% obtain high agreement with most of the expert annotations, and that the quality of our annotations is higher than that of previous crowdsourced efforts.
% \micomment{not sure if the latter is true, soften if not} \mkcomment{it's true for PD, we made 22 clear mistakes on the part of PD we annotate, compared to 76 or sth clear mistakes of PD; for preco that's 12 our mistakes vs 33 preco's; we do worst on QB, but I don't think that;s really "crowd", proble is that we haven't reported it anywhere yet}.
% \agcomment{Despite \ezcoref's relative lack of guidelines, we observe that our crowdworkers obtain high agreement with most of these expert annotations, and a careful qualitative analysis suggests that our annotations are more reasonable than that of previous crowdsourced efforts.} 
% We conclude with a qualitative analysis of our annotators' behavior and the types of annotation decisions they make, which we hope will inform future research into coreference platform development and guideline construction.
% to determine the default behavior of crowd annotators.  \kkcomment{What is the one line conclusion from this expt? It will be good to mention that here}
% We further investigate the differences in annotations for each of these datasets and compare them against annotations of crowd workers.  
%- getting crowdsource perspective on coref resolution
%This paper is the first to gather and categorize these inconsistencies and provide suggestions for future annotation efforts and evaluation decisions. \mkcomment{it's not the first to gather and categorize inconsistencies}

% Our contributions in this work are threefold: 

%(1)
%we develop ezCoref, a new annotation platform to collect crowdsourced annotations for coreference resolution, (2) We use this platform to gather crowdsourced annotations for seven existing datasets drawn from diverse genres and categorize inconsistencies among their annotation guidelines and 3) Finally, based on our observations, we highlight challenges in crowdsourcing coreferences and provide suggestions for future annotation efforts and evaluation decisions.


% \begin{enumerate}
% \setlength{\itemsep}{2pt}
% \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}

% \item We develop \ezcoref, a new annotation platform to easily collect crowdsource annotations of coreference, that can be used for multiple languages and domains.

% \item We gain a crowdsource perspective on coreference resolution by re-annotating 240 passages from seven existing datasets covering X different domains.
% \mkcomment{add somehow qualitative analysis? nobody does that cause it's so time-consuming, but also insightful - will add below; maybe add how many markables?}

% \item We perform extended quantitative and qualitative analysis showing....  

% \end{enumerate}


% \section{Introduction Rough Notes}
% - coref resolution is a task ... 

% - most corpora are annotated by experts (costly, takes time)

% - but often using different set of guidelines, very detailed guidelines

% - yet unclear why some annot choices were made 

% - alternative - crowdsourcing

% - detailed guidelines is not okay for crowdsourcing. need a way to teach people more intuitively.
%     - teach people the idea of what coref is but rely on ppls perception to decide whether two mentions are coref or not
    
%     -but will it work? because expertise level vary, cant give very detailed guidelines/linguistic knowledge. 

%     -hard to get annotations for long documents on crowdsourcing platforms. People want to do many small tasks as compared to one long task. 

%     - we simplify the task by short docs, easy guidelines, clear interface
    
%     - are we reducing the cost? 
%     - we are reducing time it takes to collect the data. 
%         - learning time is small
%         - power of many people working together
%         - different people working on different segments of a document
    
    
% - based on ppls perception we find that ... 

% - why need to care about disagreements: uncertainty estimates using disagreements among annotators. 
% - real life application: grammarly to identify cases of ambiguity.

% \textbf{Contribution of this paper}:

% - proof of concept - it can be done via crowdsourcing

% - reannotate various corpora to see what the crowd will do vs experts
%     -why???

% - analyzed disagreement, identified cases to include in guidelines
%     - inter annotator disagreements
%     - disagreements with existing guidelines; but annotators unanimously agree

% - our results indicate / show that....

% - clean software + tutorial

% - study can help inform future efforts for collecting annotations for coreference resolution and
% act as a helpful resource for designing annotation
% guidelines
    


% ========================================== 

    
% Recommendations/Advice/Key takeaway
%     1. What to include in tutorial mode
%     2. 




==> EMNLP 2022/emnlp_sections/introductionv2.tex <==
\section{Introduction}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document.
% Building a coreference system, an integral component of the preprocessing pipeline for several downstream tasks, such as summarization~\cite{azzam-etal-1999-using, steinberger-etal-2007-two}, question answering \cite{ vicedo-ferrandez-2000-importance, dhingra-etal-2018-neural}, and machine translation~\cite{hardmeier-2012-discourse, bawden-etal-2018-evaluating}, has been a long-standing goal in NLP research. 
Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase, chen-2018-preco}. \textbf{However, these datasets vary widely in their definition of coreference (expressed through annotation guidelines), resulting in inconsistent annotations both within and across languages and domains~\cite{universal-anaphora} (e.g., English news in Figure~\ref{figure:data_guidelines})}. 


\begin{table}[]
\centering
\tiny
\begin{tabular}{ll}
\hline
Dataset     & Example                                                                                                              \\ \hline \addlinespace[0.1cm]
OntoNotes   & \begin{tabular}[c]{@{}l@{}}Maybe we need a \color{teal}{[}CIA{]}\color{black}\;version of the Miranda warning : \\ You have the right to conceal your coup intentions, \\ because we may rat on you .\end{tabular}                                                                                 \\ \addlinespace[0.2cm]

ARRAU       & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the Miranda warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right to conceal \color{magenta}{[}your{]}\color{black}\; {[}coup{]}e16 intentions{]}eS{]}eS, \\ because {[}we{]}eS may rat on \color{red}{[}you{]}\color{black}\;.\end{tabular} \\ \addlinespace[0.2cm]

Crowd (this work) & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the {[}Miranda{]}eS warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right{]}eS to conceal \color{blue}{[}your{]}\color{black}\; coup intentions{]}eS, \\ because \color{brown}{[}we{]}\color{black}\; may rat on \color{blue}{[}you{]}\color{black}\;\end{tabular}    \\ \hline
\end{tabular}
\captionof{figure}{A sentence annotated according to different guidelines. \agcomment{WIP}}
\label{figure:data_guidelines}
\end{table}

% This lack of a uniform standard guidelines is crucial to address as we move towards collecting larger datasets with broader coverage of languages and domains~\cite{universal-anaphora}. 

To collect a new coreference dataset, one has to decide which guidelines to employ. \textbf{This is not a straightforward task, as the differences in existing guidelines can be significant not only in terms of what can and cannot corefer, but also in what is even considered to be a mention~(\autoref{table:motivation}).} \agcomment{the first para says in one line the main issue addressed in this paper. I wanted to elaborate on this issue in the second para and justify why this isn't a trivial problem to address.} \mkcomment{this repeats what was said two sentences ago: "However, these resources vary
widely in their annotation guidelines"} These differences further make it expensive and time-consuming to iterate over candidate guidelines, requiring expert understanding to resolve inconsistencies. \mkcomment{this is hard to understand, i think i know what you mean, but it's not immediately clear why would you even iterrate over existing guidelines} For instance,~\citet{uryupina2020annotating} iteratively refined their guidelines over approximately 10 years to maximize intercoder agreement when collecting the ARRAU dataset. 

% \mkcomment{did it take them 10y to iterate? I had the impression that the iteration was sth shortish; they do check mistakes each release but I don't think it took them 10y to come up with guidelines (?)}

To reduce annotation cost and time, more recent efforts have moved towards crowdsourcing large coreference datasets, including payment-based approaches~\cite{chen-2018-preco, guha-etal-2015-removing} and games-with-a-purpose (GWAPs) approaches~\cite{chamberlain-etal-2016-phrase}. \textbf{These efforts also face similar challenges, which guidelines to employ for crowdsourcing datasets? Furthermore, crowdsourcing setups must overcome the additional challenge of teaching complex linguistic concepts, such as coreference, to non-expert annotators.} Traditional data collection approaches involve experts (linguists) trained in lengthy guidelines~\citep[e.g.,][]{ontonotes-guidelines} explaining in detail what should and should not be considered coreference (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions).\micomment{redundant sentence} Even if it was feasible to teach such guidelines to crowd annotators, vast differences in guidelines of the existing coreference datasets make it unclear what standards ought to be used.

To address the issue of teaching coreference to crowd annotators, researchers have proposed using the notion of learning by progression~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, whereby the annotators start with simpler tasks, and then they are progressively taught more complex tasks. \textbf{However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks.} As for the issue of lack of standardized guidelines, at the moment, there is only limited consensus on the various aspects of coreference phenomena that should be covered by any annotation guidelines~\cite{universal-anaphora}. \micomment{what does this para add? seems better suited for related work}

% Some proposals have been made to adopt a strategy similar to that of the MATE proposal~(Poesio et al., 1999)- i.e., segregating various aspects of coreference into core and optional aspects. However, existing approaches often decide these differences based on linguistic concepts, and no prior work has accounted for human perspectives.  

In this work, we crowdsource coreference annotations by providing the annotators minimal training, teaching only the broad concept of coreference. \textbf{By observing agreements/disagreements among annotators under minimal training, we aim to understand which coreference concepts are easy to annotate for crowd annotators and which concepts are difficult.} Such an understanding would not only help effective crowdsourcing (e.g., employment of learning by progression strategy) but also help identify difficult concepts to prioritize and elucidate while curating annotation guidelines. 

\agcomment{Another attempt at previous para}
In this work, we crowdsource coreference annotations by providing the annotators minimal training, teaching only the broad concept of coreference. \textbf{We provide minimal training to avoid altering the unbiased/raw/natural perception of annotators. We use these collected annotations to study the deviations of crowd annotations from the existing guidelines. Such deviations can highlight the avenues that must be revisited by the research community for future data collection efforts.} Furthermore, these annotations can also help us understand which coreference concepts are easy/intuitive and difficult for crowd annotators. Such an understanding would not only help effective crowdsourcing (e.g., employment of learning by progression strategy) but also help identify difficult concepts to prioritize and elucidate while curating annotation guidelines. 

Our main contributions in this work are:
\begin{enumerate}
\setlength{\itemsep}{2pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
    % \item We explore whether we can collect high-quality coreference data with a \emph{minimal} set of guidelines, only illustrating basic phenomena like pronoun resolution (\autoref{table:tutorial_example}). \mkcomment{what does it mean high quality}
    \item We examine how well non-expert annotators agree with existing guidelines given minimal training, only illustrating basic phenomena like pronoun resolution (\autoref{table:tutorial_example}). 
    
    \item We \textbf{re-annotate a subset of documents from seven different English coreference datasets}, encompassing a diverse mix of domains and different set of guidelines. 

    \item To collect coreference annotations, we propose a \textbf{methodology}, including an intuitive, easy to use for crowdworkers and open-sourced annotation tool---\texttt{ezCoref}\footnote{Our platform's code and collected data is available in supplementary materials, and will be released publicly after blind review.}---supported with a short, effective, crowd-oriented interactive tutorial\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}"}, allowing us to teach annotators the broad concept of coreference.
    
    \item Using these collected annotations, we \textbf{answer} several interesting questions such as: 
    \begin{enumerate*}
        \item Which domains are most suitable for crowdsourcing coreferences? We observe \textbf{highest agreement among crowd annotators for the fiction domain}. 

        \item Which types of coreference is difficult to annotate in crowdsourcing setups? \textbf{We find annotators struggle with cataphora.}
        
        % \item To what extent do crowd annotators agree with expert annotators? We find annotators agree with expert annotations even without extensive training, signifying that high quality data can be obtained via crowdsourcing with minimalistic guidelines. 

        \item On which linguistic phenomena do annotators disagree with experts? We find that \textbf{appositives and copulae} have been annotated similarly by existing guidelines, but annotators naturally mark them differently and would require clarification in guidelines if expected otherwise.
    \end{enumerate*}
    \item  We conclude with a \textbf{qualitative analysis} of such cases and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and inform coreference platform development.
\end{enumerate}


\begin{table*}[]
\centering 
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{lccccclcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Domains\\ $\#$(doc, ment, tok)\end{tabular}}} & \multirow{2}{*}{\textbf{Annotators}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{2}{c}{\textbf{Mention Types}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Coreference Links}} &  \\ \cline{5-6} \cline{8-11} \addlinespace[0.05cm]
 &  &  &  & \textbf{Singletons} & \textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}} & \multicolumn{1}{c}{} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} & \textbf{Ambiguity} \\\midrule
 
\textbf{\begin{tabular}[c]{@{}l@{}}ARRAU\\ \cite{Uryupina2019}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (552, 99K, 350K)\end{tabular}  & Single Expert & Manual & Yes & None &  & Special Link & No Link & Yes & Explicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}Phrase Detectives (PD)\\ \cite{chamberlain-etal-2016-phrase}\end{tabular}}& \begin{tabular}[c]{@{}c@{}}Multiple\\ (542, 100K, 400K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Crowd (gamified) +\\ 2 Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semi\\ Automatic\end{tabular} & Yes & None &  & Special Link & Special Link & Yes & Implicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}GUM\\\cite{zeldes-2017-gum}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (25, 6K, 20K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Experts \\ (Linguistics Students)\end{tabular} & Manual & Yes & None &  & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Types)  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Type)  \end{tabular} & Yes & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}PreCo \\ \cite{chen-etal-2018-preco}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple***\\ (38K, 3.58M, 12.5M)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Non-Expert, \\ Non-Native \end{tabular}& Manual** & Yes & None &  & Coref & Coref & Yes & None \\ \addlinespace[0.1cm]

\textbf{\begin{tabular}[c]{@{}l@{}}OntoNotes\\ \cite{hovy-etal-2006-ontonotes}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (1.6K, 94K, 950K)\end{tabular}  & Experts & Mixed & No & None &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}LitBank\\ \cite{bamman-etal-2020-annotated}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (100, 29K, 210K)\end{tabular}  & Experts & Manual & Yes & ACE (selected) &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}QuizBowl\\ \cite{guha-etal-2015-removing}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (400, 9.4K, 50K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Manual\\ \& CRF*\end{tabular} & Yes & \begin{tabular}[c]{@{}c@{}}Characters,\\ Books,\\  Authors*\end{tabular} &  & Coref & Coref & If Applicable & None \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}ezCoref Pilot Dataset 
\\ (this work)\end{tabular}} & Multiple & Crowd (paid) & \begin{tabular}[c]{@{}c@{}}Fully\\ Automatic\end{tabular} & Yes & None &  & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & Implicit \\ \bottomrule
\end{tabular}
\end{adjustbox}

\caption{Summary of seven datasets analyzed in this work,
which 
differ in domain, size, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. }\scriptsize{***See Footnote \ref{fn:preco}.}} 
\label{table:motivation}
\end{table*}

% \agcomment{broad area of the paper, recent progress, key limitation}

% \agcomment{give an example of key limitation}

% \agcomment{why and where, addressing this challenge is useful. why addressing this challenge isn't trivial.}

% \agcomment{some existing efforts to address this issue, and one line limitation.}


% \agcomment{what do we do in this paper to address this issue.}


% \agcomment{our contributions}


==> EMNLP 2022/emnlp_sections/introductionv3.tex <==
\section{Introduction}

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\textwidth, scale=0.8,clip,trim=0 0 0 0mm]{figs/motivation_effort.pdf}
\caption{Annotator efforts versus efforts of a researcher interested in collecting new datasets. \ezcoref explores the minimum effort scenario for both annotators and researchers. \agcomment{this diagram is rough, i still have to carefully think which dataset to place where, and beautify it.}}
\mkcomment{PreCo-should be a bit higher on the researcher effort and a bit further on annot effort than ezCoref (because of the need to go through and first develop simplified (less than ours) guidelines; they are the most similar but also have a bit more detailed guidelines resulting in annot/researcher efforts going up just a bit; QuizBowl and PD I would assume have similar guidelines as PreCp (can be a bit closer to us cause maybe they are simpler?); the research effort in PD is definitely sky-high; why is it so for QB? need to get experts? GUM has maybe higher researcher efforsts cause they literary spend a semester teaching ppl how to annot? (ragardless of whether that's needed of not, since it's part of the class) LB I would say maybe has less annot effort as the entities are restricted? I don't remember whether they automatically identify them}
\label{figure:motivation_efforts}
\end{figure}

Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase, chen-2018-preco}. However, these datasets vary widely in their definition of coreference (expressed through annotation guidelines), resulting in inconsistent annotations both within and across languages and domains~\cite{universal-anaphora} (e.g., English news in Figure~\ref{figure:data_guidelines}). 


Because of the differences in the existing guidelines, it is difficult to know which guidelines to use when collecting datasets in a new domain or language. Furthermore, these guidelines frequently include lengthy explanations of complex linguistic concepts~\citep[e.g.,][]{ontonotes-guidelines}, detailing what should and should not be corefer (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). 
% \mkcomment{seems weird with these two e.g.; it's basically the same} 
As a result, coreference datasets have traditionally been curated by linguists (experts) already familiar with such concepts. 
Even so, annotators may have to frequently refer to these guidelines, which results in significant annotator efforts (e.g., OntoNotes and ARRAU as shown in Figure~\ref{figure:motivation_efforts}).  

% In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.

More recently, efforts have been made to crowdsource coreference annotations by utilizing non-experts to annotate large corpora~\cite{chen-2018-preco, chamberlain-etal-2016-phrase}. For instance, applying the games-with-a-purpose (GWAPs) approach~\cite{von-ahn-2006-gwap, poesio2017crowdsourcing, kicikoglu2020aggregation, madge-etal-2019-making}, which emphasizes on fun as a motivator for annotators, researchers have successfully curated coreference datasets~\cite{poesio2019crowdsourced, poesio2013phrase, chamberlain-etal-2016-phrase}. While GWAPs make it interesting and enjoyable \mkcomment{I think GWAP is a fixed term? "game-with-a-pupose" not gameS; you probably can use "GWAPs" is you really want to but I wouldn't use "games-with..."}\agcomment{great point! though, I think gameS-with-a-purpose is equally valid, for instance Poessio uses this term in \url{https://dl.acm.org/doi/pdf/10.1145/2448116.2448119}; section 2.4 and von Ahn, one of the pioneers who popularized this concept, also uses "games"} for non-expert annotators to annotate documents, these methods necessitate significant researcher efforts to build such games and keep them visible for data collection~\cite{poesio-etal-2013-PDoverview} (e.g., Phrase Detectives in Figure~2). Furthermore, even this approach %\mkcomment{this approach; it's not a system, i think} 
is challenged by complex, lengthy guidelines, as non-expert annotators in crowdsourcing setups \mkcomment{in any setup really, and it's kind of crowdsourcing anyway in nlp when you use non-experts, this is redundant} require concise, easy-to-understand guidelines to perform well and remain engaged.

Another alternative for crowdsourcing linguistic annotations, including coreferences, is to use traditional payment-based methods (e.g., Amazon Mechanical Turk)~\cite{snow-2008-cheap, cybulska-vossen-2014-using, roit-etal-2020-controlled, bornstein-2020-corefi}, which are much easier to setup the task \mkcomment{more like easier to recruit the annotators "which offer an easier way to recruit the annotators while offering a dirverse..." - task setup depends on your annot interface, etc.; also not sure about this "diverse" claim; there are very specific ppl on AMT; it's pretty much NOT direverse} and offer a diverse workforce, reducing the researcher's efforts. However, these systems have the same difficulties in teaching complicated linguistic tasks to crowd annotators. \mkcomment{what "systems", I don't think this is the best word choice}


One of the solutions proposed in the literature, also investigated for GWAPs, is to incorporate the \textit{learning by progression} approach~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, where the annotators start with simpler tasks and gradual move towards more complex problems.
% One of the proposed solutions, also investigated for GWAPs, is to use the notion of learning by progression~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, whereby the annotators start with simpler tasks, and then they are progressively taught more complex tasks. \mkcomment{One of the solutions proposed in the literature is to incorporate the \textit{learning by progression approach}, where the annotators start with simpler tasks and gradual move towards more complex problems.} 
However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks. \mkcomment{However, in order to efficiently employ the \textit{learning by progression} approach, researchers have to identify which cases are .... }

\mkcomment{this transition is a bit rough; you mention the need to identiry these easy vs difficult cases and then switch to another topic without saying that this is what we do... should finish that thing first, then switch to minimal guidelines as a way to coref}
In this work, we investigate whether it is feasible to crowdsource coreference resolution under minimal guidelines. For instance, annotations for pronoun resolution which are very useful for information extraction tasks can be obtained via minimal training, as observed in our experiments. If we can obtain good annotations via minimal training, that can speed up the process and make it easier for other researchers to collect new datasets, thereby reducing both annotator and researcher efforts. 

In particular, we propose a methodology---\texttt{ezCoref}---which includes an intuitive, easy to use for crowdworkers and open-sourced annotation tool,\footnote{Our platform's code and collected data is available in supplementary materials, and will be released publicly after blind review.} supported with a short, effective, crowd-oriented interactive tutorial,\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}"} allowing us to teach annotators the broad concept of coreference. Using \texttt{ezCoref}, we re-annotate 240 passages from seven existing English coreference datasets and for the first time compare the quality of crowdsourced coreference annotations against those of experts, and identify where their behavior differs to facilitate future annotation efforts.

We obtain a high agreement among annotators for the fiction domain, suggesting that this domain is suitable to collect crowdsourced coreference annotations. Comparing various linguistic concepts, we find that annotators struggle with cataphoras, resulting in multiple mistake when annotating QuizBowl dataset~\cite{guha-etal-2015-removing}. Finally, comparing the expert guidelines with crowd annotations, we find that appositives and copulae have been annotated similarly by existing guidelines, but annotators naturally mark them differently and would require clarification in guidelines if expected otherwise. \mkcomment{<---this sentence is not the smoothest, the point of it is too far in the forest; Finally, we find that non-expert annotators tend to annotate metions in appositives and copulae as coreferent, even though most of existing guidelines connected these with another, special link. ....though that is not true either right... they don't tend to do that, they are all over the place with copula but maybe better with appos, then it's the question of major vote} We conclude with a qualitative analysis of such cases and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and inform coreference platform development.


\begin{table}[]
\centering
\tiny
\begin{tabular}{ll}
\hline
Dataset     & Example                                                                                                              \\ \hline \addlinespace[0.1cm]
OntoNotes   & \begin{tabular}[c]{@{}l@{}}Maybe we need a \color{teal}{[}CIA{]}\color{black}\;version of the Miranda warning : \\ You have the right to conceal your coup intentions, \\ because we may rat on you .\end{tabular}                                                                                 \\ \addlinespace[0.2cm]

ARRAU       & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the Miranda warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right to conceal \color{magenta}{[}your{]}\color{black}\; {[}coup{]}e16 intentions{]}eS{]}eS, \\ because {[}we{]}eS may rat on \color{red}{[}you{]}\color{black}\;.\end{tabular} \\ \addlinespace[0.2cm]

Crowd (this work) & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the {[}Miranda{]}eS warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right{]}eS to conceal \color{blue}{[}your{]}\color{black}\; coup intentions{]}eS, \\ because \color{brown}{[}we{]}\color{black}\; may rat on \color{blue}{[}you{]}\color{black}\;\end{tabular}    \\ \hline
\end{tabular}
\captionof{figure}{A sentence annotated according to different guidelines. \agcomment{WIP}}
\label{figure:data_guidelines}
\end{table}


\begin{table*}[]
\centering 
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{lccccclcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Domains\\ $\#$(doc, ment, tok)\end{tabular}}} & \multirow{2}{*}{\textbf{Annotators}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{2}{c}{\textbf{Mention Types}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Coreference Links}} &  \\ \cline{5-6} \cline{8-11} \addlinespace[0.05cm]
 &  &  &  & \textbf{Singletons} & \textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}} & \multicolumn{1}{c}{} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} & \textbf{Ambiguity} \\\midrule
 
\textbf{\begin{tabular}[c]{@{}l@{}}ARRAU\\ \cite{Uryupina2019}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (552, 99K, 350K)\end{tabular}  & Single Expert & Manual & Yes & None &  & Special Link & No Link & Yes & Explicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}Phrase Detectives (PD)\\ \cite{chamberlain-etal-2016-phrase}\end{tabular}}& \begin{tabular}[c]{@{}c@{}}Multiple\\ (542, 100K, 400K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Crowd (gamified) +\\ 2 Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semi\\ Automatic\end{tabular} & Yes & None &  & Special Link & Special Link & Yes & Implicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}GUM\\\cite{zeldes-2017-gum}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (25, 6K, 20K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Experts \\ (Linguistics Students)\end{tabular} & Manual & Yes & None &  & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Types)  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Type)  \end{tabular} & Yes & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}PreCo \\ \cite{chen-etal-2018-preco}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple***\\ (38K, 3.58M, 12.5M)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Non-Expert, \\ Non-Native \end{tabular}& Manual** & Yes & None &  & Coref & Coref & Yes & None \\ \addlinespace[0.1cm]

\textbf{\begin{tabular}[c]{@{}l@{}}OntoNotes\\ \cite{hovy-etal-2006-ontonotes}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (1.6K, 94K, 950K)\end{tabular}  & Experts & Mixed & No & None &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}LitBank\\ \cite{bamman-etal-2020-annotated}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (100, 29K, 210K)\end{tabular}  & Experts & Manual & Yes & ACE (selected) &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}QuizBowl\\ \cite{guha-etal-2015-removing}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (400, 9.4K, 50K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Manual\\ \& CRF*\end{tabular} & Yes & \begin{tabular}[c]{@{}c@{}}Characters,\\ Books,\\  Authors*\end{tabular} &  & Coref & Coref & If Applicable & None \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}ezCoref Pilot Dataset 
\\ (this work)\end{tabular}} & Multiple & Crowd (paid) & \begin{tabular}[c]{@{}c@{}}Fully\\ Automatic\end{tabular} & Yes & None &  & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & Implicit \\ \bottomrule
\end{tabular}
\end{adjustbox}

\caption{Summary of seven datasets analyzed in this work,
which 
differ in domain, size, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. }\scriptsize{***See Footnote \ref{fn:preco}.}} 
\label{table:motivation}
\end{table*}


\ignore{
\subsubsection{bullet points}
Existing datasets differ widely in their guidelines, so we don’t know which one to employ for new data collection. 

These guidelines are often complex with many arbitrary decisions.

Complex guidelines require experts but collecting annots with experts is expensive and time consuming (small num of experts working on large num of docs)

Crowdsourcing is a non-expert alternative which was recently done by using GWAP - but that is also time consuming (development, PR); the annotators may be motivated (yay, it’s a game!) but they need simplified guidelines

Alternative is traditional crowdsourcing but just as GWAP it requires simplified guidelines - teach ppl what you want (ppl can resolve coref naturally, but need to explain them the task)

One of the proposed solutions applied also in GWAP is to use the notion of learning by progression = iterating through concepts from easy to difficult cases. But for it to be done well with minimum time from workers => it requires researchers to identify what is hard and what is easy for a better / more efficient design

In this work, we try to address this question. We collect annotations under minimal training to identify what is hard and easy for annotators. Furthermore, deviations from existing expert guidelines can help inform avenues to revisit.

\subsection{text}
\agcomment{WIP}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase, chen-2018-preco}. However, these datasets vary widely in their definition of coreference (expressed through annotation guidelines), resulting in inconsistent annotations both within and across languages and domains~\cite{universal-anaphora} (e.g., English news in Figure~\ref{figure:data_guidelines}). 

Coreference datasets vary in terms of their definition of coreference expressed via different guidelines, annotation formats and annotation platform used to collect the dataset. All these differences have impacts on the quality of collected data. These datasets not only differ in terms of what is coreference but also what is considered as a mention. Unfortunately, at the moment, there is only limited consensus on the various aspects of coreference phenomena that should be covered by any annotation guidelines~\cite{universal-anaphora}

In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.

Another complimentary dimension in which these datasets differ is how these datasets were collected. Traditionally, these datasets such as OntoNotes were collected via expert annotators trained in lengthy guidelines. More recently, impressive progress has been made towards crowdsourcing coreference annotations. Both payment based approaches and games-with-a-purpose has been proposed and impressive success has been achieved e.g., as demonstrated by the success of Phrase Detectives. However, GWAPs are often not open-sourced and require maintaining constant visibility to collect annotations, thereby significantly increasing researcher efforts to collect new datasets. 

In this work, we investigate whether it is feasible to crowdsource coreference resolution under minimal guidelines? For instance, annotations for pronoun resolution which are very useful for information extraction tasks can be obtained via minimal training, as observed in our experiments. If we can obtain good annotations via minimal training, that can speed up the process and make it easier for other researchers to collect new datasets.
}



% \agcomment{broad area of the paper, recent progress, key limitation}

% \agcomment{give an example of key limitation}

% \agcomment{why and where, addressing this challenge is useful. why addressing this challenge isn't trivial.}

% \agcomment{some existing efforts to address this issue, and one line limitation.}

% \agcomment{what do we do in this paper to address this issue.}

% \agcomment{our contributions}

==> EMNLP 2022/emnlp_sections/introductionv4.tex <==
\section{Introduction}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.5\textwidth, scale=0.8,clip,trim=0 0 0 0mm]{figs/motivation_effort.pdf}
% \caption{Annotator efforts versus efforts of a researcher interested in collecting new datasets. \ezcoref explores the minimum effort scenario for both annotators and researchers. \agcomment{this diagram is rough, i still have to carefully think which dataset to place where, and beautify it.}}
% % \mkcomment{PreCo-should be a bit higher on the researcher effort and a bit further on annot effort than ezCoref (because of the need to go through and first develop simplified (less than ours) guidelines; they are the most similar but also have a bit more detailed guidelines resulting in annot/researcher efforts going up just a bit; QuizBowl and PD I would assume have similar guidelines as PreCp (can be a bit closer to us cause maybe they are simpler?); the research effort in PD is definitely sky-high; why is it so for QB? need to get experts? GUM has maybe higher researcher efforsts cause they literary spend a semester teaching ppl how to annot? (ragardless of whether that's needed of not, since it's part of the class) LB I would say maybe has less annot effort as the entities are restricted? I don't remember whether they automatically identify them}
% \label{figure:motivation_efforts}
% \end{figure}

Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated datasets~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase}. However, these datasets vary widely in their definitions of coreference and annotation guidelines, resulting in inconsistent annotations both within and across domains and languages. For instance, in a common English news sentence, while ARRAU~\cite{Uryupina2019} treats generic pronouns as non-referring, OntoNotes chooses not to mark them at all (Figure~\ref{figure:data_guidelines}). 
% ~\cite{universal-anaphora}
%(e.g., English news in Figure~\ref{figure:data_guidelines}). 


% \begin{quote}
% \small
% \textbf{OntoNotes}: Maybe we need a {\color{red}[} CIA {\color{red}\texttt{]e1}} version of the Miranda warning: You have the right to conceal your coup intentions, because we may rat on you. \vspace{0.2cm}\\
% \textbf{ARRAU}: Maybe {\color{teal}[} we {\color{teal}\texttt{]e1}} need a {\color{red}[} CIA {\color{red}\texttt{]e2}} version of the Miranda warning: {\color{blue}[} You {\color{blue}\texttt{]e1}} have the right to conceal {\color{orange}[} your {\color{orange}\texttt{]e1}} coup intentions, because {\color{brown}[} we {\color{brown}\texttt{]e1}} may rat on {\color{violet}[} you {\color{violet}\texttt{]e1}}. \vspace{0.2cm}\\
% \textbf{Crowd (this work)}: Maybe {\color{teal}[} we {\color{teal}\texttt{]e1}} need {\color{red}[} a {\color{ForestGreen}[} CIA {\color{ForestGreen}\texttt{]e2}} version of the Miranda warning {\color{red}\texttt{]e2}}: {\color{blue}[} You {\color{blue}\texttt{]e1}} have {\color{magenta}[} the right {\color{magenta}\texttt{]e1}} to conceal {\color{orange}[} {\color{blue}[} your {\color{blue}\texttt{]e1}} coup intentions {\color{orange}\texttt{]e1}} , because {\color{teal}[} we {\color{teal}\texttt{]e1}} may rat on {\color{blue}[} you {\color{blue}\texttt{]e1}}. \vspace{0.2cm}\\
% \end{quote}

% \begin{quote}
% \small
% \textbf{OntoNotes}: {\color{red} \texttt{[}} Lloyd's, once a pillar of {\color{blue} \texttt{[}} the world insurance market {\color{blue} \texttt{]e1}}, {\color{red} \texttt{]e2}} is being shaken to {\color{red} \texttt{[}} its {\color{red} \texttt{]e2}} very foundation.\vspace{0.2cm}\\
% \textbf{ARRAU}: {\color{red} \texttt{[}} Lloyd's, once {\color{violet}\texttt{[}} a pillar of {\color{blue}\texttt{[}} the world {\color{teal}\texttt{[}} insurance {\color{teal}\texttt{]e3}} market \texttt{{\color{blue}]e2} {\color{violet}]eS1} {\color{red} ]e1}}, is being shaken to \texttt{{\color{brown}[} {\color{red}[}} its {\color{red}\texttt{]e1}} very foundation {\color{brown} \texttt{]eS2}}.
% \end{quote}

% \begin{table}[t]
% \centering
% \tiny
% \begin{tabular}{ll}
% \hline
% Dataset     & Example                                                                                                              \\ \hline \addlinespace[0.1cm]
% OntoNotes   & \begin{tabular}[c]{@{}l@{}}Maybe we need a \color{teal}{[}CIA{]}\color{black}\;version of the Miranda warning : \\ You have the right to conceal your coup intentions, \\ because we may rat on you.\end{tabular}                                                                                 \\ \addlinespace[0.2cm]

% ARRAU       & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the Miranda warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right to conceal \color{magenta}{[} \color{orange}{[}your{]} \color{magenta}{[}coup{]}\color{magenta}\; intentions{]}\color{black}, \\ because \color{violet}{[}we{]}\color{black}\; may rat on \color{red}{[}you{]}\color{black}.\end{tabular} \\ \addlinespace[0.2cm]

% Crowd (this work) & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the {[}Miranda{]}eS warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have \color{orange}{[}the right{]}\color{black}\; to 
% \color{magenta}{[}conceal \color{blue}{[}your{]} \color{magenta} coup intentions{]}\color{black}, \\ because \color{brown}{[}we{]}\color{black}\; may rat on \color{blue}{[}you{]}.\color{black}\;\end{tabular}    \\ \hline
% \end{tabular}
% \captionof{figure}{A sentence annotated according to two different guidelines and our crowd annotators. \agcomment{WIP}}
% \label{figure:data_guidelines}
% \end{table}

\begin{figure}[t]
    \centering
  %\hspace{-3mm}
  \includegraphics[width=0.45\textwidth, scale=0.7,clip,trim=0 0 0 0mm]{emnlp2022-latex/EMNLP 2022/figs/motivation_guidelines.pdf}
  \caption{A common sentence annotated by both OntoNotes~\cite{hovy-etal-2006-ontonotes} and ARRAU~\cite{Uryupina2019}. We visualize both annotations along with the crowd annotations obtained in our study using \ezcoref\ platform. 
  While OntoNotes does not mark generic pronouns and ARRAU marks them as non-referring mentions, our crowdworkers mark all generic pronouns (e.g., ``you'' and ``we'') as coreferent.}
  \vspace{-0.1in}
%   \caption{This sentence was annotated by both OntoNotes~\cite{hovy-etal-2006-ontonotes} and ARRAU~\cite{Uryupina2019}. Each dataset's respective coreference annotations are shown above, along with annotations by crowdworkers using our \ezcoref\ platform. 
% %   OntoNotes and ARRAU themselves differ in their definitions of mentions and coreferences. cx
%   While OntoNotes does not mark generic pronouns and ARRAU marks them as non-referring mentions, our crowdworkers mark all generic pronouns (e.g., ``you'' and ``we'') as coreferent. 
% %   We do not show entity ids for most of the singletons for visual clarity.
%   }
\label{figure:data_guidelines}
\end{figure}

% \footnotetext{Entity annotations for most singletons omitted for visual clarity.}
% A common sentence drawn from two datasets, OntoNotes and ARRAU, with gold annotations as per their guidelines and re-annotated by our crowdworkers by using \ezcoref. While OntoNotes and ARRAU themselves differ in their definition of mentions and coreferences, crowdworkers with minimal guidelines have a completely different perception compared to these two datasets. OntoNotes does not mark generic pronouns, ARRAU marks generic pronouns as non-referring, however, crowdworkers naturally mark generic pronouns as coreferent.

When collecting a new coreference dataset, how should the annotation guidelines be chosen? Traditionally, these guidelines have leaned towards lengthy explanations of complex linguistic concepts, such as those in the OntoNotes guidelines~\citep{ontonotes-guidelines}, which detail what should and should not be coreferent (e.g., how to deal with head-sharing noun phrases, premodifiers, and generic mentions). 
As a result, coreference datasets have traditionally been annotated by linguists (experts) already familiar with such concepts, and this reliance on experts makes the process expensive and time-consuming. Crowdsourced coreference data collection has the potential to be significantly cheaper and faster; however, teaching an exhaustive set of linguistic guidelines to non-expert crowd workers remains a formidable challenge. As a result, there has been a growing interest among researchers in curating a unified set of guidelines~\cite{universal-anaphora} suitable for annotators with various backgrounds. 

More recently, one of the proposed solution to crowdsource large coreference datasets~\cite{chamberlain-etal-2016-phrase} is to use games-with-a-purpose (GWAPs)~\cite{von-ahn-2006-gwap}, such as Phrase Detectives~\citep{poesio-etal-2013-PDoverview}. While GWAPs make it enjoyable for crowdworkers to learn complex guidelines and perform annotations using them~\cite{madge2019progression}, they also require significant effort to attract and maintain workers (e.g., Phrase Detectives Corpus 1.0 was collected over a span of six years~\cite{chamberlain-etal-2016-phrase, poesio2013phrase}), which motivates us to instead study coreference collection on more efficient payment-based platforms.
% and are often not open-sourced, making them inaccessible to other researchers interested in collecting new datasets.


% , including payment-based microtasks and games-with-a-purpose (GWAPs)~\cite{von-ahn-2006-gwap, poesio-etal-2013-PDoverview},

% Even so, annotators may have to frequently refer to these guidelines, which results in significant annotator efforts (e.g., OntoNotes and ARRAU as shown in Figure~\ref{figure:motivation_efforts}).  

% In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.
%Because of the differences in the existing guidelines, it is difficult to know which guidelines to use when collecting datasets in a new domain or language. Furthermore, these guidelines frequently include lengthy explanations of 

% More recently, efforts have been made to crowdsource coreference annotations by utilizing non-experts to annotate large corpora~\cite{chen-2018-preco, chamberlain-etal-2016-phrase}. For instance, applying the games-with-a-purpose (GWAPs) approach~\cite{von-ahn-2006-gwap, poesio2017crowdsourcing, kicikoglu2020aggregation, madge-etal-2019-making}, which emphasizes on fun as a motivator for annotators, researchers have successfully curated coreference datasets~\cite{poesio2019crowdsourced, poesio2013phrase, chamberlain-etal-2016-phrase}. While GWAPs make it interesting and enjoyable \mkcomment{I think GWAP is a fixed term? "game-with-a-pupose" not gameS; you probably can use "GWAPs" is you really want to but I wouldn't use "games-with..."}\agcomment{great point! though, I think gameS-with-a-purpose is equally valid, for instance Poessio uses this term in \url{https://dl.acm.org/doi/pdf/10.1145/2448116.2448119}; section 2.4 and von Ahn, one of the pioneers who popularized this concept, also uses "games"} for non-expert annotators to annotate documents, these methods necessitate significant researcher efforts to build such games and keep them visible for data collection~\cite{poesio-etal-2013-PDoverview} (e.g., Phrase Detectives in Figure~2). Furthermore, even this approach %\mkcomment{this approach; it's not a system, i think} 
% is challenged by complex, lengthy guidelines, as non-expert annotators in crowdsourcing setups \mkcomment{in any setup really, and it's kind of crowdsourcing anyway in nlp when you use non-experts, this is redundant} require concise, easy-to-understand guidelines to perform well and remain engaged.

% Another alternative for crowdsourcing linguistic annotations, including coreferences, is to use traditional payment-based methods (e.g., Amazon Mechanical Turk)~\cite{snow-2008-cheap, cybulska-vossen-2014-using, roit-etal-2020-controlled, bornstein-2020-corefi}, which are much easier to setup the task \mkcomment{more like easier to recruit the annotators "which offer an easier way to recruit the annotators while offering a dirverse..." - task setup depends on your annot interface, etc.; also not sure about this "diverse" claim; there are very specific ppl on AMT; it's pretty much NOT direverse} and offer a diverse workforce, reducing the researcher's efforts. However, these systems have the same difficulties in teaching complicated linguistic tasks to crowd annotators. \mkcomment{what "systems", I don't think this is the best word choice}


% \textcolor{orange}{One of the solutions proposed in the literature is to incorporate the \textit{learning by progression} approach~\cite{kicikoglu2020aggregation, madge2019progression, miller2019expertise}, where the annotators start with simpler tasks and gradually move towards more complex problems. However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks.}

% % One of the proposed solutions, also investigated for GWAPs, is to use the notion of learning by progression~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, whereby the annotators start with simpler tasks, and then they are progressively taught more complex tasks. \mkcomment{One of the solutions proposed in the literature is to incorporate the \textit{learning by progression approach}, where the annotators start with simpler tasks and gradual move towards more complex problems.} 
% However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks. \mkcomment{However, in order to efficiently employ the \textit{learning by progression} approach, researchers have to identify which cases are .... }

% \mkcomment{this transition is a bit rough; you mention the need to identiry these easy vs difficult cases and then switch to another topic without saying that this is what we do... should finish that thing first, then switch to minimal guidelines as a way to coref}
\agcomment{WIP from here onwards}
Specifically, our work investigates the feasibility of crowdsourcing coreference annotations by providing \emph{minimal} guidelines to workers on the Amazon Mechanical Turk Platform (AMT). In contrast to more elaborate guidelines used in previous work, 
our minimal guidelines 
%cover the broad concept 
teach workers only the broad
concept
of coreference, focusing on basic phenomena that have similar treatment across existing guidelines,
such as pronouns. 
%pronouns in ``\textcolor{red}{{[}John{]}} doesn’t like 
%\textcolor{teal}{{[}Fred{]}}, but \textcolor{red}{{[}he{]}} still invited \textcolor{teal}{{[}him{]}} to \textcolor{violet}{{[}the party{]}}").

% \agcomment{added minimal guidelines definition}
% \micomment{need to loosely define minimal guidelines. have a sentence explaining what is covered by the guidelines here (at a high level with some specific examples in parenthetical).} 
% \textcolor{orange}{By observing agreements/disagreements among annotators under \emph{minimal} training, we aim to understand which coreference concepts are easy to annotate for crowd annotators and which concepts would require more explanations in the guidelines. Such an understanding would not only help effective crowdsourcing but also help to prioritize difficult concepts while curating annotation guidelines.} 
% We train our annotators using these \emph{minimal} guidelines in order to investigate which coreference concepts are easier to annotate for crowd annotators and which concepts require more explanations in the guidelines.
% \mkcomment{We...XYZ (teach, present, or sth) ... in order to investigate....(give justification for minimal guidelines)??? <--- maybe like this you can add it?}
% For instance, annotations for pronoun resolution which are very useful for information extraction tasks can be obtained via minimal training, as observed in our experiments. If we can obtain good annotations via minimal training, that can speed up the process and make it easier for other researchers to collect new datasets, thereby reducing both annotator and researcher efforts.
To facilitate collection of these annotations, we develop a methodology---\texttt{ezCoref}---which includes an intuitive, open-sourced annotation tool
% \footnote{Our platform's code and collected data is available in supplementary material, and will be released publicly after review.}
supported by a short crowd-oriented interactive tutorial that includes annotation guidelines.\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}" (\autoref{table:tutorial_feedback} in Appendix)} We use \texttt{ezCoref} to re-annotate 240 passages from seven existing English coreference datasets. Our results show that high-quality annotations (measured by agreement with expert annotations) are obtained from non-experts with the minimal training facilitated by our annotation platform (>90$\%$ B3~\cite{bagga-1998-algorithms} agreement with experts).
% \micomment{can you say something about the quality of annotations from ezcoref, like we get high agreement with expert-annotated datasets}
\mkcomment{make the contributions clearer}
Our annotation study uniquely allows us to identify where the behavior of our crowd annotators differs from that of experts. For example, we qualitatively observe that crowd workers mark all generic pronouns as coreferent, while existing guidelines treat them as non-referring, and we observe similar deviations from expert guidelines for appositives and copulae. Furthermore, annotators find it easier to annotate pronouns than other coreference types, and they exhibit higher agreement when annotating familiar texts (e.g., childhood stories or fiction) compared to texts rich in cataphoric expressions or those requiring world knowledge.
% \micomment{the following insights should be reordered by interestingness/impactfulness and condensed}
% We obtain a high agreement among annotators for the fiction domain, suggesting that this domain is suitable to collect crowdsourced coreference annotations. Comparing various linguistic concepts, we find that annotators struggle with cataphoras, resulting in multiple mistake when annotating QuizBowl dataset~\cite{guha-etal-2015-removing}. Finally, comparing the expert guidelines with crowd annotations, we find that appositives and copulae have been annotated similarly by existing guidelines, but annotators naturally mark them differently and would require clarification in guidelines if expected otherwise. 
% \mkcomment{<---this sentence is not the smoothest, the point of it is too far in the forest; Finally, we find that non-expert annotators tend to annotate metions in appositives and copulae as coreferent, even though most of existing guidelines connected these with another, special link. ....though that is not true either right... they don't tend to do that, they are all over the place with copula but maybe better with appos, then it's the question of major vote}
We conclude with a qualitative analysis and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and coreference platform development.





\begin{table*}[]
\centering 
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{lccccclcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Domains\\ $\#$(doc, ment, tok)\end{tabular}}} & \multirow{2}{*}{\textbf{Annotators}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{2}{c}{\textbf{Mention Types}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Coreference Links}} &  \\ \cline{5-6} \cline{8-11} \addlinespace[0.05cm]
 &  &  &  & \textbf{Singletons} & \textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}} & \multicolumn{1}{c}{} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} & \textbf{Ambiguity} \\\midrule
 
\textbf{\begin{tabular}[c]{@{}l@{}}ARRAU\\ \cite{Uryupina2019}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (552, 99K, 350K)\end{tabular}  & Single Expert & Manual & Yes & None &  & Special Link & No Link & Yes & Explicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}Phrase Detectives (PD)\\ \cite{chamberlain-etal-2016-phrase}\end{tabular}}& \begin{tabular}[c]{@{}c@{}}Multiple\\ (542, 100K, 400K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Crowd (gamified) +\\ 2 Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semi\\ Automatic\end{tabular} & Yes & None &  & Special Link & Special Link & Yes & Implicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}GUM\\\cite{zeldes-2017-gum}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (25, 6K, 20K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Experts \\ (Linguistics Students)\end{tabular} & Manual & Yes & None &  & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Types)  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Type)  \end{tabular} & Yes & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}PreCo \\ \cite{chen-etal-2018-preco}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple***\\ (38K, 3.58M, 12.5M)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Non-Expert, \\ Non-Native \end{tabular}& Manual** & Yes & None &  & Coref & Coref & Yes & None \\ \addlinespace[0.1cm]

\textbf{\begin{tabular}[c]{@{}l@{}}OntoNotes\\ \cite{hovy-etal-2006-ontonotes}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (1.6K, 94K, 950K)\end{tabular}  & Experts & Mixed & No & None &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}LitBank\\ \cite{bamman-etal-2020-annotated}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (100, 29K, 210K)\end{tabular}  & Experts & Manual & Yes & ACE (selected) &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}QuizBowl\\ \cite{guha-etal-2015-removing}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (400, 9.4K, 50K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Manual\\ \& CRF*\end{tabular} & Yes & \begin{tabular}[c]{@{}c@{}}Characters,\\ Books,\\  Authors*\end{tabular} &  & Coref & Coref & If Applicable & None \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}ezCoref Pilot Dataset 
\\ (this work)\end{tabular}} & Multiple & Crowd (paid) & \begin{tabular}[c]{@{}c@{}}Fully\\ Automatic\end{tabular} & Yes & None &  & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & Implicit \\ \bottomrule
\end{tabular}
\end{adjustbox}

\caption{Summary of seven datasets analyzed in this work,
which 
differ in domain, size, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. }\scriptsize{***See Footnote \ref{fn:preco}.}} 
\vspace{-0.1in}
\label{table:motivation}
\end{table*}


\ignore{
\subsubsection{bullet points}
Existing datasets differ widely in their guidelines, so we don’t know which one to employ for new data collection. 

These guidelines are often complex with many arbitrary decisions.

Complex guidelines require experts but collecting annots with experts is expensive and time consuming (small num of experts working on large num of docs)

Crowdsourcing is a non-expert alternative which was recently done by using GWAP - but that is also time consuming (development, PR); the annotators may be motivated (yay, it’s a game!) but they need simplified guidelines

Alternative is traditional crowdsourcing but just as GWAP it requires simplified guidelines - teach ppl what you want (ppl can resolve coref naturally, but need to explain them the task)

One of the proposed solutions applied also in GWAP is to use the notion of learning by progression = iterating through concepts from easy to difficult cases. But for it to be done well with minimum time from workers => it requires researchers to identify what is hard and what is easy for a better / more efficient design

In this work, we try to address this question. We collect annotations under minimal training to identify what is hard and easy for annotators. Furthermore, deviations from existing expert guidelines can help inform avenues to revisit.

\subsection{text}
\agcomment{WIP}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase, chen-2018-preco}. However, these datasets vary widely in their definition of coreference (expressed through annotation guidelines), resulting in inconsistent annotations both within and across languages and domains~\cite{universal-anaphora} (e.g., English news in Figure~\ref{figure:data_guidelines}). 

Coreference datasets vary in terms of their definition of coreference expressed via different guidelines, annotation formats and annotation platform used to collect the dataset. All these differences have impacts on the quality of collected data. These datasets not only differ in terms of what is coreference but also what is considered as a mention. Unfortunately, at the moment, there is only limited consensus on the various aspects of coreference phenomena that should be covered by any annotation guidelines~\cite{universal-anaphora}

In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.

Another complimentary dimension in which these datasets differ is how these datasets were collected. Traditionally, these datasets such as OntoNotes were collected via expert annotators trained in lengthy guidelines. More recently, impressive progress has been made towards crowdsourcing coreference annotations. Both payment based approaches and games-with-a-purpose has been proposed and impressive success has been achieved e.g., as demonstrated by the success of Phrase Detectives. However, GWAPs are often not open-sourced and require maintaining constant visibility to collect annotations, thereby significantly increasing researcher efforts to collect new datasets. 

In this work, we investigate whether it is feasible to crowdsource coreference resolution under minimal guidelines? For instance, annotations for pronoun resolution which are very useful for information extraction tasks can be obtained via minimal training, as observed in our experiments. If we can obtain good annotations via minimal training, that can speed up the process and make it easier for other researchers to collect new datasets.
}



% \agcomment{broad area of the paper, recent progress, key limitation}

% \agcomment{give an example of key limitation}

% \agcomment{why and where, addressing this challenge is useful. why addressing this challenge isn't trivial.}

% \agcomment{some existing efforts to address this issue, and one line limitation.}

% \agcomment{what do we do in this paper to address this issue.}

% \agcomment{our contributions}

==> EMNLP 2022/emnlp_sections/introductionv5.tex <==
\section{Introduction}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by datasets annotated by experts
% expert-annotated datasets \mkcomment{while it's better than "expertly" I would just go with the good old "datasets annotated by experts...}~
\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase}. However, these datasets vary widely in their definitions of coreference (expressed via annotation guidelines), 
% \mkcomment{definition of coref and annot guidlines is basically saying the same thing twice, also I think the basic definition of coref is the same, whats different is details, how universal anaphora complain about this? },
resulting in inconsistent annotations both within and across domains and languages. For instance, as shown in Figure~\ref{figure:data_guidelines}, while  ARRAU~\cite{Uryupina2019} treats generic pronouns as non-referring, OntoNotes chooses not to mark them at all.
% \mkcomment{the connection between these two sentences is not very smooth; maybe that middle sentence makes it less smooth the "common English news" part}
% (Figure~\ref{figure:data_guidelines}). 
% ~\cite{universal-anaphora}
%(e.g., English news in Figure~\ref{figure:data_guidelines}). 


\begin{figure}[t]
    \centering
  %\hspace{-3mm}
  \includegraphics[width=0.45\textwidth, scale=0.7,clip,trim=0 0 0 0mm]{figs/motivation_guidelines.pdf}
  \caption{A common sentence from news domain annotated by two expert-curated datasets: OntoNotes~\cite{hovy-etal-2006-ontonotes} and ARRAU~\cite{Uryupina2019}. We visualize the two expert annotations along with the crowd annotations obtained in our study using \ezcoref\ platform. 
  While OntoNotes does not mark generic pronouns and ARRAU marks them as non-referring mentions, our crowdworkers mark all mentions of generic pronoun ``you” as coreferent and similarly for ``we”.
%   While OntoNotes does not mark generic pronouns and ARRAU marks them as non-referring mentions, our crowdworkers mark all generic pronouns (e.g., ``you'' and ``we'') as coreferent.\micomment{this is a bit confusing, since it could be interpreted as ``you'' and ``we'' are coreferent in the example, which is obviously not true. i'd reword}
}
  \vspace{-0.1in}
\label{figure:data_guidelines}
\end{figure}

% \footnotetext{Entity annotations for most singletons omitted for visual clarity.}
% A common sentence drawn from two datasets, OntoNotes and ARRAU, with gold annotations as per their guidelines and re-annotated by our crowdworkers by using \ezcoref. While OntoNotes and ARRAU themselves differ in their definition of mentions and coreferences, crowdworkers with minimal guidelines have a completely different perception compared to these two datasets. OntoNotes does not mark generic pronouns, ARRAU marks generic pronouns as non-referring, however, crowdworkers naturally mark generic pronouns as coreferent.
It is thus unclear which guidelines one should employ when collecting coreference annotations in a new domain or language.
% When collecting a new coreference dataset, how should the annotation guidelines be chosen? \mkcomment{personal preferences, I don't find these questions very strong, would do sth like: Hence, it is unclear how... }
Traditionally, existing guidelines have leaned towards lengthy explanations of complex linguistic concepts, such as those in the OntoNotes guidelines~\citep{ontonotes-guidelines}, which detail what should and should not be coreferent (e.g., how to deal with head-sharing noun phrases, premodifiers, and generic mentions). 
As a result, coreference datasets have traditionally been annotated by linguists (experts) already familiar with such concepts, which makes the process expensive and time-consuming. Crowdsourced coreference data collection has the potential to be significantly cheaper and faster; however, teaching an exhaustive set of linguistic guidelines to non-expert crowd workers remains a formidable challenge. As a result, there has been a growing interest among researchers in curating a unified set of guidelines~\cite{universal-anaphora} suitable 
% \mkcomment{"suitable" is ok,but it's often used as in "suitable for children" etc., I find "accessible" (==easy to understand) or comprehensible better choices} 
for annotators with various backgrounds. 

More recently, games-with-a-purpose (GWAPs)~\cite{von-ahn-2006-gwap, poesio-etal-2013-PDoverview} were proposed to aid crowdsourcing of large coreference datasets~\cite{chamberlain-etal-2016-phrase-custom, yu-etal-PDv3-2022}.
% More recently, games-with-a-purpose (GWAPs)~\citep{von-ahn-2006-gwap}, such as Phrase Detectives~\citep{poesio-etal-2013-PDoverview} and LingoTowns\footnote{\url{https://lingotowns.com/}}, were proposed to crowdsource large coreference datasets~\cite{chamberlain-etal-2016-phrase, yu-etal-PDv3-2022}.
% \micomment{the citations and parentheticals in the prev sentence are hard to parse. simplify (possibly by moving some citations to related work?)}
% \mkcomment{important first? More recently, games-with-a-purpose (GWAPs) were proposed as...}
While GWAPs make it enjoyable for crowdworkers 
%\mkcomment{are these crowdworker?}\agcomment{yes, table 1}
to learn complex guidelines 
% \mkcomment{do they learn complex guidelines? rather are being presented with simple guidelines} \agcomment{i don't think we can really say whether the guidelines they use are simple, they are some combination of other guidelines, thus we used word complex}
and perform annotations using them~\cite{madge2019progression}, 
% \mkcomment{missing citations, should cite PD v3.0 and lingotowns}, \agcomment{added in previous sentence}
they also require significant effort to attract and maintain workers. For instance, Phrase Detectives Corpus 1.0 was collected over a span of six years~\cite{chamberlain-etal-2016-phrase-custom, poesio2013phrase, yu-etal-PDv3-2022},  
%\mkcomment{they report more in 3.0}), 
% \mkcomment{end sentence here? "In this work, we explore more efficient...}
% \micomment{again, this parenthetical is confusing and doesn't actually end. i'd recommend not using citations within parentheticals}
which motivates us to instead study coreference collection on more efficient payment-based platforms. 
% and are often not open-sourced, making them inaccessible to other researchers interested in collecting new datasets.


% , including payment-based microtasks and games-with-a-purpose (GWAPs)~\cite{von-ahn-2006-gwap, poesio-etal-2013-PDoverview},

% Even so, annotators may have to frequently refer to these guidelines, which results in significant annotator efforts (e.g., OntoNotes and ARRAU as shown in Figure~\ref{figure:motivation_efforts}).  

% In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.
%Because of the differences in the existing guidelines, it is difficult to know which guidelines to use when collecting datasets in a new domain or language. Furthermore, these guidelines frequently include lengthy explanations of 

% More recently, efforts have been made to crowdsource coreference annotations by utilizing non-experts to annotate large corpora~\cite{chen-2018-preco, chamberlain-etal-2016-phrase}. For instance, applying the games-with-a-purpose (GWAPs) approach~\cite{von-ahn-2006-gwap, poesio2017crowdsourcing, kicikoglu2020aggregation, madge-etal-2019-making}, which emphasizes on fun as a motivator for annotators, researchers have successfully curated coreference datasets~\cite{poesio2019crowdsourced, poesio2013phrase, chamberlain-etal-2016-phrase}. While GWAPs make it interesting and enjoyable \mkcomment{I think GWAP is a fixed term? "game-with-a-pupose" not gameS; you probably can use "GWAPs" is you really want to but I wouldn't use "games-with..."}\agcomment{great point! though, I think gameS-with-a-purpose is equally valid, for instance Poessio uses this term in \url{https://dl.acm.org/doi/pdf/10.1145/2448116.2448119}; section 2.4 and von Ahn, one of the pioneers who popularized this concept, also uses "games"} for non-expert annotators to annotate documents, these methods necessitate significant researcher efforts to build such games and keep them visible for data collection~\cite{poesio-etal-2013-PDoverview} (e.g., Phrase Detectives in Figure~2). Furthermore, even this approach %\mkcomment{this approach; it's not a system, i think} 
% is challenged by complex, lengthy guidelines, as non-expert annotators in crowdsourcing setups \mkcomment{in any setup really, and it's kind of crowdsourcing anyway in nlp when you use non-experts, this is redundant} require concise, easy-to-understand guidelines to perform well and remain engaged.

% Another alternative for crowdsourcing linguistic annotations, including coreferences, is to use traditional payment-based methods (e.g., Amazon Mechanical Turk)~\cite{snow-2008-cheap, cybulska-vossen-2014-using, roit-etal-2020-controlled, bornstein-2020-corefi}, which are much easier to setup the task \mkcomment{more like easier to recruit the annotators "which offer an easier way to recruit the annotators while offering a dirverse..." - task setup depends on your annot interface, etc.; also not sure about this "diverse" claim; there are very specific ppl on AMT; it's pretty much NOT direverse} and offer a diverse workforce, reducing the researcher's efforts. However, these systems have the same difficulties in teaching complicated linguistic tasks to crowd annotators. \mkcomment{what "systems", I don't think this is the best word choice}


% \textcolor{orange}{One of the solutions proposed in the literature is to incorporate the \textit{learning by progression} approach~\cite{kicikoglu2020aggregation, madge2019progression, miller2019expertise}, where the annotators start with simpler tasks and gradually move towards more complex problems. However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks.}

% % One of the proposed solutions, also investigated for GWAPs, is to use the notion of learning by progression~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, whereby the annotators start with simpler tasks, and then they are progressively taught more complex tasks. \mkcomment{One of the solutions proposed in the literature is to incorporate the \textit{learning by progression approach}, where the annotators start with simpler tasks and gradual move towards more complex problems.} 
% However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks. \mkcomment{However, in order to efficiently employ the \textit{learning by progression} approach, researchers have to identify which cases are .... }

% \mkcomment{this transition is a bit rough; you mention the need to identiry these easy vs difficult cases and then switch to another topic without saying that this is what we do... should finish that thing first, then switch to minimal guidelines as a way to coref}
%\agcomment{WIP from here onwards}

Specifically, our work investigates the quality of crowdsourced coreference annotations when annotators are taught only simple coreference cases that are treated uniformly across existing datasets (e.g., pronouns). By providing only these simple cases, we are able to teach the annotators the concept of coreference, while allowing them to freely interpret cases treated differently across the existing datasets. This setup allows us to identify cases where our annotators disagree among each other, but more importantly cases where they unanimously agree with each other but disagree with the expert, thus suggesting cases that should be revisited by the research community when curating future unified annotation guidelines. 

% Specifically, our work investigates the quality of crowdsourced coreference annotations with annotators being taught only simple coreference 
% % \mkcomment{"with annotators being taught only..."?}
% cases that are treated uniformly 
% % \mkcomment{"uniformly" similarly is not the same}
% across existing datasets (e.g., pronouns). These coreference cases teach workers the broad concept of coreference \mkcomment{"By doing so, we are able to teach the annotators the concept of coreference, while allowing them to freely interpret cases treated differently across the existing datasets. This lets us to identify cases where our annotators disagree among each other, and cases where they agree with each other but disagree with the expert sth..." <-- or sth like that} while allowing us to identify cases of disagreements among crowd and expert annotations, thus suggesting cases that should be revisited by the research community when curating future unified annotation guidelines. 

Our main contributions are:
\begin{enumerate}
    \item We develop a crowdsourcing-friendly coreference annotation methodology---\ezcoref--- 
    % \mkcomment{I'm not too married to calling that methodology, but i guess?}
    which includes an intuitive, open-sourced annotation tool
    supported by a short crowd-oriented interactive tutorial.\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}" (\autoref{table:tutorial_feedback} in Appendix)}
    \item We use \ezcoref to re-annotate 240 passages from seven existing English coreference datasets on Amazon Mechanical Turk (AMT), and conduct a comparative analysis of crowd and expert annotations. 
    %\mkcomment{--> separate point?not sure-->}
    We find that high-quality annotations are already achievable from non-experts without extensive training (>90$\%$ B3~\cite{bagga-1998-algorithms} agreement between crowd and expert annotations).
    % \mkcomment{maybe we can add sth like "We find that high-quality annotations are already achievable from non-experts without extensive training, as the majority of annotators... sth about resolving the more challenging cases like in guidelines? though I guess thats contradictory? I feel like this high agreement needs to be explained}
    \item We further qualitatively analyze remaining disagreements among crowd and expert annotations and identify linguistic cases that crowd unanimously marks as coreferent but
    % \mkcomment{"which" such a nice word} \agcomment{"We further qualitatively analyze remaining disagreements among crowd and expert annotations and identify linguistic cases that crowd unanimously marks as coreferent which lack unified treatment in existing datasets"....this seem not easily readable, we also loose the contrast.}
    lack unified treatment in existing datasets (e.g., generic pronouns as shown in~Figure~\ref{figure:data_guidelines}). 
    % \mkcomment{new item here? "Additioanlly, we analyze ... and ...}
    Additionally, analyzing inter-annotator agreement among the crowd reveals that crowd exhibits higher agreement when annotating familiar texts (e.g., childhood stories or fiction) compared to texts rich in cataphoras or those requiring world knowledge. 
    % \mkcomment{next point}
    Finally, our qualitative analysis also provides an empirical evidence to support previous findings in literary studies (\citeauthor{szakolczai2016novels}’s \citeyearpar{szakolczai2016novels} analysis of Bleak House) and psychology (\citeauthor{Orvell2020}’s \citeyearpar{Orvell2020} claims about generic “you”).
\end{enumerate}

% We conclude with a qualitative analysis and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and coreference platform development.

% Specifically, our work investigates the feasibility of crowdsourcing coreference annotations by providing \emph{minimal} guidelines to workers on the Amazon Mechanical Turk Platform (AMT). In contrast to more elaborate guidelines used in previous work, 
% our minimal guidelines 
% %cover the broad concept 
% teach workers only the broad
% concept
% of coreference, focusing on basic phenomena that have similar treatment across existing guidelines,
% such as pronouns. 


% To facilitate collection of these annotations, we develop a methodology---\texttt{ezCoref}---which includes an intuitive, open-sourced annotation tool
% % \footnote{Our platform's code and collected data is available in supplementary material, and will be released publicly after review.}
% supported by a short crowd-oriented interactive tutorial that includes annotation guidelines.\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}" (\autoref{table:tutorial_feedback} in Appendix)} We use \texttt{ezCoref} to re-annotate 240 passages from seven existing English coreference datasets. 

% Our results show that high-quality annotations (measured by agreement with expert annotations) are obtained from non-experts with the minimal training facilitated by our annotation platform (>90$\%$ B3~\cite{bagga-1998-algorithms} agreement with experts).
% % \micomment{can you say something about the quality of annotations from ezcoref, like we get high agreement with expert-annotated datasets}
% \mkcomment{make the contributions clearer}
% Our annotation study uniquely allows us to identify where the behavior of our crowd annotators differs from that of experts. For example, we qualitatively observe that crowd workers mark all generic pronouns as coreferent, while existing guidelines treat them as non-referring, and we observe similar deviations from expert guidelines for appositives and copulae. 

% Furthermore, annotators find it easier to annotate pronouns than other coreference types, and they exhibit higher agreement when annotating familiar texts (e.g., childhood stories or fiction) compared to texts rich in cataphoric expressions or those requiring world knowledge.
% We conclude with a qualitative analysis and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and coreference platform development.


\begin{table*}[]
\centering 
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{lccccclcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Domains\\ $\#$(doc, ment, tok)\end{tabular}}} & \multirow{2}{*}{\textbf{Annotators}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{2}{c}{\textbf{Mention Types}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Coreference Links}} &  \\ \cline{5-6} \cline{8-11} \addlinespace[0.05cm]
 &  &  &  & \textbf{Singletons} & \textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}} & \multicolumn{1}{c}{} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} & \textbf{Ambiguity} \\\midrule
 
\textbf{\begin{tabular}[c]{@{}l@{}}ARRAU\\ \cite{Uryupina2019}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (552, 99K, 350K)\end{tabular}  & Single Expert & Manual & Yes & None &  & Special Link & No Link & Yes & Explicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}Phrase Detectives (PD)\\ \cite{chamberlain-etal-2016-phrase}\end{tabular}}& \begin{tabular}[c]{@{}c@{}}Multiple\\ (542, 100K, 400K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Crowd (gamified) +\\ 2 Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semi\\ Automatic\end{tabular} & Yes & None &  & Special Link & Special Link & Yes & Implicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}GUM\\\cite{zeldes-2017-gum}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (25, 6K, 20K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Experts \\ (Linguistics Students)\end{tabular} & Manual & Yes & None &  & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Types)  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Type)  \end{tabular} & Yes & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}PreCo \\ \cite{chen-etal-2018-preco}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple***\\ (38K, 3.58M, 12.5M)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Non-Expert, \\ Non-Native \end{tabular}& Manual** & Yes & None &  & Coref & Coref & Yes & None \\ \addlinespace[0.1cm]

\textbf{\begin{tabular}[c]{@{}l@{}}OntoNotes\\ \cite{hovy-etal-2006-ontonotes}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (1.6K, 94K, 950K)\end{tabular}  & Experts & Mixed & No & None &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}LitBank\\ \cite{bamman-etal-2020-annotated}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (100, 29K, 210K)\end{tabular}  & Experts & Manual & Yes & ACE (selected) &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}QuizBowl\\ \cite{guha-etal-2015-removing}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (400, 9.4K, 50K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Manual\\ \& CRF*\end{tabular} & Yes & \begin{tabular}[c]{@{}c@{}}Characters,\\ Books,\\  Authors*\end{tabular} &  & Coref & Coref & If Applicable & None \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}ezCoref Pilot Dataset 
\\ (this work)\end{tabular}} & Multiple & Crowd (paid) & \begin{tabular}[c]{@{}c@{}}Fully\\ Automatic\end{tabular} & Yes & None &  & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & Implicit \\ \bottomrule
\end{tabular}
\end{adjustbox}

\caption{Summary of seven datasets analyzed in this work,
which 
differ in domain, size, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. }\scriptsize{***See Footnote \ref{fn:preco}.}} 
\vspace{-0.1in}
\label{table:motivation}
\end{table*}


\ignore{
\subsubsection{bullet points}
Existing datasets differ widely in their guidelines, so we don’t know which one to employ for new data collection. 

These guidelines are often complex with many arbitrary decisions.

Complex guidelines require experts but collecting annots with experts is expensive and time consuming (small num of experts working on large num of docs)

Crowdsourcing is a non-expert alternative which was recently done by using GWAP - but that is also time consuming (development, PR); the annotators may be motivated (yay, it’s a game!) but they need simplified guidelines

Alternative is traditional crowdsourcing but just as GWAP it requires simplified guidelines - teach ppl what you want (ppl can resolve coref naturally, but need to explain them the task)

One of the proposed solutions applied also in GWAP is to use the notion of learning by progression = iterating through concepts from easy to difficult cases. But for it to be done well with minimum time from workers => it requires researchers to identify what is hard and what is easy for a better / more efficient design

In this work, we try to address this question. We collect annotations under minimal training to identify what is hard and easy for annotators. Furthermore, deviations from existing expert guidelines can help inform avenues to revisit.

\subsection{text}
\agcomment{WIP}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase, chen-2018-preco}. However, these datasets vary widely in their definition of coreference (expressed through annotation guidelines), resulting in inconsistent annotations both within and across languages and domains~\cite{universal-anaphora} (e.g., English news in Figure~\ref{figure:data_guidelines}). 

Coreference datasets vary in terms of their definition of coreference expressed via different guidelines, annotation formats and annotation platform used to collect the dataset. All these differences have impacts on the quality of collected data. These datasets not only differ in terms of what is coreference but also what is considered as a mention. Unfortunately, at the moment, there is only limited consensus on the various aspects of coreference phenomena that should be covered by any annotation guidelines~\cite{universal-anaphora}

In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.

Another complimentary dimension in which these datasets differ is how these datasets were collected. Traditionally, these datasets such as OntoNotes were collected via expert annotators trained in lengthy guidelines. More recently, impressive progress has been made towards crowdsourcing coreference annotations. Both payment based approaches and games-with-a-purpose has been proposed and impressive success has been achieved e.g., as demonstrated by the success of Phrase Detectives. However, GWAPs are often not open-sourced and require maintaining constant visibility to collect annotations, thereby significantly increasing researcher efforts to collect new datasets. 

In this work, we investigate whether it is feasible to crowdsource coreference resolution under minimal guidelines? For instance, annotations for pronoun resolution which are very useful for information extraction tasks can be obtained via minimal training, as observed in our experiments. If we can obtain good annotations via minimal training, that can speed up the process and make it easier for other researchers to collect new datasets.
}



% \agcomment{broad area of the paper, recent progress, key limitation}

% \agcomment{give an example of key limitation}

% \agcomment{why and where, addressing this challenge is useful. why addressing this challenge isn't trivial.}

% \agcomment{some existing efforts to address this issue, and one line limitation.}

% \agcomment{what do we do in this paper to address this issue.}

% \agcomment{our contributions}

==> EMNLP 2022/emnlp_sections/limitations.tex <==
\section{Limitations}
\label{sec:limitations}
We list some of the limitations of our study which researchers and practitioners would hopefully benefit from when interpreting our analysis. Firstly, our analysis is only applicable to the English language and how native English speakers understand coreferences. In this work, we have taken a step towards building a framework to facilitate the comparison of the crowd and expert annotations, and the variations observed in non-native speakers should be explored in future studies. Secondly, as a result of resource constraints, we limited ourselves to one set of guidelines and compared crowd annotations under these guidelines with expert annotations. Understanding the effects of various guidelines on annotator behavior is left for future research. Thirdly, even the best automatic mention detection algorithm could have errors, especially when tested out-of-domain. Some of the proposed solutions are to directly crowdsource mentions or verify the automatically identified mentions via crowdsourcing~\cite{madge2019progression}, which can be utilized for future collection of high-quality corpora.

% \agcomment{to edit}
% limitations of crowd study regarding the guidelines and pre-labeling the dataset with an algorithm.

% automatic mention identification is not sufficient. PD group has crowdsourced pre-processing steps too. 

% A broad space of prior work on how to enable inexperts to accurately perform tasks traditionally performed by experts.

% instructions on emnlp website:
% This section will appear at the end of the paper, after the discussion/conclusions section and before the references, and will not count towards the page limit. 
% Mentioning that the method works mostly for languages with limited morphology, like English, is a much better alternative. In addition, limitations such as low scalability to long text, the requirement of large GPU resources, or other things that inspire crucial further investigation are welcome.


% Mention identification for annotation is typi- cally done semi-automatically, using first an auto- matic mention detector (or extractor) (Uryupina and Zanoli, 2016) and then checking its output by hand. Automatic mention detectors developed for coreference systems are generally used in the first step. Mention detection was recognized early on as a key step for overall coreference quality (Stoy- anov et al., 2009; Hacioglu et al., 2005; Zhekova and Ku ̈bler, 2010; Uryupina and Zanoli, 2016), so a number of good quality mention detectors were developed, such as the mention detector included in the Stanford CORE pipeline (Manning et al., 2014), used by many of the top-performing sys- tems in the 2012 CONLL Shared Task (Pradhan et al., 2012).1 But this performance can be im- proved. The first contribution of this paper are new fully-trainable, language-independent mention de- tectors that outperform the Stanford CORE men- tion detector in a variety of genres.~\cite{madge2019crowdsourcing}

% Even the current best mention detection algorithm can be prone to errors. Future work can explore crowdsourcing mentions or semi-automatically curating them.

==> EMNLP 2022/emnlp_sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}

% \mkcomment{About PD: the pointers appearing after the initial tutorials are misleading: wisdom of crowd works if it's independent (same about confirmation)? You could do validation without risking ppl agreeing because that's their natural behaviour.}
% \mkcomment{need few words of intro; ok, update, actually wrote sth, not good at writing this part though... }

% Our work builds on previous efforts to collect coreference data, especially those that rely on crowdsourcing. 


% \begin{table*}[h!]
% \tiny
% \begin{center}
% \begin{tabular}{ llrrrrrrrrrrr } 
%  \toprule
% System & Type & \begin{tabular}[c]{@{}l@{}}Mentions \\pre-selected\end{tabular} & \begin{tabular}[c]{@{}l@{}}Open\\Source\end{tabular} & Webapp & \begin{tabular}[c]{@{}l@{}}Coref\\only\end{tabular} & \begin{tabular}[c]{@{}l@{}}Keyboard\\+ Mouse\end{tabular} & \begin{tabular}[c]{@{}l@{}}MTurk\\Tested\end{tabular} & \begin{tabular}[c]{@{}l@{}}Simple\\Instructions\end{tabular} & \begin{tabular}[c]{@{}l@{}}Annotation\\Verification\end{tabular} & \begin{tabular}[c]{@{}l@{}}Span\\Nesting\end{tabular} & Tutorial & \begin{tabular}[c]{@{}l@{}}Doc Length\\Control\end{tabular} \\
% \midrule
% \citet{stenetorp-etal-2012-brat} & & \xmarkcol & \checkmarkcol & \checkmarkcol & \xmarkcol \\
% \citet{widlcher-2012-glozz} & \\
% \citet{landragin-etal-2012-analec} \\
% \citet{yimam-etal-2013-webanno} \\ \citet{girardi-etal-2014-cromer} \\ 
% \citet{kopec-2014-mmax2} \\
% \citet{oberle-2018-sacr} \\
% \citet{reiter-2018-corefannotator} \\
% \citet{bornstein-2020-corefi} \\
% QuizBowl \\
% PhraseDetective \\
% \midrule
% \ezcoref (this work) & Cluster & \checkmarkcol & \checkmarkcol  & \checkmarkcol & \checkmarkcol & \checkmarkcol & \checkmarkcol & \checkmarkcol & \checkmarkcol \\
% \bottomrule
% \end{tabular}
% \end{center}
% \caption{A comparison of different coreference annotation tools.}
% \label{tab:prior-work-compare}
% \end{table*}


% OntoNotes~\cite{hovy-etal-2006-ontonotes}, LitBank~\cite{bamman-etal-2020-annotated}, PreCo~\cite{chen-etal-2018-preco}, ARRAU~\cite{Uryupina2019}, GUM~\cite{zeldes-2017-gum}, Phrase Detectives~\cite{chamberlain-etal-2016-phrase}, and QuizBowl~\cite{guha-etal-2015-removing}

\paragraph{Existing coreference datasets:} 
\autoref{table:motivation} provides an overview of seven prominent coreference datasets, which differ widely in their annotator population, mention detection, and coreference guidelines.\footnote{Many others exist too; for example, see Jonathan Kummerfeld's \href{https://docs.google.com/spreadsheets/d/1DTuzCAOcqEzKqQNFcLVAx0KQb1DTUYVQbZV55LONXHI/edit\#gid=0}{spreadsheet list} (accessed Jan.\ 2022).} 
Many datasets are annotated by experts heavily trained in linguistic standards, including ARRAU~\cite{Uryupina2019}, LitBank~\cite{bamman-etal-2020-annotated},
GUM~\cite{zeldes-2017-gum}, and OntoNotes~\cite{hovy-etal-2006-ontonotes}). 
% which we define as annotators heavily trained in the project's linguistic standards for coreference, who typically give many hours of annotations on the same dataset. 
Due to its scale and quality, OntoNotes is likely the most widely used for NLP coreference research, including in two CoNLL shared tasks \cite{pradhan-etal-2011-conll,pradhan-etal-2012-conll}. Coreference datasets annotated by non-experts include
those created by part-time non-native English speakers (PreCo; \citet{chen-etal-2018-preco}),
domain but not linguistic experts (QuizBowl; \citet{guha-etal-2015-removing}), and gamified crowdsourcing without financial compensation (Phrase Detectives; \citet{chamberlain-etal-2016-phrase-custom}). 
% There is considerable variation within these datasets on what is a mention and a coreference (Table~\ref{table:motivation}).
%\micomment{need to cite all of these!} 

% Mention definition is a crucial step, where several datasets ask annotators
% to identify mention spans manually (LitBank, ARRAU, QuizBowl, and GUM);
% OntoNotes (ON) and Phrase Detectives (PD) make use of
% rule-based extraction from syntax trees.
% %(ON from gold standard parses; PD from automatic parses, plus manual verification).  
% QuizBowl and LitBank heavily restrict the types of entities that are annotated at all for coreference.
% Finally, different annotation choices are made for whether various constructions (e.g.\ predicative NPs) are considered coreferent. % such as predicative NPs,
% % As for the mention detection, LitBank, ARRAU, QuizBowl, and GUM~\cite{zeldes-2017-gum} ask annotators to identify the mentions manually, OntoNotes considers all noun phrases automatically extracted from its treebank data as mentions allowing for manual annotation of verbs and premodifiers,
% % Other mention types (premodifiers, verb phrases, etc.) in OntoNotes are curated manually. 
% % while Phrase Detectives (PD) adopts a semi-automatic approach by using Berkeley Parser~\cite{petrov-klein-2007-improved} to identify mentions followed by manual verification. Finally, datasets use different definitions of mentions and coreference: LitBank limits its mention sets to selected ACE-style-entities; QuizBowl annotates only authors, characters, and works; 
% % both Quizbowl and PreCo allow predicative NPs, GUM annotates predicative NPs as coreference but adds a sub-type, while other datasets do not allow for NPs in predicative structures to corefer.
% %and GUM \agcomment{PreCo, and QuizBowl} allows predicative NPs and link between generics. 
% We use a unique set of such decisions for \ezcoref---fully automatic mention detection, annotator intuition, and paid crowdsourcing.
%---justified in Section \ref{} \btocomment{todo}.

% In contrast to previous works, \ezcoref\ is the first crowdsourced effort to use purely automatic mention detection to collect coreference annotations, while not imposing any constraints on coreference types.

% \agcomment{A line/footnote about PreCo not available.} \mkcomment{it's in the introduction, you can move it here, I guess}
% \textbf{Mention Types}
% These datasets also annotate different kinds of mentions. \footnote{QuizBowl only allows other types of mentions when they are an answer to a question} OntoNotes while allowing unrestricted coreference, does not annotate singletons. PreCo, Phrase Detectives, ARRAU, and GUM, consider a wider variety of mentions, including all noun phrases, generics, and singletons. In addition, Phrase Detectives and ARRAU also mark expletives and split antecedents. While ARRAU allows all premodifiers (if referred to), PreCo limits them to common nouns and proper noun modifiers as mentions.

% \textbf{Coreference Links}


\paragraph{Coreference annotation tools:}

% \kkcomment{How about a table comparing the different annotation tools for coreference, using tick/crossmarks to compare strengths / weaknesses? Like table 1 here - https://aclanthology.org/D18-1241.pdf}

Several coreference annotation tools with similar features to \ezcoref\ have already been developed (See \autoref{tab:tools-prior-work-compare} in Appendix for more details). However, these are difficult to port to a crowdsourced workflow, as they require users to install software on their local machine~\cite{widlcher-2012-glozz, landragin-etal-2012-analec, kopec-2014-mmax2, reiter-2018-corefannotator}, or have complicated UI design with multiple drag and drop actions and/or multiple windows~\cite{stenetorp-etal-2012-brat-custom, widlcher-2012-glozz, landragin-etal-2012-analec, yimam-etal-2013-webanno, girardi-etal-2014-cromer, kopec-2014-mmax2, oberle-2018-sacr}. Closest to our work is \texttt{CoRefi}~\citep{bornstein-2020-corefi}, a web-based coreference annotation tool that can be embedded into crowdsourcing websites.  Subjectively, we found its user interface difficult to use (e.g., users have to memorize multiple key combinations). It also does not allow for nested spans, reducing its usability. 

\paragraph{Crowdsourcing coreference annotations:} 
Several efforts have been made to crowdsource linguistic annotations~\cite{snow-2008-cheap, callison-burch-2009-fast, howe2008crowdsourcing, lawson-etal-2010-annotating}, including on payment-based microtasks via platforms like AMT and GWAPs~\cite{von-ahn-2006-gwap}. Many GWAPs~\cite{poesio-etal-2013-phrase, kicikoglu2019wormingo, madge-et-al-2019-wordclicker, fort-et-al-2014-zombilingo} have been used in NLP to collect linguistic annotations including coreferences; with some broader platforms~\cite{venhuizen-etal-2013-gamification, madge2019progression} aiming to gamify the entire text annotation pipeline. One solution to teaching crowd workers complex guidelines is to incorporate \textit{learning by progression}~\cite{kicikoglu2020aggregation, madge2019progression, miller2019expertise}, where annotators start with simpler tasks and gradually move towards more complex problems, but this requires subjective judgments of task difficulty. In contrast to the payment-based microtask setting studied in this work, GWAPs are not open-sourced, need significant development, take longer to collect data, and require continuous efforts to maintain visibility~\cite{poesio-etal-2013-phrase}.
% , requiring significant work from a researcher interested in using existing tools to collect new data.

% In this work, we use payment-based microtasking, which minimizes researcher efforts and is also shown to be more effective than GWAPs when collecting small to medium-scale annotations for analysis (the focus of this work) rather than large-scale resource creation~\cite{madge2019crowdsourcing}.

% \textcolor{cadmiumgreen}{Teaching crowdworkers complex  guidelines has remained challenging while crowdsourcing linguistic annotations. One of the solutions proposed in the literature is to incorporate the \textit{learning by progression}~\cite{kicikoglu2020aggregation, madge2019progression, miller2019expertise}, where the annotators start with simpler tasks and gradually move towards more complex problems. However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks. In this work, we provide minimal training to our crowd workers, which allows us to observe annotator agreements/disagreements and identify easy and complex coreference concepts. We hope our observations will help reduce annotator efforts and facilitate more effective crowdsourcing.} 


% However, GWAPs entail significant efforts on the part of researchers, as they are generally not open-sourced, require significant development efforts, take much longer to collect data~\cite{madge2019crowdsourcing}, and require continuous efforts to maintain visibility~\cite{poesio-etal-2013-phrase}. 

% \agcomment{added new}
% More recently, several efforts have been made to crowdsource linguistic annotations~\cite{snow-2008-cheap, callison-burch-2009-fast, howe2008crowdsourcing, lawson-etal-2010-annotating}, obtaining expert-level quality at a fraction of cost required for expert annotations by employing sufficiently large number of workers. Crowdsourcing takes many forms, including citizen science (e.g., Wikipedia), payment-based microworking via platforms like Amazon Mechanical Turk and games-with-a-purpose (GWAP)~\cite{von-ahn-2006-gwap}. GWAPs such as Phrase Detectives~\cite{poesio-etal-2013-phrase}, Wormingo~\cite{kicikoglu2019wormingo}, WordClicker~\cite{madge-et-al-2019-wordclicker} and Zombie Lingo~\cite{fort-et-al-2014-zombilingo} have been used in NLP to collect annotations on several linguistic features including coreferences; broader platforms such as Wordrobe~\cite{venhuizen-etal-2013-gamification} and TitleAttack~\cite{madge2019progression} to gamify the entire text annotation pipeline. GWAPs, however, entail significant efforts on the part of researchers, as they are generally not open-sourced, require significant development efforts, and finally, mandate continuous efforts to maintain visibility~\cite{poesio-etal-2013-phrase}. GWAPs also take much longer to collect data; for instance, ~\citet{madge2019crowdsourcing} collected data via AMT using gamified HITs for speedy data collection in order to validate their GWAP for markable identification. Furthermore, while GWAPs promise data collection with very low costs, payments in the form of prizes are still required to attract annotators and require frequent adjustment to prize mechanisms to ensure maximum effectiveness~\cite{poesio-etal-2013-phrase}. In this work, we instead use a traditional payment-based microworking approach to not only minimize researcher efforts but also because our main objective is not to collect a large corpus but to test whether crowdsourcing is feasible under minimal guidelines. As also advocated by ~\citet{madge2019crowdsourcing}, AMT based approach is best suited to collect small to medium-scale annotations where the objective is data analysis rather than large resource creation.

% -among crowdsourcing approaches, two approaches are prominent. a) payment based b)game based \\
% - game based methods \\

% he most notable development is the attempt to defray the high cost of annotated resource development through crowdsourcing using Amazon Mechanical Turk4 and similar systems, and the so-called “games-with-a-purpose”, as described in Poesio et al.

% which suggests that the GWAP approach can defi- nitely be used to annotate at least medium-size (1M–10M words), high-quality corpora, provided, however, that a number of issues are paid attention to and that a continuous effort is made to maintain the game visible.


% These difficulties in interpretation suggest the need to collect multiple judgments for each expression—a task very well suited for Web collaboration of any type—and that in cases of disagreement it may be best to preserve such judgments rather than attempting to make a choice between them.

% In order to attract the number of participants required to make a suc- cess of the GWAP methodology it is not enough to develop attractive games; successful and continuous advertising is also required. Activities to raise the profile of Phrase Detectives were started from the very beginning, attempting to attract the attention not only of the computational linguistics community, but also of other scientists, and of the general public.


% A revolution in the way language annotation tasks are carried out was achieved by crowdsourcing (Howe, 2008; Snow et al., 2008). Crowdsourcing comes in many forms, including citizen science and microworking. A third approach is to use a game-with-a-purpose (GWAP) to aggregate data from non-expert players for collective decisions similar to those from an expert (von Ahn, 2006). The game-based approach to collecting language data is initially costly, but once a game is deployed it can continue to collect data with very little finan- cial support, especially if there is an active com- munity. GWAPs such as Phrase Detectives (Poesio et al., 2013), JeuxDesMots (Joubert and Lafour- cade, 2008) and Zombie Lingo (Fort et al., 2014) have been used in NLP to collect data on specific linguistic features; broader platforms such as Wor- drobe (Venhuizen et al., 2013) to gamify the entire text annotation pipeline




% \btocomment{I removed speed comparison. If we want to make it, report and compare in Sec 5 where you talk about speed, and forward reference from here.}\kkcomment{perhaps we can add here stuff from table 2, like no nested span support / expert terminology in Corefi?} \mkcomment{expert terminology was here and seems like it was deleted; added nested spans}
% In our experiments \ezcoref\ annotators worked faster than reported in \citeauthor{bornstein-2020-corefi} (approx.\ 600 vs.\ 400 tokens per hour), though datasets and other experimental details differ.

% However, the platform has a steep learning curve in the particulars of its user interface requiring the annotators to memorize multiple key combinations and learn from feedback, which quickly disappears. \agcomment{re-write: However, the platform has a steep learning curve with multiple key combinations to memorize and feedback, which quickly disappears, increasing overall annotator efforts. As a result, teaching crowd workers how to use this tool is challenging.} Furthermore, the default instructions use technical terms such as ``entity,'' ``mention,'' or ``cluster bank,'' which may be confusing for crowd annotators.\micomment{these critiques seem weak.} 
% These factors presumably contribute to the slow reported annotation speed of up to 400 mentions per hour, compared to 600 mentions per hour with \ezcoref.
% \agcomment{Our speed = 600 mentions per hour. Avg time per passage=4.15 min, average mentions per passage=42, approx 40 minutes for 400 mentions. Can say 1.5 times faster than \texttt{CoRefi}}

% \footnote{\texttt{CoRefi} also provided manual feedback (in addition to a tutorial) to their annotators for their mistakes, consuming 30-40 minutes of researcher time per trained annotator. Our annotators receive the instructions/feedback only via the tutorial, and there is no interaction with researchers.} 


% \mkcomment{I think i understand that the intrustion quickly dissapear but not sure if this is clear}
% \agcomment{your rewrite is great as there are lot of instructions shown in the beginning which the user cannot remember. But additionally, when doing the task the instructions/feedback appear and then disappear before a user can read them and understand what to do.}

% Furthermore, \citet{yimam-etal-2013-webanno} allows only documents of certain length, considerably restricting the type of collected data.

% \mkcomment{the last one is not really a good claim for crowdsourcing, do we have anything else on them? Also now I overly simplified it with "hard to use" = no mannual OR drag and drop OR multiple windows; maybe will rewrite later. Is the "no manual claim ok? do we have manual?}
% \agcomment{~\citet{yimam-etal-2013-webanno} has a manual, it is web-based tool to annotate multiple semantic tasks, including coref, requires drag and drop to create relations between two spans}
% \mkcomment{I'm not talking about yimam. You wrote " A few tools lack a setup manual~\cite{girardi-etal-2014-cromer}" and I'm just wondering whether we have a manual ^^" I guess we can make one, lol}



% Several existing tools for coreference annotations are often not well-suited for crowdsourcing environments, either requiring slow and complex drag and drop actions~\cite{stenetorp-etal-2012-brat, widlcher-2012-glozz, oberle-2018-sacr} or consists of multiple windows and menus~\cite{kopec-2014-mmax2}, or works only well for texts of a certain length becoming unresponsive for book-long texts~\cite{yimam-etal-2013-webanno}. Some tools are stand-alone applications requiring local downloads and installations~\cite{widlcher-2012-glozz, landragin-etal-2012-analec, kopec-2014-mmax2, reiter-2018-corefannotator}. 

% A few tools lack a setup manual~\cite{girardi-etal-2014-cromer} or have one that is only accessible in a particular language~\cite{landragin-etal-2012-analec}. Furthermore, some tools require annotators to fill in a generic template (a human-friendly name for the entity, comments, description, etc.) for each newly identified entity, slowing down the annotation process~\cite{landragin-etal-2012-analec, kopec-2014-mmax2}. 

% \agcomment{I have put in many arguments against corefi, feel free to pick and choose most reasonable ones}

% Few tools for coreference annotations have been designed with crowdsourcing in mind. \cite{bornstein-2020-corefi} developed a web-based coreference annotation tool embeddable into crowdsourcing websites. However, the platform requires annotators to use multiple keyboard shortcuts for different functionalities, which initially can be hard to remember. 
% No navigation signals are provided, and instructions quickly disappear, not allowing enough time for the annotator to understand the desired actions. 
% Visually, more emphasis is given to the currently user-selected entity than the current mention being annotated, which may confuse some annotators. 
% In the training phase, the concept of coreferences is explained using some advanced NLP concepts (e.g., named entities, head words, etc.), which may be unfamiliar to annotators in a crowdsourcing setup. Furthermore, the reported annotation speed is ~400 mentions per hour, much slower than EZCoref. 

% \mkcomment{asked some questions about this, need ans before edit confidently but will try to add it }
% \citet{aralikatte-sogaard-2020-model} also proposed a model-based annotation tool suitable for crowdsourcing that automatically identifies entities and requires annotators to assign pronouns to these entities. However, they leverage the unique structure of Wikipedia, parsing URL links present in the document for entity identification, which may not be available for other domains and languages, posing a limitation for type of entities that can be annotated using this tool. 


% \mkcomment{long story short, need to rethink everything below in this section (I.e., dataset in related work), also GAWP - everything below in this section is an unedited WIP; maybe divide intro crowdsourced (PD, QB) and linguistic experts?}

% \mkcomment{I think we may want to have crowdsourcing approach and then experts, pretty much as it is but this means NO PD or QB in the "existing datasets", they should rater go here. So (1) software - there are some for experts, but not good for the crowd; the limited ones for crowd have their problems; (2) datasets by experts - many different guidelines/design choices, (3) crowd annot - QB - limited to quiz, not really your usualy crowd but game experts, limited entities annotated; PD - gamifying approach hard to develop and advertise; need to rethink this}


% \agcomment{This section will be re-written based on our data analysis in experiments sections. For now, I mentioned some basic aspects about the seven datasets we analyzed.}
% A plethora of datasets have been developed for the task of Coreference Resolution through the years. With the CoNLL shared tasks~\cite{pradhan-etal-2011-conll, pradhan-2012-conll}, OntoNotes has become the dominant resource for anaphora resolution research, predominantly used as the benchmark dataset in all state-of-the-art implementations~\cite{fernandes-etal-2014-latent, bjorkelund-kuhn-2014-learning, martschat-strube-2015-latent, clark-manning-2015-entity, clark-manning-2016-deep, clark-manning-2016-improving, lee-etal-2017-end, lee-etal-2018-higher}. OntoNotes consists of Arabic, Chinese and English documents from several domains but predominantly news. One frequently discussed limitation of OntoNotes is the absence of singletons ~\cite{Marneffe2015ModelingTL, chen-2018-preco}, requiring separate models to identify non-singletons mentions a pre-processing step~\cite{poesio-etal-2018-anaphora}. 

% A number of smaller corpora provide linguistically richer information. In ARRAU~\cite{poesio-etal-2018-anaphora}, for example, singletons are annotated and split antecedent plurals, generic coreference, discourse deixis, and bridging references. Furthermore, the ARRAU corpus was single annotated by a highly experienced annotator, who was allowed to mark various cases of ambiguities. 

% The recently introduced PreCo\footnote{At the time of writing the PreCo dataset is not available from the source provided by the authors. We also tried to contact the authors directly, but received no response.} corpus~\cite{chen-2018-preco} is the largest existing coreference corpus, consisting of 35,000 documents for a total of 12.5M tokens and 3.8M mentions, half of which are singletons. However, only the 3000 most common English words appear in the documents (the majority of the documents are from Chinese high-school English tests). In general, the corpus follows the OntoNotes guidelines, with a few important differences: singleton mentions and generic coreference are annotated, event anaphoras are not, and predicative NPs are annotated as co-referring with their argument. However, this dataset is not avaialabel on the link provided in the paper. 

% \citet{poesio-etal-2019-crowdsourced, chamberlain-etal-2016-phrase} collect crowdsourced coreference annotations through a game-with-a-purpose approach~\cite{poesio-etal-2013-phrase}. The corpus has a rich annotation scheme, covering singletons, expletives, and split-antecedent plurals. The corpus also comes with individual crowdsourced labels, allowing study of disagreements on anaphoric interpretation. Furthermore, the corpus also consists of aggregated labels inferred using probabilistic modeling. 

% \citet{bamman-etal-2020-annotated} collected coreference annotations for different literary novels, annotated for coreference relations between the ACE categories of people, locations, organizations, facilities, geopolitical entities, and vehicles~\cite{walker2006ace}. The annotation style largely follows that of OntoNotes, with some differences. They allow marking singletons, quantified, and negated noun phrases. They do not mark honorifics separately.  

% ~\citet{zeldes-2017-gum} collected a class-sourced corpus for coreference annotations where 21 students enrolled in a class were asked to annotate a single text of their choice throughout the course. These students had linguistic backgrounds and were provided with simplified OntoNotes like instructions in addition to original OntoNotes guidelines. In the GUM corpus, singletons and generic mentions are included. They also allow predicative NPs, appositives, expletives, and split antecedents. Furthermore, GUM distinguishes between anaphora and cataphora. 

% \agcomment{Need to add quizbowl}

% \textbf{Other Crowdsourcing Approaches for Coreference Resolution} \citet{poesio-etal-2013-phrase} uses a \textit{Game-With-A-Purpose}(GWAP) method for collecting coreference annotations, using "fun" as a significant motivator. Consequently, the Phrase detectives game produces the required dataset as a byproduct of the users' playing. However, the challenges with such an approach are developing such a game and maintaining high visibility for it. Achieving visibility and maintaining it requires constant effort and may incur additional expenditures. Furthermore, such a platform is not easy to set up by other researchers in the community. An alternative approach based on active learning has also been employed for pairwise coreference annotations~\cite{zhao-ng-2014-domain, li-etal-2020-active-learning, ravenscroft-etal-2021-cd}. However, pairwise annotations is often time-consuming and expensive, requiring labeling each pair of spans in the document.

% \section{Old Related Work}

% \agcomment{Putting arguments for each paper. Still need to make a coherent picture out these.}
% \textbf{Existing Annotation Software}

% \mkcomment{What we need here, I think, is: (1) there are some tools (CITE) (2) however they have this problem (CITE), or this problem (CITE) [if anything good then acknowledge. I wouldn't talk about mention detection here unless it's necessary (it's part of the tool and will restrict markables)}


% \citet{aralikatte-sogaard-2020-model} proposed a model-based annotation tool that automatically identifies entities and requires annotators to assign pronouns to these entities. However, they leverage the unique structure of Wikipedia, parsing URL links present in the document for entity identification, which may not be available for other domains and languages, posing a challenge for high recall entity identification. 

% %identify mentions of entities based on wiki, ask annot to assign pronouns


% Cromer~\cite{girardi-etal-2014-cromer}, CorefAnnotator~\cite{reiter-2018-corefannotator}, and SACR~\cite{oberle-2018-sacr} require annotators to identify mention spans themselves and then cluster mentions that refer to the same entity, thereby complicating the overall task without facilitating mention detection during preprocessing. Methods like this are prone to missing some mentions by annotators. Furthermore, the interface relies upon somewhat slow operations, such as drag-and-drop or selection from a drop-down list to cluster mentions. 

% \textbf{CoRefi} \cite{bornstein-2020-corefi} The platform requires annotators to use multiple keyboard shortcuts for different functionalities, which can be hard to remember initially. In the training phase, the concept of coreferences is explained using some advanced NLP concepts (e.g., named entities, head words, etc.), which may be unfamiliar to annotators in a crowdsourcing setup. Additionally, for practitioners to use the platform, they must upload extracted mentions as input in addition to the text.  Furthermore, the reported annotation speed is ~400 mentions per hour, much slower than EZCoref. 

% \textbf{Phrase Detectives}
% Several approaches have been proposed to crowdsourcing ever-larger annotated corpora for coreference resolution. \citet{poesio-etal-2013-phrase} uses a \textit{Game-With-A-Purpose }(GWAP) method, which uses "fun" as a significant motivator. Consequently, the Phrase detectives game produces the required dataset as a byproduct of the users' playing. However, the challenges with such an approach are developing such a game and maintaining high visibility for it. Achieving visibility and maintaining it requires constant effort and may incur additional expenditures. Furthermore, such a platform is not easy to set up by other researchers in the community. 

% \textbf{Active Learning/Pairwise}
% An alternative approach based on active learning has also been employed for pairwise coreference annotations~\cite{zhao-ng-2014-domain, li-etal-2020-active-learning, ravenscroft-etal-2021-cd}. However, the issue with pairwise annotations is that labeling each pair of spans in the document is expensive and infeasible.

% \textbf{Pair-Wise approach}
% \cite{hladka-etal-2009-play} requires annotators to identify if a mention pair corefer. \cite{chamberlain-etal-2016-phrase} requires annotators to identify a mention in the text that co-refer with the highlighted mention. 

% \textbf{Existing Datasets}

% \mkcomment{I know it looks overwhelming, but let's not overthink this, can add table to show key differences, or use the motivating example, or both, should be 2 short paragraphs (unless we somehow happen to have more space)}


% Related Work
%     1. Existing datasets (ACE, Onto, LitBank, PD, ARRAU)
%         Zombie dataset: PreCo
%     %2. existing disagreement studies
%     3. existing softwares/crowdsourcing approaches

==> EMNLP 2022/emnlp_sections/software.tex <==
\section{\ezcoref: A Crowdsourced Coreference Annotation Platform}
\label{sec:software}


% \mkcomment{the rewrite starts below, I think we should mention what we improve on but need to say it, even if mentioned in related work}
% \btocomment{bad to be so repetitive with intro. i'm trying to reformulate to be specific.}
% We develop \ezcoref, a coreference annotation software, designed to address the cost and scalability issues in coreference annotation.
The \ezcoref user experience consists of (1) a step-by-step interactive tutorial %which familiarizes the annotators with the interface and annotation guidelines, as well as 
and (2) an annotation interface, which are part of a pipeline including automatic mention detection and AMT Integration.

% By open-sourcing \ezcoref, we hope to facilitate the creation of large-scale coreference datasets for multiple domains and languages, reducing the time required to collect annotations while maintaining good quality. 


% \subsection{Design Choices}

\paragraph{Annotation structure:}
Two annotation approaches are prominent in the literature: (1) a local pairwise approach, 
annotators are shown a pair of mentions and asked whether they refer to the same entity \cite{hladka-etal-2009-play, chamberlain-etal-2016-phrase, li-etal-2020-active-learning, ravenscroft-etal-2021-cd}, which is time-consuming;
or (2) a cluster-based approach~\cite{reiter-2018-corefannotator, oberle-2018-sacr, bornstein-2020-corefi}, in which annotators group all mentions of the same entity into a single cluster. In \ezcoref\ we use the latter approach, which can be faster but requires the UI to support more complex actions for creating and editing cluster structures.
\begin{figure}[t]
    \centering
  %\hspace{-3mm}
  \includegraphics[width=0.48\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/Interface.pdf}
  \caption{Part of the \ezcoref interface (\S\ref{sec:software})}
  %\vspace{-0.1in}
  \label{figure:interface}
\end{figure}
\paragraph{User interface:}
%\mkcomment{add figure - screenshot main, partially annotated}
We spent two years iteratively designing, implementing, and user testing the interface to make it as simple and crowdsourcing-friendly as possible (\autoref{figure:interface}).\footnote{The interface is implemented in \href{https://reactjs.org/}{ReactJS}.}
Marked mentions are surrounded by color-coded frames with entity IDs. %, which also facilitates the understanding of nested mentions. 
The currently selected mention (``the book"),
is highlighted with a flashing yellow cursor-like box.
The core annotation action is to select other mentions that corefer with the current mention, and then advance to a later unassigned mention; annotators can also re-assign a previously annotated mention to another cluster.  
Advanced users can exclusively use keyboard shortcuts,
undo and redo actions were added to allow error correction.
Finally, \ezcoref provides a side panel showing mentions of the entity currently being annotated to spot mentions assigned to the wrong cluster.

%\footnote{The annotators can, at any time, re-assign a previously annotated mention to another cluster. The undo and redo buttons were added to reduce annotator efforts when correcting errors.} 

\paragraph{Coreference tutorial:}
To teach crowdworkers the basic definition of coreference and familiarize them with the interface, we develop a tutorial (aimed to take $\sim 20$ minutes) that familiarizes them with the mechanics of the annotation tool, and then trains them in a minimal set of annotation guidelines (\autoref{table:tutorial_example}). Our minimal guidelines cover cases that are annotated similarly across most guidelines and are unlikely to be disputed.
% Since most existing datasets have been annotated using extensive guidelines, our setup naturally lends us an ablation study comparing annotations with minimal guidelines versus without minimal guidelines.
% ...\agcomment{justify what we use is the minimal, why we don't need several minimal guidelines or any sort of ablation.}
%\micomment{put a table/list of the phenomena covered in this tutorial}\agcomment{Added Table~\ref{table:tutorial_example}} 
% It is aimed to take approximately 20 minutes.
% Throughout the tutorial, the annotators are encouraged to mark all mentions referring to one entity before moving to the subsequent entity. 
The tutorial concludes with a quality control example to exclude poor quality annotators.\footnote{Examples of the tutorial interface and the quality control example are provided in Appendix.} Training examples, feedback, and annotation guidelines can be easily customized using a simple JSON schema. 

% ~\ref{sec:tutorial_appendix}
\paragraph{Annotation workflow:}
The annotators are presented with one passage (or ``document'') at a time
(\autoref{figure:interface}), and all mentions have to be annotated before proceeding to the next passage. There is no limitation to the length or language of the passage.
% as long as the mentions have been automatically identified beforehand.  %% BTO: this clause is really rough. auto mentions is the next paragraph.
In this work, we divide an initial document into a sequence of shorter passages of complete sentences, on average 175 tokens, as shorter passages minimize the need to scroll, reducing annotator effort.  
While this obviously cannot capture longer distance coreference,\footnote{We leave this for future work---for example, more sophisticated user interfaces to support longer documents, or merging coreference chains between short passages. As documents get progressively longer, such as book chapters or books, the task takes on aspects of cross-document coreference and entity linking\ (e.g.\ \citealp{bagga-baldwin-1998-entity-based,fitzgerald-etal-2021-moleman, logan-iv-etal-2021-benchmarking}).}
a large portion of important coreference phenomena is local:
within the OntoNotes written genres, for pronominal mentions,
the closest antecedent is contained within the current or previous two sentences more than 95\% of the time.
% is a reasonable limitation is re
% We calculated that \btocomment{todo me - bound stuff i've shown yall}

% which could be handled in future work with a step to merge coreference chains between passages and 
%\micomment{but in practice there is. should mention exactly how long the documents we use are, and the tradeoffs of long vs short docs}  
% The interface also supports loading partially or fully annotated documents, allowing to review or continue the annotations.

\begin{table}[]
\centering \tiny
\begin{tabular}{ll}
\toprule
\textbf{Example} &
  \textbf{Phenomena Taught} \\ \hline
\begin{tabular}[c]{@{}l@{}}\textcolor{red}{{[}John{]}} doesn’t like \textcolor{teal}{{[}Fred{]}}, but \textcolor{red}{{[}he{]}} still \\ invited \textcolor{teal}{{[}him{]}}to \textcolor{violet}{{[}the party{]}}.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}} (1) personal pronouns\\ (2) singletons\end{tabular} \\
  \addlinespace[0.2cm]
  
\begin{tabular}[c]{@{}l@{}}\textcolor{teal}{{[}This dog{]}} likes to play \textcolor{blue}{{[}catch{]}}.\textcolor{teal}{{[}It{]}}’s \\ better than other \textcolor{magenta}{{[}dogs{]}} at \textcolor{blue}{{[}this game{]}}. \\ \textcolor{red}{{[}\textcolor{teal}{{[}Its{]}} owner{]}} is really proud.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}}(1) possessive pronouns\\ (2) semantically similar expression \\ which are not coreferring \\ (3) non-person entities (animals) \end{tabular} \\ \addlinespace[0.2cm]
  
\begin{tabular}[c]{@{}l@{}}\textcolor{teal}{{[}Director \textcolor{magenta}{{[}Mackenzie{]}}{]}} spent \textcolor{red}{{[}last two years{]}}\\  working on a \textcolor{blue}{{[}“Young Adam”{]}}. During \\ \textcolor{red}{{[}this time{]}} \textcolor{teal}{{[}he{]}} often had to make \textcolor{violet}{{[}compromises{]}}\\ but \textcolor{blue}{{[}the movie{]}} turned out to exceed expectations.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}} (1) nested spans \\ (2) non-person entities (time, item) \end{tabular} \\ \addlinespace[0.2cm]
  
\begin{tabular}[c]{@{}l@{}}\textcolor{teal}{{[}The office{]}} wasn’t exactly small either.\\ \textcolor{red}{{[}I{]}}’m sure that 50, or maybe even 60,  \textcolor{violet}{{[}people{]}}\\ could easily fit \textcolor{teal}{{[}there{]}}.\end{tabular} &
  \begin{tabular}[c]{@{}l@{}} (1) non-person entities (place) \end{tabular} \\ \bottomrule
\end{tabular}
\caption{Minimal guidelines explained by our tutorial.}
%\vspace{-0.1in}
\label{table:tutorial_example}
\end{table}

\paragraph{Automatic mention detection:}
\label{sec:mention_detection}
As a first step to collect coreference annotations, we must identify mentions in the documents from each of the seven existing datasets; this process is done in a diverse array of ways (from manually to automatic) in prior work as shown in \autoref{table:motivation}. We decided to automatically identify mentions to give all crowdworkers an identical set of mentions, which simplifies the annotation task and also allows us to easily compare and study their coreference annotations via inter-annotator agreement.
% As a byproduct, it also simplifies the annotation task for crowdworkers, as they are not forced to mark mention boundaries in the text, a task known to be much more challenging~\cite{madge2019crowdsourcing}. This approach considerably reduces the annotator's effort while speeding annotation; however, it relies heavily on the performance of the mention detection algorithm, which also can detect non-referring expressions (e.g., ``hand'' in ``on the other hand'').} 
% We leave an investigation of annotator behavior when identifying mentions for future work.
% Future work investigating annotator behavior for mention identification can utilize crowdsourcing to verify the automatically identified mentions~\cite{madge2019crowdsourcing}.} 
% As a first step to collect crowdsourced annotations, we must identify mentions in documents from each of the seven existing datasets. \autoref{table:motivation} shows that existing datasets use many methods and criteria to identify mentions, from completely manual to semi-automatic and fully automatic procedures, making it unclear which one to choose. Furthermore, gold mentions provided with existing datasets cannot be directly used to compare the inter annotator agreement of crowd annotations across different domains. Thus, instead of choosing an existing standard, we implement a simple automatic mention detection algorithm that yields a high average recall over all seven of these datasets.
% To simplify the annotation task for crowdworkers, we decide to automatically annotate mentions instead of forcing workers to mark mention boundaries in the text. This approach considerably reduces the annotator's effort while speeding annotation; however, it relies heavily on the performance of the mention detection algorithm, which also can detect non-referring expressions (e.g., ``hand'' in ``on the other hand'').
% \micomment{what is the prev sentence trying to say?} \mkcomment{seems like is was reworded: automatic mention detection can speed up things, but mention quality heavily relies on the quality of the mention detection algorithm, one thing that is happening is that (and it's in our data) non-refering expressions (such that can never refer to anything, not just singletons) as being marked} %\micomment{mention some downsides of automatic mention detection also} 
% Since mention detection is separate from the annotation pipeline (i.e., any mention detection algorithm can be employed), researchers can use \ezcoref\ to collect data for different languages and domains provided a good mention detector exists. 
% \autoref{table:motivation} shows that existing datasets use many methods and criteria to identify mentions, from completely manual to semi-automatic and fully automatic procedures.
% Furthermore, they also use very different criteria to identify these mentions (e.g., LitBank and QuizBowl impose entity restrictions, OntoNotes does not allow for singletons, ARRAU allows all premodifiers to be mentions, while PreCo restricts them to noun premodifiers),
%\micomment{give some examples of these criteria in a parenthetical} 
% which makes it unclear which one to choose. 
Specifically, we implement a simple algorithm that yields a high average recall over all seven datasets.\footnote{Note that any mention detection algorithm can be used as long as its recall across all datasets is high, and ours is only one such algorithm. However, we don’t collect and compare crowd annotations for mentions obtained from these potential algorithms as it would be prohibitively expensive. Furthermore, while advanced mention detection methods can definitely improve annotation quality, our goal is not to collect highest quality coreference dataset, but to study annotator behaviour when provided a common set of mentions.}
% \agcomment{why we implemented our own? Since existing datasets differ in their mention detection criteria, gold annotations cannot be directly compared against each other in terms of agreement. We use this automatic mention detection algorithm so that we can eliminate a source of variability i.e., "what constitutes as a mention" and focus on agreement over "what constitutes as coreference link between given set of mentions". Reducing annotator burden is not the main objective here.}
% \agcomment{to answer: we don't crowdsource mentions as done by some of the previous work and we don't need experiments with different mention detection algorithm}
% As a first step to collect crowdsourced annotations, we must identify mentions in documents from each dataset. Existing datasets use very different methods to identify such mentions, ranging from manual, semi-automatic, to fully automatic procedures. Furthermore, they also use very different criteria to identify these mentions. As a result, mentions provided with these datasets cannot be directly used to compare the inter annotator agreement of crowd annotations across different domains.

It considers all noun phrases (including proper nouns, common nouns, and pronouns) as markables, extracting them using the Stanza dependency parser (version 1.3.0; ~\citet{qi2020stanza}). We allow for nested mentions and proper noun premodifiers (e.g.,  \textcolor{red}{\textbf{[}}U.S.\textcolor{red}{\textbf{]}}  in ``U.S. policy''). We also include all conjuncts with the entire coordinated noun phrase (\textcolor{red}{\textbf{[}}Mark\textcolor{red}{\textbf{]}}, \textcolor{red}{\textbf{[}}Mary\textcolor{red}{\textbf{]}}, as well as \textcolor{red}{\textbf{[}}Mark and Mary\textcolor{red}{\textbf{]}}, are all considered mentions);  see Appendix~\ref{sec:md_algo} for more details.
% Finally, we allow for nested mentions, such as \textcolor{red}{\textbf{[}}\textcolor{teal}{\textbf{[}}his\textcolor{teal}{\textbf{]}} home\textcolor{red}{\textbf{]}}.
%\mkcomment{Ankita, can you check if this makes sense?}

% \agcomment{we need to say why we designed this custom algorithm, why not use any existing methods to identify mentions. In the last section we say that any mention detection algo can be used and in this section we say how our custom algo finds mentions, but we didn't say why this particular algo is needed.} \jmcomment{Maybe this paper is helpful?: "A Typology of Near-Identity Relations for Coreference (NIDENT)" I remember looking at it when working on this and designing around allowing for near/non-identity mentions.}
% We pre-identify the mentions using our customized mention detection algorithm. 

% As markables, we consider noun phrases including proper nouns, common nouns, and pronouns. \mkcomment{need to discuss why we include non-referring expressions, and also relatives}
% % \agcomment{need to discuss over call}
% We focus on high recall with regard to the existing datasets, as the mentions in these datasets were identified or validated by experts. Thus, any missed mentions could potentially impact the quality of annotated chains. On the other hand, spurious mentions can be marked as singletons, having little to no impact on the identified chains.

%Utilizing syntax, we implement following simple yet broad-coverage heuristics to detect mentions. 

% We detect the mentions using the following steps:

% \agcomment{I think this was one of major design choices we had, and should be included somewhere in short, ``We also encourage the annotators to mark all the spans that refer to the same entity before moving to the subsequent entity." }
% \mkcomment{Yeah, that would go to the tutorial, we don't enforce this during the actual annotation task}

% \agcomment{we also need to say that the interface can be pre-loaded with annotations, thereby supporting reviewing annotations.}
% \mkcomment{yeah, added}




% Aiming to address the cost and scalability issues in coreference annotation, we present EzCoref. This tool can be easily integrated into any crowdsourcing platform to support an end-to-end crowdsourcing process while providing several contributions over earlier annotation tools. \mkcomment{what contributions? it's a bit vague, I think}\agcomment{I thought, the previous section is related work, where we can say our contributions compared to existing tools. So, i thought, it will be clear from the context, but can remove this clause altogether. } EzCoref includes an automated training phase, familiarizing annotators with the tool functionality and the guidelines for the annotation task.\mkcomment{huh, made a comment and it's gone, must have been the net, anyway th} Following that, actual annotation is performed through a simple and efficient interface that supports mouse and keyboard operations. By open-sourcing EzCoref, we hope to facilitate the creation of large-scale coreference datasets, especially for the different domains, at a modest cost while maintaining annotation quality.

% EzCoref supports both the annotator training and annotation collection phases, as illustrated in Figure x. The training phase (Section y) consists of broadly two types of tasks. Firstly, annotators are guided through a step-by-step interactive tutorial to teach the tool's functionality. The second task is to practice guided annotation, interactively learning the basics of the annotation guidelines \mkcomment{annotation guidelines can be different, we hardly give any, can this be customized to support different approaches?}.\agcomment{can add something like this ``The examples presented in the guided annotation task and the automated feedback are easily configurable using a simple JSON configuration schema. EzCoref can be customized for different datasets and annotation guidelines by utilizing this feature."} Finally, a quality control example can be used to evaluate the annotators at the end of the training phase. After the training phase, EzCoref provides the annotation collection phase, where a user-friendly interface (Section z) can be used to collect coreference annotations. \agcomment{comment to myself....write about....The task provider can upload any documents to be annotated with pre-processed mentions. No restriction on the length of document. Pre-processed mentions are required.}
% \mkcomment{I want to rewrite the above, will post it below, @ankita: asked you some questions above, will rewrite once get answers, feel free to change the rewrite etc.}

% We develop \ezcoref, a coreference annotation software, designed to address the cost and scalability issues in coreference annotation. \ezcoref can be easily integrated with any crowdsourcing platform to support an end-to-end crowdsourcing process. \ezcoref includes a tutorial which   

% \subsection{Design Choices}

% \textbf{Annotation Approach}
% Two different annotation approaches are prominent in the prior work: the local pairwise approach and the cluster-based approach. In the local pairwise approach, the annotators decide whether a pair of mentions refer to the same entity or not.  However, this approach is often expensive and time-consuming, as it might require comparing a mention to all other mentions in the text. The cluster-based approach, which we follow in this paper, involves annotators annotating all mentions of the same entity together into one single cluster. In this approach, a mention needs to be compared only against the entities marked so far.  In EzCoref, we follow this approach as it allows us to conduct an exhaustive coreference annotation. 

% \textbf{User Interface}
% A key component of EzCoref is annotation visualization. A better visualization of marked mentions helps to reduced the cognitive load. Marked mentions are surrounded by colored frames and a unique numerical identifier, allowing an easy and quick view of the annotator's progress. This visualization also aids in understanding several levels of nested mentions.

% Another aspect of EzCoref is the visualization of the mention, which is being currently annotated. The current mention is highlighted in a specific colored frame (yellow), reserved for the current mention only, along with a flashing box around it. This feature allows the annotator to concentrate on the current mention and recognize all other mentions related to it. We also encourage the annotators to mark all the spans that refer to the same entity before moving to the subsequent entity. 

% Keeping track of all the entities encountered so far in a text is difficult yet necessary to link other co-referential mentions. To support this requirement, EzCoref provides a side panel which lists all the entities encountered so far and all the mentions assigned to these entities. Using this feature, annotators can see already annotated mentions and decide whether or not to attach the mention they are currently working on to a previously defined entity. This list may also be utilize to check if a mention has not been assigned to the wrong entity.

% \textbf{Others Points}

% \agcomment{these things needs to be integrated with rest of description}

% 1. EzCoref also supports the undo and redo functionality that speeds up the annotation process by reducing annotator effort while correcting errors. 

% 2. The platform requires all mentions to be marked before moving on to the subsequent passage. We allow task submission only once all candidate
% mentions are processed. 

% 3. The platform also contains a link to a document that explains each step during the training phase for annotators to review. 

% 4. At any point, the annotator can re-assign a previously assigned mention to another cluster.

% 5. To simplify annotation, the tool
% allows only non-overlapping spans.


% \subsection{Mention Detection}
% We delegate mention detection to a preprocessing stage, providing annotators with predetermined mentions. It simplifies the task and allows annotators to focus on the coreference decisions. Thus, in addition to the input document, EzCoref takes as input pre-identified mentions. We present a mention detection algorithm that detects noun phrases as mentions including proper nouns, common nouns and pronouns.

% EZCoref, however, is not constrained by our mention detection algorithm. The researchers may also opt to implement their own automated mention detection algorithm or use a separate manual annotation tool for mention annotation, according to their desired mention detection guidelines (which often vary across projects). The resulting mentions can then be fed into EzCoref for coreference annotations. 

% We focus on high recall than precision for the mention detection because, for any existing corpora, mentions have been identified or validated by experts. Thus, any missed mentions are guaranteed to impact the final coreference chains identified in the text. On the other hand, spurious mentions may not impact the identified chains since they can be assigned to singleton clusters.

% Utilizing syntax, we implement following simple yet broad-coverage heuristics to detect mentions. 
% \begin{enumerate}
%     \item We start by identifying all noun phrases. We use dependency relations\footnote{stanza software} to identify which words should be merged to construct a valid noun phrase. For each word with a noun-related POS tag (including pronouns, nouns, proper nouns, and numbers), we recursively traverse all its children in the dependency graph until the dependency relation is present in a whitelist. We allow all multi-word expression relations (compound, flat,  fixed) and modifier relations (determiners, adjectival modifier, numeric modifier, nominal modifier, and possessive nominal modifier) in the whitelist. The maximal span, which covers all words related by relations in the whitelist, is considered as candidate mention.
%     \item Possessive nominal modifiers of nouns are also considered candidate mentions. For example, in the sentence, "Mary's book is on the table," "Mary" is also considered as a mention in addition to the noun phrase "Mary's book." 
%     \item Modifier words that are proper nouns in a multi-word expression are considered as mentions. For example, in "U.S. foreign policy," "U.S." is also considered as a mention. 
%     \item All conjuncts, including the headword and the other words depending on it via the conjunct relation, are considered mentions in a coordinated noun phrase. For example, in the sentence, "John, Bob, and Mary went to the party.", the detected mentions are "John," "Bob," "Mary," and the noun phrase "John, Bob, and Mary."
%     \item We remove a mention if a larger mention with the same headword exists. We also merge any overlapping spans into one large span.
% \end{enumerate}

% \subsubsection{Tutorial}

% - steps

% - choice of examples

% - quality control


% \subsubsection{Main Task}

% Interface/Software Details

%     1.design choices (UI)
    
%     2. Mention Detection Algorithm 
    
%     3.choice of examples
    
%     4.quality control strategy 
    
%     5.release of data



==> emnlp_sections/abstract_v1.tex <==
\begin{abstract}
%\agcomment{WIP} 
Large-scale high-quality corpora are critical for advancing research in coreference resolution. However, existing datasets vary widely in their definition of coreference (expressed through annotation guidelines), making it unclear which guidelines to employ when collecting a corpus in a new language or domain. Furthermore, because these guidelines contain lengthy explanations of complex linguistic phenomena, they are best suited for expert annotators (e.g., linguists) rather than untrained crowd workers. In this work, we investigate whether it is feasible to crowdsource coreference annotations by providing \emph{minimal} guidelines to non-expert annotators, thereby reducing time and effort on the part of both annotators and researchers. We develop a crowdsourced coreference annotation platform called \ezcoref\ and use it to re-annotate 240 passages from seven existing English coreference datasets. 
We find annotators agree (>90$\%$ B3) with expert annotations (e.g., those in OntoNotes) even without extensive training, signifying that high-quality data can be obtained via crowdsourcing with minimalistic guidelines. Additionally, we observe deviations between crowd annotators and existing guidelines on linguistic phenomena such as general pronouns, appositives, and copulae, which can help inform guideline creation for future coreference annotation efforts.

% \mkcomment{I think the focus is off in the abstract -- basically seems like we braging that we got good annots with no guidelines, so 'easy things are easy' -- my least fav review, ugh!}

% [Shortened version of the above] Large-scale high-quality corpora are critical for advancing research in coreference resolution. However, existing datasets vary widely in their definitions of coreference, expressed through annotation guidelines. Furthermore, these guidelines contain lengthy explanations of complex linguistic phenomena and are most suited for expert annotators (e.g. linguists). In this work, we propose to crowdsource coreference annotations by providing \emph{minimal} guidelines to non-expert annotators, therefore reducing time and effort on the part of both annotators and researchers. We develop a crowdsourced coreference annotation platform called \ezcoref\ and use it to annotate 240 passages from seven existing English coreference datasets. We find that without extensive training, crowd workers provide annotations that mostly agree with expert annotations (e.g., those in OntoNotes). This signifies that high-quality data can be obtained via crowdsourcing with minimal guidelines. Additionally, we analyze deviations between crowd annotators on linguistic phenomena such as cataphora, appositives, and copulae, to inform guideline creation for future coreference annotation in new languages and domains.

% In particular, we observe a high agreement among annotators in the fiction domain and that annotating cataphora is challenging for crowd annotators. We also find that appositives and copulae have been treated similarly by existing guidelines, but non-expert annotators naturally mark them differently and would require clarification in guidelines if expected otherwise. 

% This paper is the first to compare the quality of crowdsourced coreference annotations against those of experts, and to identify where their behavior differs to facilitate future annotation efforts.

% To address these challenges,
% we develop and release \ezcoref, an easy-to-use coreference annotation tool and annotation methodology
% that facilitates crowdsourced data collection across multiple domains, currently in English.

% Instead of teaching crowdworkers how to handle non-trivial cases (e.g., near-identity coreferences), \ezcoref\ provides only a minimal set of guidelines sufficient for understanding the basics of the task. To validate this decision, we deploy \ezcoref on Mechanical Turk to re-annotate 240 passages from seven existing English coreference datasets across seven domains, achieving an average rate of 2530 tokens per hour, for one annotator. 

\ignore{Large-scale high-quality corpora are critical for advancing research in coreference resolution. 
Coreference annotation is typically time-consuming and expensive, since
researchers generally hire expert annotators %(e.g., trained linguists) 
and train them
with an extensive set of guidelines.
% This process is expensive and time-consuming, which motivates cheaper and quicker 
Crowdsourcing is a promising alternative,
but coreference includes complex semantic phenomena 
difficult to explain to untrained crowdworkers,
and the clustering structure is difficult to manipulate in a user interface. \agcomment{mentioning clustering structure here is too detailed}
% With the advent of deep learning, a large annotated corpus is crucial for advancing the development of coreference systems. %However, coreference annotations have traditionally been arduous and time-consuming, with a small number of trained linguists providing extensive annotations. 
% One way to quickly collect a large-scale coreference corpus is to use crowdsourcing (CITE) but this approach requires an intuitive annotation tool and simplified guidelines. 
% In this paper, we propose a new, more human-friendly paradigm to collect crowdsourced coreference annotations. 
To address these challenges,
we develop and release \ezcoref, an easy-to-use coreference annotation tool and annotation methodology
that facilitates crowdsourced data collection across multiple domains, currently in English.
% \ezcoref\ can facilitate the annotation process across multiple domains and languages\kkcomment{did we do expts on other languages? Not sure if we should say this if no expts} \mkcomment{no, we didn't but I think it's a strong aspect of the tool and can't see how it would break at least for languages that use the same alphabet, or am i missing sth?\micomment{since we didn't do an exps, we shouldnt mention this in the abstract. maybe in future work} }, 
%% BTO: auto detection assumes English, so our current software could NOT be applied to nonEnglish.
%and received positive feedback from the crowd workers. \mkcomment{well, actually that was about the tutorial, but it's probably ok} \agcomment{we collected feedback for  main task as well, though not many annotators responded. The small number of feedback was positive/neutral.}
% \mkcomment{yeah, I hope we will be able to get more from the survey}
Instead of teaching crowdworkers how to handle non-trivial cases (e.g., near-identity coreferences), \ezcoref\ provides only a minimal set of guidelines sufficient for understanding the basics of the task. To validate this decision, we deploy \ezcoref on Mechanical Turk to re-annotate 240 passages from seven existing English coreference datasets across seven domains, achieving an average rate of 2530 tokens per hour, for one annotator. \agcomment{why is this rate important to mention here?}
%
\agcomment{the following line is the main crux of the paper}\textbf{This paper is the first to compare the quality of crowdsourced coreference annotations against those of experts, and to identify where their behavior differs to facilitate future annotation efforts.}
We show that it is possible to collect coreference annotations of a reasonable quality in a fraction of time it would traditionally require.
%We provide the crowd workers with minimal annotation guidelines and identify what they intuitively mark as coreference. We utilize this data and provide suggestions for future annotation efforts.  


%Further, we study the differences in annotations for each dataset and compare them against crowdsourced annotations. This paper is the first to gather and categorize these inconsistencies and provide suggestions for future annotation efforts and evaluation decisions. Despite increased attention on crowdsourcing annotations for coreference resolution, there are still many open problems, which we highlight in this paper.


%ORIGINAL:
% With the advent of deep learning, large annotated corpora are crucial for advancing the development of models for coreference resolution. The need to collect large-scale corpora with reduced costs \mkcomment{time?} and efforts has motivated interest in developing annotation platforms to collect crowdsourced annotations for this task. However, there is still a need for an easy-to-use and intuitive platform which can facilitate the annotation process across multiple domains and languages. In this paper, we present an easy-to-use and intuitive annotation platform to collect coreference annotations. Using this platform, we collect crowdsourced annotations for seven existing datasets, covering a range of genres and annotation procedures. We examine the challenges while collecting annotations using crowdsourcing.
% Further, we study the differences in annotations for each dataset and compare them against crowdsourced annotations. This paper is the first to gather and categorize these inconsistencies and provide suggestions for future annotation efforts and evaluation decisions. Despite increased attention on crowdsourcing annotations for coreference resolution, there are still many open problems, which we highlight in this paper.
}


\end{abstract}

==> emnlp_sections/introductionv1.tex <==
% \section{Introduction Skeleton}
% \label{sec:intro}

% \begin{itemize}
%     \item Training coreference systems require lots of data. Several expert annotated and crowdsourced datasets have been collected to this end.

%   \item However, these datasets use different guidelines and annotation standards, making it hard to translate progress in one domain/language to other domains/languages~\cite{universal-anaphora}. Even within the same language and domain (e.g., English fiction), these datasets adopt very different annotation schema and guidelines. \mkcomment{just a comment, but its not like we solve this problem}

%   \item In order to collect data for any new domain/language, one faces an evident challenge, what guidelines and annotation standards to choose from among the existing ones or how to combine them together? \mkcomment{again, here too, we don't solve this problem either; not saying to get rid of it, just pay attention when writing? (how you phrase it)}
  

%   \item it is very expensive to iterate over guidelines/ annotation schema for a new domain, especially since many existing guidelines are extensive (e.g. ontonotes manual is X pages). 
  
%   \item Gamified approaches try to address this problem by XX which is good, but suffers from ... 
  
%   \item In this paper, we examine how well non-expert crowd workers agree with existing guidelines given only minimal training. 

% Our main contributions are:

% \item To collect these annotations, we propose a methodology, including an annotation tool supported with an interactive tutorial which focuses on step-by-step learning via progression, allowing us to teach annotators the broad phenomena of coreference.

% \item We collect annotations for documents from 7 different existing datasets, allowing us to examine the details of conference phenomena as perceived by human annotators without extensive training. 

% \item Using these collected annotations, we investigate several interesting questions such as: 
% \begin{enumerate}
%     \item  Which domains are most suitable for crowdsourcing coreferences? We find that fiction domain is easy.
%     or for which domains where can we expect good quality/good agreement/reasonable annotations?
    
%     \item which types of coref is difficult to annotate in crowdsourcing setups? we find annotators struggle with cataphora.
    
%     \item To what extent do crowd annotators agree with expert annotators? We find annotators agree with expert annotations even without extensive training, signifying that high quality data can be obtained via crowdsourcing with minimalistic guidelines. 
%     \mkcomment{this sounds nice, but not sure (don't remember the numbers) where it's not too strong? }
    
%     \agcomment{i re-read results section today. I think we can say this, perhaps hedge it a bit.}
%     \mkcomment{awesome}
    
%     \item On which linguistic phenomena do annotators agree with experts? We find that appositives and copulae have been annotated similarly by existing guidelines, but annotators naturally mark them differently. We provide qualitative analysis of such cases and highlight cases with genuine ambiguity.
% \end{enumerate}
    
% \item We hope our observations can inform future annotation efforts and guidelines construction.

% \end{itemize}

\section{Introduction}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity
in a given document. Coreference systems are an integral component of the preprocessing pipeline for many downstream tasks, such as summarization~\cite{azzam-etal-1999-using, steinberger-etal-2007-two}, question answering \cite{ vicedo-ferrandez-2000-importance, dhingra-etal-2018-neural}, and machine translation~\cite{hardmeier-2012-discourse, bawden-etal-2018-evaluating}. 

State-of-the-art coreference systems~\citep[e.g., ][]{
% lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert} are trained on large expert-annotated datasets such as OntoNotes~\citep{weischedel-etal-2013-ontonotes}. Collection of such datasets have traditionally involved linguists trained in lengthy guidelines~\citep[e.g.,][]{ontonotes-guidelines} that explain in detail what should and should not be considered coreference (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). 

While many datasets have been curated, these existing coreference datasets vary widely in their annotation guidelines, resulting in inconsistent annotations across languages and domains
% , with challenging cross-lingual and cross-domain issues
~\cite{universal-anaphora}, and even sometimes within the same language and domain (e.g., English news in Figure~\ref{figure:data_guidelines}).


% and PreCo~\citep{chen-etal-2018-preco} .



\begin{table}[]
\centering
\tiny
\begin{tabular}{ll}
\hline
Dataset     & Example                                                                                                                                                                                                                                                                     \\ \hline \addlinespace[0.1cm]
OntoNotes   & \begin{tabular}[c]{@{}l@{}}Maybe we need a \color{teal}{[}CIA{]}\color{black}\;version of the Miranda warning : \\ You have the right to conceal your coup intentions, \\ because we may rat on you .\end{tabular}                                                                                 \\ \addlinespace[0.2cm]

ARRAU       & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the Miranda warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right to conceal \color{magenta}{[}your{]}\color{black}\; {[}coup{]}e16 intentions{]}eS{]}eS, \\ because {[}we{]}eS may rat on \color{red}{[}you{]}\color{black}\;.\end{tabular} \\ \addlinespace[0.2cm]

Crowd (this work) & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the {[}Miranda{]}eS warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right{]}eS to conceal \color{blue}{[}your{]}\color{black}\; coup intentions{]}eS, \\ because \color{brown}{[}we{]}\color{black}\; may rat on \color{blue}{[}you{]}\color{black}\;\end{tabular}    \\ \hline
\end{tabular}
\captionof{figure}{A sentence annotated according to different guidelines. \agcomment{WIP}}
\label{figure:data_guidelines}
\end{table}

% \agcomment{OntoNotes and ARRAU have such detailed guidelines, is coreference underspecified then?}
\agcomment{Crux of para: coref is hard to specify, thus collected by experts taught with lengthy guidelines. But these guidelines differ alot}
Coreference is a complex phenomenon that is difficult to specify to annotators. 
\mkcomment{Yet, all people on the planet do it every day in order to communicate... This doesn't make much sense as it is right now. I know what you want to say but for that I believe this has to be reworded. Also can it even be explained if ppl perceive it differently as it's not a binary IS/IS NOT problem?}
As such, collecting coreference datasets has traditionally involved linguists trained in lengthy guidelines~\citep[e.g.,][]{ontonotes-guidelines} that explain in detail what should and should not be considered coreference (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). Existing coreference datasets vary widely in their annotation guidelines, resulting in inconsistent annotations across languages and domains
% , with challenging cross-lingual and cross-domain issues
~\cite{universal-anaphora}, and even sometimes within the same language and domain (e.g., English news in Figure~\ref{figure:data_guidelines}).
\mkcomment{This sounds much better than before!!!! :)}
% , these datasets~\cite{ontonotes-guidelines, Uryupina2019} adopt very different annotation guidelines (Figure~\ref{figure:data_guidelines} and \autoref{table:motivation}). 
% \citep[e.g., ][]{hovy-etal-2006-ontonotes, poesio-artstein-2008-anaphoric, Uryupina2019}. Datasets such as OntoNotes explain in detail to their annotators what should and should not be considered coreference

% These lengthy guidelines contain complex instructions clarifying how to handle specific linguistic phenomena .

% \mkcomment{I don't think "expertly-collected" sounds good (expertly == skillfully https://www.merriam-webster.com/thesaurus/expertly). I offered a rewrite to this paragraph (connecting it with the following one) but cannot find this comment now. Was that deleted? Maybe sth like this: For instance, datasets, such as OntoNotes, collected by experts, explain what should and should not be considered coreference via legthy guidelines~\cite{ontonotes-guidelines} which contain complex instructions about lingustic paradigms (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). }

% Acquiring these datasets has traditionally been difficult, expensive, and time-consuming, requiring linguists trained in fine-grained annotation schemas \citep[e.g., ][]{hovy-etal-2006-ontonotes, poesio-artstein-2008-anaphoric, Uryupina2019}. For instance, expertly-collected datasets such as OntoNotes explain what should and should not be considered coreference via a lengthy set of guidelines~\cite{ontonotes-guidelines} 
% that covers many complex linguistic details (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). 
% \mkcomment{For instance, datasets, such as OntoNotes, collected by experts, explain in details what should and should not be considered coreference~\cite{ontonotes-guidelines}. The lengthy guidelines contain complex instructions clarifying how to handle specific linguistic phenomena (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). } 
% Furthermore, these datasets differ widely in their annotation guidelines, resulting in inconsistent annotations across languages and domains, with challenging cross-lingual and cross-domain issues \cite{universal-anaphora}.
% \mkcomment{These annotation guidelines vary greatly across datasets, resulting in inconsistent annotations across languages and domains, with challenging cross-lingual and cross-domain issues \cite{universal-anaphora}.}


% \mkcomment{These datasets differ widely in their annotation standards, resulting in inconsistent annotations across languages and domains}
% \mkcomment{"with challenging cross-lingual and cross-domain issues" this is too vague; the next sentence repeats kind of the first sentences. The flow of this paragraph now is: The guidelines are difference (in general)--> this leads to different annot across langs --> within lang still different }


% In order to collect data for any new domain or language, one faces an evident challenge: what guidelines and annotation standards to choose from among the existing ones or how to combine them together? 
\agcomment{Crux of para: coming up with guidelines for a new domain/language is not easy because of these differences in existing guidelines}
In order to collect data for new languages or domains, one has to decide which guidelines to employ.
% Since existing coreference datasets differ widely in terms of what is considered as a mention and what types of links should be annotated (\citet{universal-anaphora} and \autoref{table:motivation}), it is not straightforward to combine these guidelines.
This is not a straightforward task, as the differences in existing guidelines can be significant not only in terms of what can and cannot corefer, but also in what is even considered to be a mention. 
\mkcomment{The above just repeats what's in line 44.}
% (<<== writing again they differ widely in guidelines is a bit too much; btw my rewrite is also poor; I don't like both)} 
Furthermore, it is expensive and time-consuming to iterate over candidate guidelines, requiring expert understanding to resolve differences in choice of mentions and coreference links (e.g., whether mentions related via copulae verb should corefer or should they be treated as a separate special link, requiring expert knowledge of what are copulae and the implications of treating them as coreference versus a special link; \autoref{table:motivation}).

\mkcomment{half of this also repeats what was said before}


% inconsistencies.
\agcomment{reworded}
\micomment{what kind of inconsistencies? why do they require expert understanding?} 
%\mkcomment{this is also a bit awkward}
For instance,~\citet{uryupina2020annotating} iteratively refined their guidelines over approximately 10 years to maximize intercoder agreement when collecting the ARRAU dataset.
%spanning approximately 10 years 
% \mkcomment{here it's not clear what does this mean, this is about PD (crowdsourcing) and they did adjust their guidelines for the GWAP}\agcomment{reworded. Is this clearer?}


To reduce annotation costs, more recent efforts have moved towards crowdsourcing coreference datasets with non-expert workers~\cite{chamberlain-etal-2016-phrase, chen-2018-preco, kicikoglu2019wormingo, madge2019crowdsourcing},
% \mkcomment{Xu, Chamberlain is about correcting errors not corefs per say, though they discuss PD} 
which suffer even more from the lack of standardized guidelines compared to expert data collection.\micomment{suffer in what way?}
\agcomment{not only the choice of guidelines is important, moreover they have to be simple and easy to understand}
\mkcomment{To reduce annotation costs, more recent efforts have moved towards crowdsourcing coreference datasets with non-expert workers~\cite{chamberlain-etal-2016-phrase, chen-2018-preco, kicikoglu2019wormingo, madge2019crowdsourcing}. <--- end sentence here, and maybe write in next that the guidelines for experts are not applicable cause XYZ; need simplified guidelines but this is also hard cause the expert ones are so different to begin with -- just so to not repeat too much (not say again that they different widely)}
% \mkcomment{more than what?}
The crowd annotators are often working on many competing tasks in very short time, mandating concise and easy-to-comprehend guidelines. To address this challenge of  teaching complex linguistic concepts to crowd annotators,  \textit{game with a purpose} (GWAP) methods incorporating a notion of progression have been proposed~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, whereby the annotators start with simpler tasks, and then they are progressively taught more complex tasks. However, developing GWAPs and collecting annotations takes much longer and requires maintaining constant high visibility for it~\cite{poesio2013phrase}.  
\mkcomment{(e.g., it took over 10 years to ...} \micomment{this GWAP stuff is not integrated into the rest of the introduction. you need to break down the different types of crowdsourcing settings (not just GWAP) and then say that we're examining MTurk because you can obtain annotations on it much more rapidly with bigger worker population. and this para should be concise, so don't cite so much stuff and cut details}


\begin{table*}[]
\centering 
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{lccccclcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Domains\\ $\#$(doc, ment, tok)\end{tabular}}} & \multirow{2}{*}{\textbf{Annotators}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{2}{c}{\textbf{Mention Types}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Coreference Links}} &  \\ \cline{5-6} \cline{8-11} \addlinespace[0.05cm]
 &  &  &  & \textbf{Singletons} & \textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}} & \multicolumn{1}{c}{} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} & \textbf{Ambiguity} \\\midrule
 
\textbf{\begin{tabular}[c]{@{}l@{}}ARRAU\\ \cite{Uryupina2019}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (552, 99K, 350K)\end{tabular}  & Single Expert & Manual & Yes & None &  & Special Link & No Link & Yes & Explicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}Phrase Detectives (PD)\\ \cite{chamberlain-etal-2016-phrase}\end{tabular}}& \begin{tabular}[c]{@{}c@{}}Multiple\\ (542, 100K, 400K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Crowd (gamified) +\\ 2 Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semi\\ Automatic\end{tabular} & Yes & None &  & Special Link & Special Link & Yes & Implicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}GUM\\\cite{zeldes-2017-gum}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (25, 6K, 20K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Experts \\ (Linguistics Students)\end{tabular} & Manual & Yes & None &  & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Types)  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Type)  \end{tabular} & Yes & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}PreCo \\ \cite{chen-etal-2018-preco}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple***\\ (38K, 3.58M, 12.5M)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Non-Expert, \\ Non-Native \end{tabular}& Manual** & Yes & None &  & Coref & Coref & Yes & None \\ \addlinespace[0.1cm]

\textbf{\begin{tabular}[c]{@{}l@{}}OntoNotes\\ \cite{hovy-etal-2006-ontonotes}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (1.6K, 94K, 950K)\end{tabular}  & Experts & Mixed & No & None &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}LitBank\\ \cite{bamman-etal-2020-annotated}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (100, 29K, 210K)\end{tabular}  & Experts & Manual & Yes & ACE (selected) &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}QuizBowl\\ \cite{guha-etal-2015-removing}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (400, 9.4K, 50K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Manual\\ \& CRF*\end{tabular} & Yes & \begin{tabular}[c]{@{}c@{}}Characters,\\ Books,\\  Authors*\end{tabular} &  & Coref & Coref & If Applicable & None \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}ezCoref Pilot Dataset 
\\ (this work)\end{tabular}} & Multiple & Crowd (paid) & \begin{tabular}[c]{@{}c@{}}Fully\\ Automatic\end{tabular} & Yes & None &  & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & Implicit \\ \bottomrule
\end{tabular}
\end{adjustbox}

\caption{Summary of seven datasets analyzed in this work,
which 
differ in domain, size, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. }\scriptsize{***See Footnote \ref{fn:preco}.}} 

% \agcomment{ezCoref is not a dataset, should not call last row as ezCoref}\btocomment{changed. i think `ours' sounds bad.}
\label{table:motivation}
\end{table*}

% This work aims at identifying the default behavior of crowd annotators, presented only with minimal guidelines explaining the broad phenomena of coreference. For instance, we explore what are the linguistic phenomena where annotators have disagreements and hence require clarification in the annotation guidelines. What are the cases where annotators most often agree unanimously and should be included in guidelines only if downstream applications expect otherwise? Finally, which cases entail high agreement among annotators but have been resolved differently in existing guidelines? To answer the above questions, we re-annotate a subset of documents from seven different English coreference datasets, encompassing a diverse mix of domains and different set of guidelines. 

In this paper, we examine how well non-expert annotators agree with existing guidelines given only minimal training.\micomment{why are we doing this? currently the motivation for these experiments is not clear} In particular, we re-annotate a subset of documents from seven different English coreference datasets (Table~\autoref{table:motivation}), encompassing a diverse mix of domains and different set of guidelines. To collect these annotations, we teach crowd annotators only the broad concept of coreference, including cases where most of the existing guidelines agree. We explore what are the cases where annotators disagree, and hence require further clarification in the annotation guidelines. Furthermore, we identify cases which most crowd annotators mark a certain way but have been resolved differently in the existing guidelines.\micomment{honestly i think this para is redundant given the contributions list that follows. the intro needs to be shorter anyway so maybe you can cut this}
\agcomment{agreed}
% , and what are the cases which most annotators naturally mark as coreferent, and therefore should be included in the guidelines only if the downstream application expect otherwise.

% we explore what are the linguistic phenomena where annotators disagree on, and hence require further clarification in the annotation guidelines, and what are the cases where annotators show high agreement, and therefore should be included in the guidelines only if the downstream application expect different behavior. Furthermore, we identify cases with high agreement among the crowd annotators that have been resolved differently in the existing guidelines. 
% In order to do so, we re-annotate a subset of documents from seven different English coreference datasets, encompassing a diverse mix of domains and different set of guidelines.


% Consequently, a natural question arises when planning any future coreference data collection efforts: what is a simplified set of guidelines that can be reliably used?
% Should we adopt one of the existing guidelines, or should we combine all the existing guidelines? Since existing coreference datasets differ widely in terms of what is considered as a mention and what types of links should be annotated (\citet{universal-anaphora} and \autoref{table:motivation}), it is not straightforward to combine these guidelines, especially resolving cases that are handled differently by each guideline. These challenges are further exacerbated in crowdsource settings, where annotators are eager to maximize their monetary returns by completing many tasks in a short duration, further mandating short and easy-to-comprehend guidelines.
% \mkcomment{I think that sure "This rises a question" but I would rather approach this from a psycholinguistic perspective. So people consider coreference, when given no guidelines. We didn;t really experiment with simplified guidelines as in what works and what does not, we just "let people do what they want" could potentially connect it to some of these papers about using all annots, etc. as in there is noise but there is also a gunuine disagreeent. TLDR: I think we should do psycholinguistic approach, we investigate what people do when not being forced into any system.}
% \mkcomment{just to bring back Poesio's comment today: ""especially ppl whom you haven't trained to death to agree with you" -- maybe this is the way to frame it}

Following are the main contributions of our work:
\begin{enumerate}
\setlength{\itemsep}{2pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
    % \item We explore whether we can collect high-quality coreference data with a \emph{minimal} set of guidelines, only illustrating basic phenomena like pronoun resolution (\autoref{table:tutorial_example}). \mkcomment{what does it mean high quality}
    
    \item We examine how well non-expert annotators agree with existing guidelines given minimal training, only illustrating basic phenomena like pronoun resolution (\autoref{table:tutorial_example}). 

    \item To collect coreference annotations, we propose a methodology, including an intuitive, easy to use for crowdworkers and open-sourced annotation tool---\texttt{ezCoref}\footnote{Our platform's code and collected data is available in supplementary materials, and will be released publicly after blind review.}---supported with a short, effective, crowd-oriented interactive tutorial\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}"} that features step-by-step learning via progression, allowing us to teach annotators the broad concept of coreference.
    
    \item We re-annotate a subset of documents from seven different English coreference datasets, encompassing a diverse mix of domains and different set of guidelines. Our analysis demonstrate that the crowd annotators obtain high agreement with most of the expert annotations, and the quality of our annotations is higher than that of previous crowdsourced efforts.
    \item Using these collected annotations, we answer several interesting questions such as: 
    \begin{enumerate*}
        \item Which domains are most suitable for crowdsourcing coreferences? We observe highest agreement among crowd annotators for the fiction domain. 

        \item Which types of coreference is difficult to annotate in crowdsourcing setups? We find annotators struggle with cataphora.
        
        % \item To what extent do crowd annotators agree with expert annotators? We find annotators agree with expert annotations even without extensive training, signifying that high quality data can be obtained via crowdsourcing with minimalistic guidelines. 

        \item On which linguistic phenomena do annotators agree with experts? We find that appositives and copulae have been annotated similarly by existing guidelines, but annotators naturally mark them differently.
    \end{enumerate*}
    \item  We conclude with a qualitative analysis of such cases and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and inform coreference platform development.
\end{enumerate}

% Coreference resolution is the task of identifying all textual expressions
% that refer to the same discourse entity
% in a given document, and thus grouping such coreferent expressions (mentions) into clusters (entities). Systems trained to solve this task are often an integral component of the preprocessing pipeline for many downstream tasks, such as summarization~\cite{azzam-etal-1999-using, steinberger-etal-2007-two}, question answering \cite{ vicedo-ferrandez-2000-importance, dhingra-etal-2018-neural}, and machine translation~\cite{hardmeier-2012-discourse, bawden-etal-2018-evaluating}.
% % such as summarization~\cite{azzam-etal-1999-using, steinberger-etal-2007-two}, question answering \cite{morton-1999-using, vicedo-ferrandez-2000-importance, dhingra-etal-2018-neural}, relation extraction \cite{zelenko-etal-2004-coreference, verga-etal-2018-simultaneously}, machine translation \cite{hardmeier-2012-discourse, miculicich-werlen-popescu-belis-2017-using, bawden-etal-2018-evaluating}, and sentiment analysis~\cite{jakob-gurevych-2010-using}.
% Modern coreference systems are implemented via data-hungry neural network models~\citep[e.g., ][]{ lee-etal-2017-end, moosavi-strube-2018-using, joshi-etal-2019-bert} trained on large-scale expert-annotated datasets such as OntoNotes~\citep{weischedel-etal-2013-ontonotes}.
% % and PreCo~\citep{chen-etal-2018-preco}. 

% \begin{figure}[t]
%     \centering
%   %\hspace{-3mm}
%   \includegraphics[width=0.48\textwidth, scale=1,clip,trim=0 0 0 0mm]{figs/Interface.pdf}
%   \caption{Part of the \ezcoref interface (\S\ref{sec:software})}
%   \label{figure:interface}
% \end{figure}

% ~\cite{wiseman-etal-2015-learning, clark-manning-2016-deep, lee-etal-2017-end, moosavi-strube-2018-using,  kantor-globerson-2019-coreference, fei-etal-2019-end, joshi-etal-2019-bert},  and various/a number of  datasets~\cite{pradhan-etal-2012-conll, weischedel-etal-2013-ontonotes, poesio-etal-2013-phrase,  cybulska-vossen-2014-using, guha-etal-2015-removing, zeldes-2017-gum, webster-etal-2018-mind, chen-etal-2018-preco, bamman-etal-2020-annotated}. 
% \kkcomment{Can probably move lots of these cites to the related work, currently intro is pretty long and it takes a while until it gets to contributions of work (ezCoref)}

% \agcomment{The OntoNotes and PreCo examples are for language but we are talking about domains too. Also it seems weird to cite so many datasets in previous line and then say that there are only few language or domains} 
% \mkcomment{What's weird is that they keep on making datasets mostly for English and mostly news/informatives, maybe lit.  Anyway I don't think we need these citations in this way. Was that note about datasets always there? somehow remember it saying models but not datasets, seems like we need to clarify that? I mean we are saying there is a lot of datasets then saying we need one. Was it always saying "DIVERSE" datasets? this seems like there are many with many domains etc.}
% \agcomment{yes, we had written models and several datasets and then added citations for both model and datasets}
% \mkcomment{then now it stands out more, "diverse" suggest there are many, and they cover a lot (are very different from each other), changed "diverse" to "various/number of", delete these comments if you agree}





% \begin{table*}[t]
% \centering \scriptsize
% \begin{tabular}{llllcccccc}
% \toprule
% \textbf{Dataset} & \textbf{Domains} & \textbf{Annotators} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{3}{c}{\textbf{Mention Types}} & \multicolumn{3}{c}{\textbf{Coreference Links}} \\ \cmidrule(lr){5-7} \cmidrule(lr){8-10}
%  &  &  &  & \textbf{Singletons} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Entire \\ Appositive\\ Span\end{tabular}}} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} \\ 
%  \midrule
% \textbf{ARRAU} & Multiple & Single expert & Manual & Yes & None & Yes & Special& No Link & Yes \\ \addlinespace[0.2cm]
% \textbf{PD} & Multiple & \begin{tabular}[c]{@{}l@{}}Crowd +\\ 2 experts\end{tabular} & \begin{tabular}[c]{@{}l@{}}Semi\\ automatic\end{tabular} & Yes & None & Yes & Special& Special Link & Yes \\ \addlinespace[0.2cm]
% \textbf{GUM} & Multiple & \begin{tabular}[c]{@{}l@{}}University\\ students with \\ Linguistics\\ background\end{tabular} & Manual & Yes & None & No & Coref (Cop) & Special Link & Yes \\ \addlinespace[0.2cm]
% \textbf{PreCo} & Multiple* & ESL Crowd & Manual** & Yes & None & Yes & Coref & Coref & Yes \\ \addlinespace[0.2cm]
% \textbf{ON} & Multiple & Experts & Mixed & No & None & Yes & Special& Special Link & \begin{tabular}[c]{@{}l@{}}Only with\\ Pronominals\end{tabular} \\ \addlinespace[0.2cm]
% \textbf{LB} & Single & Experts & Manual & Yes & ACE & No & Special& Special Link & \begin{tabular}[c]{@{}l@{}}Only with\\ Pronominals\end{tabular} \\ \addlinespace[0.2cm]
% \textbf{QBZ} & Single & \begin{tabular}[c]{@{}l@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}l@{}}Manual\\ \& CRF\end{tabular} & Yes & \begin{tabular}[c]{@{}l@{}}Characters,\\ Books,\\ Authors*\end{tabular} & No & Coref & Coref & Unspecified \\ \addlinespace[0.2cm]
% \textbf{\ezcoref} & Multiple & Crowd & \begin{tabular}[c]{@{}l@{}}Fully\\ Automatic\end{tabular} & Yes & None & No  &  &  &  \\
% \bottomrule
% \end{tabular}
% \caption{Summary of seven datasets analyzed in this work (abbreviations defined in \S\ref{TODO} \btocomment{cur this is sec2 or sec4.1?? somewhere we need to show/define the boldfaced abbrevs we use in this table and in other tables, along with full names and citations for the datasets.}),
% which differ in domain, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. } \mkcomment{Checking the table for consistancy}}
% \label{table:motivation}
% \end{table*}

% Acquiring these datasets has traditionally been difficult, expensive and time-consuming, requiring linguists trained in fine-grained annotation schemas \citep[e.g., ][]{hovy-etal-2006-ontonotes, poesio-artstein-2008-anaphoric, Uryupina2019}. As such, coreference datasets exist only for a small set of  languages (mostly English) and even then only for limited domains (mainly news and fiction). 
% % \btocomment{is `mainly' a fair summary?} \mkcomment{yes, but should add fiction there}
% Furthermore, these datasets differ widely in their annotation guidelines, resulting in inconsistent annotations across languages and domains,
% with challenging cross-lingual and cross-domain issues \cite{universal-anaphora}.
% %Consider the following sentence that was annotated by both OntoNotes and ARRAU:


%While OntoNotes has only three mentions, ARRAU annotates five mentions, 

% \noindent
% Is it possible to use crowdsourcing and non-expert annotators to generate high-quality coreference data?  As in other types of linguistic annotations, crowdsourcing could reduce costs \cite{snow-etal-2008-cheap}, allowing for larger scale datasets.  Furthermore, by using a standard platform like Amazon Mechanical Turk, this approach is accessible to a wider range of researchers, who may wish to collect new data for different corpora or even languages.


% To this end, we develop \texttt{ezCoref}, a crowdsourced coreference annotation platform that is intuitive and easy to use for crowdworkers, and open-source for other researchers to utilize.\footnote{Our platform's code and collected data is available in supplementary materials, and will be released publicly after blind review.}
% % \ezcoref\ facilitates fast annotations at scale with reduced costs. 
% % \agcomment{need to check this claim, are we reducing costs} \mkcomment{yeah, i think this will always ddepend on how much you are willing to pay (both crowdworkers and linguists... I changed it to possible cost reduction}
% Unlike existing crowdsourced coreference efforts~\cite{chamberlain-etal-2016-phrase, bornstein-2020-corefi, li-etal-2020-active-learning}, \ezcoref\ simplifies the annotation task for workers by using automatically detected mention boundaries\footnote{The syntax-based mention detector is our system's only English-specific component.}, is easily integrable with platforms like Amazon Mechanical Turk, and offers a short, effective, crowd-oriented interactive tutorial\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}"
%  }. %\micomment{add 1-2 more takeaways of the differences} \mkcomment{ankita, we need to look at this when doing final check over zoom}

% In order to train the annotators, we provide a customizable tutorial where annotators are introduced to the annotation task in a fun and interactive manner. Our experiments demonstrate that this tutorial also helps identify annotators genuinely interested in the task.


%  crowdsourcing, which has been demonstrated as a successful approach for several NLP tasks~\cite{snow-2008-cheap, bowman-etal-2015-large, rajpurkar-etal-2016-squad}. 
% This success has led to the development of few annotation
%However, these advances have been hampered, as coreference resolution is a complex linguistic task, which requires not only annotation platform but also simplified yet informative annotation guidelines compatible with crowdsourcing scenario.

%\mkcomment{SIMPLIFY: However, coreference resolution is a complex linguistic task, which requires not only suitable annotation platform but also simplified yet informative annotation guidelines compatible with crowdsourcing scenario /// However, coreference resolution is a complex linguistic task. As such, it requires not only intuitive annotation platform but also simplified yet informative annotation guidelines compatible with crowdsourcing scenario. }

%Standard training procedures used by the existing coreference datasets typically employ lengthy and detailed linguistic guidelines. As such, they are not suitable for crowdsourcing platforms that require task descriptions to be as concise as possible.
% These existing platforms either require annotators to annotate mention pairs~\citep[e.g., ][]{hladka-etal-2009-play, chamberlain-etal-2016-phrase, li-etal-2020-active-learning, ravenscroft-etal-2021-cd},\micomment{what does mention pairs mean? you haven't explained the terminology yet. rewrite into something more intuitive} making the task time-consuming, and therefore less appealing to the crowd workers, or use multiple keyboard key combinations and/or non-intuitive interface \citep[e.g., ][]{bornstein-2020-corefi}, which may be challenging especially for non-experts~\cite{wang-etal-2013-perspectives}.
% \micomment{this paragraph feels out of place. we don't directly compare ezcoref to any of these interfaces, so we can't really claim to be better than them. i think we should just reference them as exsiting work and move onto the main experiments (reannotating existing datasets)}

% \agcomment{will we be offending corefi authors by this statement?}
% \mkcomment{@Ankita: changed the complicated language to multiple keyboard key combinations}

% \agcomment{following two para should be emphasized more}
% With this new interface, we turn to the question of how to define coreference to untrained crowdworkers.
% Expertly-collected datasets such as OntoNotes explain what should and should not be considered coreference via a lengthy set of guidelines~\cite{ontonotes-guidelines} that covers many complex linguistic details (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions).
% %\agcomment{(e.g., how to identify appositive heads and copular structures, some of which should not corefer, which premodifiers can or cannot be linked, etc.)}
% %\micomment{give example in parentheses}\mkcomment{example added} 
% Even if it was feasible to teach such guidelines to crowdworkers, existing coreference datasets differ widely in terms of what is considered as a mention and what types of links should be annotated (\citet{universal-anaphora} and \autoref{table:motivation}), so it is unclear what standards ought to be used.

% Furthermore, crowdsourcing requires concise yet informative guidelines, especially given a complex linguistic task such as coreference resolution.
% Yet, existing annotation guidelines are typically lengthy and cover many linguistic details, some of which may be unnecessary %and can be simplified/omitted/shortened 
% as the annotators would intuitively annotate these types of cases/mentions as coreference.
%they include exhaustive instructions on cases crowd annotators would intuitively annotate as coreferring. 
%details/instructions on cases categories, examples, items, details on annotations crowd workers would do by default, as they include detailed instructions on cases crowd annotator would annotate as corefs by default
%are reflecting the default behavior of the crowd annotators.%As such, they are not suitable for crowdsourcing platforms that require task descriptions to be as concise as possible.
% \mkcomment{this is written as if the system is the main contribution, for now I will leave it as it is as this flow is a bit more coherent}
% \agcomment{we can possibly change the flow in conjunction with the experiments section, since our main arguments for data analysis part are WIP}
% \agcomment{the detailed guidelines are "reflecting the default behavior of the crowd annotators"? I didn't follow this at first. }
% \mkcomment{rewrote it}
% \agcomment{I wonder why this is an issue, or worth mentioning? Traditionally, annotation guidelines must incorporate corner cases where there may be ambiguity, or cases where the task provider wants a specific behaviour from annotators}

%\mkcomment{There is something missing here. You can make an argument "well, but if you simplify, what information do you get out of it". Need to make an argument that: it's even unclear if the lengthy descriptions are needed in the first place, maybe we can get more with less}

% This problem is exacerbated by the fact that the annotation guidelines of the existing datasets differ widely from each other in terms of what is considered as a mention, and what types of links should be annotated~\cite{universal-anaphora} (see FIGURE). Thus, it is unclear which guidelines to employ and how to simplify them so that they will be accessible not only to trained linguists but also to crowd annotators. \jmcomment{Does ezCoref solve this problem or does it introduce another mention detection algo? At this point it's not clear that ezCoref uses its own algorithm or why it's better than existing mention detection criteria. Maybe a one sentence mention that ezCoref uses something better and point to the mention algo section.} \kkcomment{+1 to JM, it's not really clear to me from the intro what exactly ezCoref does that makes it easy for crowdworkers, focusing on mention detection algo + intuitive UI with figure will be helpful}

%the process of familiarizing the annotators with the concept of coreference itself poses a great challenge, requiring deeper analysis. %require more research  

%1existing datasets have different and complicated guidelines
%2if used that than a lot of study
%3hence not feasible for crowdsourcing (also which one to choose anyway)
%4hence we study this

% For instance, consider an example sentence shown in~\ref{fig:motivating_example}, which has been annotated according to seven different annotation guidelines, corresponding to seven coreference datasets drawn from diverse genres and annotation styles. \agcomment{need to fill this up based on example}
% \agcomment{why is this an issue? why having different annotation guidelines a problem?}
% \mkcomment{as to why this is an issue, see my previous comments. need to rewrite this paragraph to make it stronger, dont address reader directly - not to myself}

%Another challenge has been the lack of software that can be easily integrated with crowdsourcing platforms. While there is a number of coreference annotation software designed with crowdsourcing in mind~\cite{chamberlain-etal-2016-phrase, bornstein-2020-corefi, li-etal-2020-active-learning}, they are either time-consuming to set up by the researchers or have a complicated user interface which may pose a challenge for crowd annotators~\cite{wang-etal-2013-perspectives}.
%\mkcomment{Now we are repeating it but I think this should be said earlier where I moved it. (where we first mention the software.}
% \agcomment{I felt like there is a disconnect while moving to this para, can ignore for now}

% Instead, we explore whether we can collect
% high-quality coreference data with a \emph{minimal} set of guidelines, 
% only illustrating basic phenomena like pronoun resolution
% (\autoref{table:tutorial_example}).
% \micomment{add parenthetical about what these guidelines include e.g., pronoun reoslution} \mkcomment{can change to pronoun resolution etc. but I feel like all we give them is what all datasets agree on, and that's strong point, we also list that in a table which we can refer to here} 
% We use \ezcoref\ to re-annotate a subset of documents from seven different English coreference datasets. \agcomment{why? what is the purpose of using so many datasets?} Our crowdworkers
% , each of which uses a different set of guidelines. \mkcomment{that's the third time we mention different set of guidelines, I wonder if we have to have it here?} 
% obtain high agreement with most of the expert annotations, and that the quality of our annotations is higher than that of previous crowdsourced efforts.
% \micomment{not sure if the latter is true, soften if not} \mkcomment{it's true for PD, we made 22 clear mistakes on the part of PD we annotate, compared to 76 or sth clear mistakes of PD; for preco that's 12 our mistakes vs 33 preco's; we do worst on QB, but I don't think that;s really "crowd", proble is that we haven't reported it anywhere yet}.
% \agcomment{Despite \ezcoref's relative lack of guidelines, we observe that our crowdworkers obtain high agreement with most of these expert annotations, and a careful qualitative analysis suggests that our annotations are more reasonable than that of previous crowdsourced efforts.} 
% We conclude with a qualitative analysis of our annotators' behavior and the types of annotation decisions they make, which we hope will inform future research into coreference platform development and guideline construction.
% to determine the default behavior of crowd annotators.  \kkcomment{What is the one line conclusion from this expt? It will be good to mention that here}
% We further investigate the differences in annotations for each of these datasets and compare them against annotations of crowd workers.  
%- getting crowdsource perspective on coref resolution
%This paper is the first to gather and categorize these inconsistencies and provide suggestions for future annotation efforts and evaluation decisions. \mkcomment{it's not the first to gather and categorize inconsistencies}

% Our contributions in this work are threefold: 

%(1)
%we develop ezCoref, a new annotation platform to collect crowdsourced annotations for coreference resolution, (2) We use this platform to gather crowdsourced annotations for seven existing datasets drawn from diverse genres and categorize inconsistencies among their annotation guidelines and 3) Finally, based on our observations, we highlight challenges in crowdsourcing coreferences and provide suggestions for future annotation efforts and evaluation decisions.


% \begin{enumerate}
% \setlength{\itemsep}{2pt}
% \setlength{\parskip}{0pt}
% \setlength{\parsep}{0pt}

% \item We develop \ezcoref, a new annotation platform to easily collect crowdsource annotations of coreference, that can be used for multiple languages and domains.

% \item We gain a crowdsource perspective on coreference resolution by re-annotating 240 passages from seven existing datasets covering X different domains.
% \mkcomment{add somehow qualitative analysis? nobody does that cause it's so time-consuming, but also insightful - will add below; maybe add how many markables?}

% \item We perform extended quantitative and qualitative analysis showing....  

% \end{enumerate}


% \section{Introduction Rough Notes}
% - coref resolution is a task ... 

% - most corpora are annotated by experts (costly, takes time)

% - but often using different set of guidelines, very detailed guidelines

% - yet unclear why some annot choices were made 

% - alternative - crowdsourcing

% - detailed guidelines is not okay for crowdsourcing. need a way to teach people more intuitively.
%     - teach people the idea of what coref is but rely on ppls perception to decide whether two mentions are coref or not
    
%     -but will it work? because expertise level vary, cant give very detailed guidelines/linguistic knowledge. 

%     -hard to get annotations for long documents on crowdsourcing platforms. People want to do many small tasks as compared to one long task. 

%     - we simplify the task by short docs, easy guidelines, clear interface
    
%     - are we reducing the cost? 
%     - we are reducing time it takes to collect the data. 
%         - learning time is small
%         - power of many people working together
%         - different people working on different segments of a document
    
    
% - based on ppls perception we find that ... 

% - why need to care about disagreements: uncertainty estimates using disagreements among annotators. 
% - real life application: grammarly to identify cases of ambiguity.

% \textbf{Contribution of this paper}:

% - proof of concept - it can be done via crowdsourcing

% - reannotate various corpora to see what the crowd will do vs experts
%     -why???

% - analyzed disagreement, identified cases to include in guidelines
%     - inter annotator disagreements
%     - disagreements with existing guidelines; but annotators unanimously agree

% - our results indicate / show that....

% - clean software + tutorial

% - study can help inform future efforts for collecting annotations for coreference resolution and
% act as a helpful resource for designing annotation
% guidelines
    


% ========================================== 

    
% Recommendations/Advice/Key takeaway
%     1. What to include in tutorial mode
%     2. 




==> emnlp_sections/introductionv2.tex <==
\section{Introduction}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document.
% Building a coreference system, an integral component of the preprocessing pipeline for several downstream tasks, such as summarization~\cite{azzam-etal-1999-using, steinberger-etal-2007-two}, question answering \cite{ vicedo-ferrandez-2000-importance, dhingra-etal-2018-neural}, and machine translation~\cite{hardmeier-2012-discourse, bawden-etal-2018-evaluating}, has been a long-standing goal in NLP research. 
Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase, chen-2018-preco}. \textbf{However, these datasets vary widely in their definition of coreference (expressed through annotation guidelines), resulting in inconsistent annotations both within and across languages and domains~\cite{universal-anaphora} (e.g., English news in Figure~\ref{figure:data_guidelines})}. 


\begin{table}[]
\centering
\tiny
\begin{tabular}{ll}
\hline
Dataset     & Example                                                                                                              \\ \hline \addlinespace[0.1cm]
OntoNotes   & \begin{tabular}[c]{@{}l@{}}Maybe we need a \color{teal}{[}CIA{]}\color{black}\;version of the Miranda warning : \\ You have the right to conceal your coup intentions, \\ because we may rat on you .\end{tabular}                                                                                 \\ \addlinespace[0.2cm]

ARRAU       & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the Miranda warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right to conceal \color{magenta}{[}your{]}\color{black}\; {[}coup{]}e16 intentions{]}eS{]}eS, \\ because {[}we{]}eS may rat on \color{red}{[}you{]}\color{black}\;.\end{tabular} \\ \addlinespace[0.2cm]

Crowd (this work) & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the {[}Miranda{]}eS warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right{]}eS to conceal \color{blue}{[}your{]}\color{black}\; coup intentions{]}eS, \\ because \color{brown}{[}we{]}\color{black}\; may rat on \color{blue}{[}you{]}\color{black}\;\end{tabular}    \\ \hline
\end{tabular}
\captionof{figure}{A sentence annotated according to different guidelines. \agcomment{WIP}}
\label{figure:data_guidelines}
\end{table}

% This lack of a uniform standard guidelines is crucial to address as we move towards collecting larger datasets with broader coverage of languages and domains~\cite{universal-anaphora}. 

To collect a new coreference dataset, one has to decide which guidelines to employ. \textbf{This is not a straightforward task, as the differences in existing guidelines can be significant not only in terms of what can and cannot corefer, but also in what is even considered to be a mention~(\autoref{table:motivation}).} \agcomment{the first para says in one line the main issue addressed in this paper. I wanted to elaborate on this issue in the second para and justify why this isn't a trivial problem to address.} \mkcomment{this repeats what was said two sentences ago: "However, these resources vary
widely in their annotation guidelines"} These differences further make it expensive and time-consuming to iterate over candidate guidelines, requiring expert understanding to resolve inconsistencies. \mkcomment{this is hard to understand, i think i know what you mean, but it's not immediately clear why would you even iterrate over existing guidelines} For instance,~\citet{uryupina2020annotating} iteratively refined their guidelines over approximately 10 years to maximize intercoder agreement when collecting the ARRAU dataset. 

% \mkcomment{did it take them 10y to iterate? I had the impression that the iteration was sth shortish; they do check mistakes each release but I don't think it took them 10y to come up with guidelines (?)}

To reduce annotation cost and time, more recent efforts have moved towards crowdsourcing large coreference datasets, including payment-based approaches~\cite{chen-2018-preco, guha-etal-2015-removing} and games-with-a-purpose (GWAPs) approaches~\cite{chamberlain-etal-2016-phrase}. \textbf{These efforts also face similar challenges, which guidelines to employ for crowdsourcing datasets? Furthermore, crowdsourcing setups must overcome the additional challenge of teaching complex linguistic concepts, such as coreference, to non-expert annotators.} Traditional data collection approaches involve experts (linguists) trained in lengthy guidelines~\citep[e.g.,][]{ontonotes-guidelines} explaining in detail what should and should not be considered coreference (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions).\micomment{redundant sentence} Even if it was feasible to teach such guidelines to crowd annotators, vast differences in guidelines of the existing coreference datasets make it unclear what standards ought to be used.

To address the issue of teaching coreference to crowd annotators, researchers have proposed using the notion of learning by progression~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, whereby the annotators start with simpler tasks, and then they are progressively taught more complex tasks. \textbf{However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks.} As for the issue of lack of standardized guidelines, at the moment, there is only limited consensus on the various aspects of coreference phenomena that should be covered by any annotation guidelines~\cite{universal-anaphora}. \micomment{what does this para add? seems better suited for related work}

% Some proposals have been made to adopt a strategy similar to that of the MATE proposal~(Poesio et al., 1999)- i.e., segregating various aspects of coreference into core and optional aspects. However, existing approaches often decide these differences based on linguistic concepts, and no prior work has accounted for human perspectives.  

In this work, we crowdsource coreference annotations by providing the annotators minimal training, teaching only the broad concept of coreference. \textbf{By observing agreements/disagreements among annotators under minimal training, we aim to understand which coreference concepts are easy to annotate for crowd annotators and which concepts are difficult.} Such an understanding would not only help effective crowdsourcing (e.g., employment of learning by progression strategy) but also help identify difficult concepts to prioritize and elucidate while curating annotation guidelines. 

\agcomment{Another attempt at previous para}
In this work, we crowdsource coreference annotations by providing the annotators minimal training, teaching only the broad concept of coreference. \textbf{We provide minimal training to avoid altering the unbiased/raw/natural perception of annotators. We use these collected annotations to study the deviations of crowd annotations from the existing guidelines. Such deviations can highlight the avenues that must be revisited by the research community for future data collection efforts.} Furthermore, these annotations can also help us understand which coreference concepts are easy/intuitive and difficult for crowd annotators. Such an understanding would not only help effective crowdsourcing (e.g., employment of learning by progression strategy) but also help identify difficult concepts to prioritize and elucidate while curating annotation guidelines. 

Our main contributions in this work are:
\begin{enumerate}
\setlength{\itemsep}{2pt}
\setlength{\parskip}{0pt}
\setlength{\parsep}{0pt}
    % \item We explore whether we can collect high-quality coreference data with a \emph{minimal} set of guidelines, only illustrating basic phenomena like pronoun resolution (\autoref{table:tutorial_example}). \mkcomment{what does it mean high quality}
    \item We examine how well non-expert annotators agree with existing guidelines given minimal training, only illustrating basic phenomena like pronoun resolution (\autoref{table:tutorial_example}). 
    
    \item We \textbf{re-annotate a subset of documents from seven different English coreference datasets}, encompassing a diverse mix of domains and different set of guidelines. 

    \item To collect coreference annotations, we propose a \textbf{methodology}, including an intuitive, easy to use for crowdworkers and open-sourced annotation tool---\texttt{ezCoref}\footnote{Our platform's code and collected data is available in supplementary materials, and will be released publicly after blind review.}---supported with a short, effective, crowd-oriented interactive tutorial\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}"}, allowing us to teach annotators the broad concept of coreference.
    
    \item Using these collected annotations, we \textbf{answer} several interesting questions such as: 
    \begin{enumerate*}
        \item Which domains are most suitable for crowdsourcing coreferences? We observe \textbf{highest agreement among crowd annotators for the fiction domain}. 

        \item Which types of coreference is difficult to annotate in crowdsourcing setups? \textbf{We find annotators struggle with cataphora.}
        
        % \item To what extent do crowd annotators agree with expert annotators? We find annotators agree with expert annotations even without extensive training, signifying that high quality data can be obtained via crowdsourcing with minimalistic guidelines. 

        \item On which linguistic phenomena do annotators disagree with experts? We find that \textbf{appositives and copulae} have been annotated similarly by existing guidelines, but annotators naturally mark them differently and would require clarification in guidelines if expected otherwise.
    \end{enumerate*}
    \item  We conclude with a \textbf{qualitative analysis} of such cases and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and inform coreference platform development.
\end{enumerate}


\begin{table*}[]
\centering 
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{lccccclcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Domains\\ $\#$(doc, ment, tok)\end{tabular}}} & \multirow{2}{*}{\textbf{Annotators}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{2}{c}{\textbf{Mention Types}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Coreference Links}} &  \\ \cline{5-6} \cline{8-11} \addlinespace[0.05cm]
 &  &  &  & \textbf{Singletons} & \textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}} & \multicolumn{1}{c}{} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} & \textbf{Ambiguity} \\\midrule
 
\textbf{\begin{tabular}[c]{@{}l@{}}ARRAU\\ \cite{Uryupina2019}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (552, 99K, 350K)\end{tabular}  & Single Expert & Manual & Yes & None &  & Special Link & No Link & Yes & Explicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}Phrase Detectives (PD)\\ \cite{chamberlain-etal-2016-phrase}\end{tabular}}& \begin{tabular}[c]{@{}c@{}}Multiple\\ (542, 100K, 400K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Crowd (gamified) +\\ 2 Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semi\\ Automatic\end{tabular} & Yes & None &  & Special Link & Special Link & Yes & Implicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}GUM\\\cite{zeldes-2017-gum}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (25, 6K, 20K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Experts \\ (Linguistics Students)\end{tabular} & Manual & Yes & None &  & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Types)  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Type)  \end{tabular} & Yes & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}PreCo \\ \cite{chen-etal-2018-preco}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple***\\ (38K, 3.58M, 12.5M)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Non-Expert, \\ Non-Native \end{tabular}& Manual** & Yes & None &  & Coref & Coref & Yes & None \\ \addlinespace[0.1cm]

\textbf{\begin{tabular}[c]{@{}l@{}}OntoNotes\\ \cite{hovy-etal-2006-ontonotes}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (1.6K, 94K, 950K)\end{tabular}  & Experts & Mixed & No & None &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}LitBank\\ \cite{bamman-etal-2020-annotated}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (100, 29K, 210K)\end{tabular}  & Experts & Manual & Yes & ACE (selected) &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}QuizBowl\\ \cite{guha-etal-2015-removing}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (400, 9.4K, 50K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Manual\\ \& CRF*\end{tabular} & Yes & \begin{tabular}[c]{@{}c@{}}Characters,\\ Books,\\  Authors*\end{tabular} &  & Coref & Coref & If Applicable & None \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}ezCoref Pilot Dataset 
\\ (this work)\end{tabular}} & Multiple & Crowd (paid) & \begin{tabular}[c]{@{}c@{}}Fully\\ Automatic\end{tabular} & Yes & None &  & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & Implicit \\ \bottomrule
\end{tabular}
\end{adjustbox}

\caption{Summary of seven datasets analyzed in this work,
which 
differ in domain, size, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. }\scriptsize{***See Footnote \ref{fn:preco}.}} 
\label{table:motivation}
\end{table*}

% \agcomment{broad area of the paper, recent progress, key limitation}

% \agcomment{give an example of key limitation}

% \agcomment{why and where, addressing this challenge is useful. why addressing this challenge isn't trivial.}

% \agcomment{some existing efforts to address this issue, and one line limitation.}


% \agcomment{what do we do in this paper to address this issue.}


% \agcomment{our contributions}


==> emnlp_sections/introductionv3.tex <==
\section{Introduction}

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\textwidth, scale=0.8,clip,trim=0 0 0 0mm]{figs/motivation_effort.pdf}
\caption{Annotator efforts versus efforts of a researcher interested in collecting new datasets. \ezcoref explores the minimum effort scenario for both annotators and researchers. \agcomment{this diagram is rough, i still have to carefully think which dataset to place where, and beautify it.}}
\mkcomment{PreCo-should be a bit higher on the researcher effort and a bit further on annot effort than ezCoref (because of the need to go through and first develop simplified (less than ours) guidelines; they are the most similar but also have a bit more detailed guidelines resulting in annot/researcher efforts going up just a bit; QuizBowl and PD I would assume have similar guidelines as PreCp (can be a bit closer to us cause maybe they are simpler?); the research effort in PD is definitely sky-high; why is it so for QB? need to get experts? GUM has maybe higher researcher efforsts cause they literary spend a semester teaching ppl how to annot? (ragardless of whether that's needed of not, since it's part of the class) LB I would say maybe has less annot effort as the entities are restricted? I don't remember whether they automatically identify them}
\label{figure:motivation_efforts}
\end{figure}

Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase, chen-2018-preco}. However, these datasets vary widely in their definition of coreference (expressed through annotation guidelines), resulting in inconsistent annotations both within and across languages and domains~\cite{universal-anaphora} (e.g., English news in Figure~\ref{figure:data_guidelines}). 


Because of the differences in the existing guidelines, it is difficult to know which guidelines to use when collecting datasets in a new domain or language. Furthermore, these guidelines frequently include lengthy explanations of complex linguistic concepts~\citep[e.g.,][]{ontonotes-guidelines}, detailing what should and should not be corefer (e.g., how to deal with head-sharing noun phrases, which premodifiers can and cannot corefer, or how to annotate generic mentions). 
% \mkcomment{seems weird with these two e.g.; it's basically the same} 
As a result, coreference datasets have traditionally been curated by linguists (experts) already familiar with such concepts. 
Even so, annotators may have to frequently refer to these guidelines, which results in significant annotator efforts (e.g., OntoNotes and ARRAU as shown in Figure~\ref{figure:motivation_efforts}).  

% In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.

More recently, efforts have been made to crowdsource coreference annotations by utilizing non-experts to annotate large corpora~\cite{chen-2018-preco, chamberlain-etal-2016-phrase}. For instance, applying the games-with-a-purpose (GWAPs) approach~\cite{von-ahn-2006-gwap, poesio2017crowdsourcing, kicikoglu2020aggregation, madge-etal-2019-making}, which emphasizes on fun as a motivator for annotators, researchers have successfully curated coreference datasets~\cite{poesio2019crowdsourced, poesio2013phrase, chamberlain-etal-2016-phrase}. While GWAPs make it interesting and enjoyable \mkcomment{I think GWAP is a fixed term? "game-with-a-pupose" not gameS; you probably can use "GWAPs" is you really want to but I wouldn't use "games-with..."}\agcomment{great point! though, I think gameS-with-a-purpose is equally valid, for instance Poessio uses this term in \url{https://dl.acm.org/doi/pdf/10.1145/2448116.2448119}; section 2.4 and von Ahn, one of the pioneers who popularized this concept, also uses "games"} for non-expert annotators to annotate documents, these methods necessitate significant researcher efforts to build such games and keep them visible for data collection~\cite{poesio-etal-2013-PDoverview} (e.g., Phrase Detectives in Figure~2). Furthermore, even this approach %\mkcomment{this approach; it's not a system, i think} 
is challenged by complex, lengthy guidelines, as non-expert annotators in crowdsourcing setups \mkcomment{in any setup really, and it's kind of crowdsourcing anyway in nlp when you use non-experts, this is redundant} require concise, easy-to-understand guidelines to perform well and remain engaged.

Another alternative for crowdsourcing linguistic annotations, including coreferences, is to use traditional payment-based methods (e.g., Amazon Mechanical Turk)~\cite{snow-2008-cheap, cybulska-vossen-2014-using, roit-etal-2020-controlled, bornstein-2020-corefi}, which are much easier to setup the task \mkcomment{more like easier to recruit the annotators "which offer an easier way to recruit the annotators while offering a dirverse..." - task setup depends on your annot interface, etc.; also not sure about this "diverse" claim; there are very specific ppl on AMT; it's pretty much NOT direverse} and offer a diverse workforce, reducing the researcher's efforts. However, these systems have the same difficulties in teaching complicated linguistic tasks to crowd annotators. \mkcomment{what "systems", I don't think this is the best word choice}


One of the solutions proposed in the literature, also investigated for GWAPs, is to incorporate the \textit{learning by progression} approach~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, where the annotators start with simpler tasks and gradual move towards more complex problems.
% One of the proposed solutions, also investigated for GWAPs, is to use the notion of learning by progression~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, whereby the annotators start with simpler tasks, and then they are progressively taught more complex tasks. \mkcomment{One of the solutions proposed in the literature is to incorporate the \textit{learning by progression approach}, where the annotators start with simpler tasks and gradual move towards more complex problems.} 
However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks. \mkcomment{However, in order to efficiently employ the \textit{learning by progression} approach, researchers have to identify which cases are .... }

\mkcomment{this transition is a bit rough; you mention the need to identiry these easy vs difficult cases and then switch to another topic without saying that this is what we do... should finish that thing first, then switch to minimal guidelines as a way to coref}
In this work, we investigate whether it is feasible to crowdsource coreference resolution under minimal guidelines. For instance, annotations for pronoun resolution which are very useful for information extraction tasks can be obtained via minimal training, as observed in our experiments. If we can obtain good annotations via minimal training, that can speed up the process and make it easier for other researchers to collect new datasets, thereby reducing both annotator and researcher efforts. 

In particular, we propose a methodology---\texttt{ezCoref}---which includes an intuitive, easy to use for crowdworkers and open-sourced annotation tool,\footnote{Our platform's code and collected data is available in supplementary materials, and will be released publicly after blind review.} supported with a short, effective, crowd-oriented interactive tutorial,\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}"} allowing us to teach annotators the broad concept of coreference. Using \texttt{ezCoref}, we re-annotate 240 passages from seven existing English coreference datasets and for the first time compare the quality of crowdsourced coreference annotations against those of experts, and identify where their behavior differs to facilitate future annotation efforts.

We obtain a high agreement among annotators for the fiction domain, suggesting that this domain is suitable to collect crowdsourced coreference annotations. Comparing various linguistic concepts, we find that annotators struggle with cataphoras, resulting in multiple mistake when annotating QuizBowl dataset~\cite{guha-etal-2015-removing}. Finally, comparing the expert guidelines with crowd annotations, we find that appositives and copulae have been annotated similarly by existing guidelines, but annotators naturally mark them differently and would require clarification in guidelines if expected otherwise. \mkcomment{<---this sentence is not the smoothest, the point of it is too far in the forest; Finally, we find that non-expert annotators tend to annotate metions in appositives and copulae as coreferent, even though most of existing guidelines connected these with another, special link. ....though that is not true either right... they don't tend to do that, they are all over the place with copula but maybe better with appos, then it's the question of major vote} We conclude with a qualitative analysis of such cases and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and inform coreference platform development.


\begin{table}[]
\centering
\tiny
\begin{tabular}{ll}
\hline
Dataset     & Example                                                                                                              \\ \hline \addlinespace[0.1cm]
OntoNotes   & \begin{tabular}[c]{@{}l@{}}Maybe we need a \color{teal}{[}CIA{]}\color{black}\;version of the Miranda warning : \\ You have the right to conceal your coup intentions, \\ because we may rat on you .\end{tabular}                                                                                 \\ \addlinespace[0.2cm]

ARRAU       & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the Miranda warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right to conceal \color{magenta}{[}your{]}\color{black}\; {[}coup{]}e16 intentions{]}eS{]}eS, \\ because {[}we{]}eS may rat on \color{red}{[}you{]}\color{black}\;.\end{tabular} \\ \addlinespace[0.2cm]

Crowd (this work) & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the {[}Miranda{]}eS warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right{]}eS to conceal \color{blue}{[}your{]}\color{black}\; coup intentions{]}eS, \\ because \color{brown}{[}we{]}\color{black}\; may rat on \color{blue}{[}you{]}\color{black}\;\end{tabular}    \\ \hline
\end{tabular}
\captionof{figure}{A sentence annotated according to different guidelines. \agcomment{WIP}}
\label{figure:data_guidelines}
\end{table}


\begin{table*}[]
\centering 
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{lccccclcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Domains\\ $\#$(doc, ment, tok)\end{tabular}}} & \multirow{2}{*}{\textbf{Annotators}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{2}{c}{\textbf{Mention Types}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Coreference Links}} &  \\ \cline{5-6} \cline{8-11} \addlinespace[0.05cm]
 &  &  &  & \textbf{Singletons} & \textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}} & \multicolumn{1}{c}{} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} & \textbf{Ambiguity} \\\midrule
 
\textbf{\begin{tabular}[c]{@{}l@{}}ARRAU\\ \cite{Uryupina2019}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (552, 99K, 350K)\end{tabular}  & Single Expert & Manual & Yes & None &  & Special Link & No Link & Yes & Explicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}Phrase Detectives (PD)\\ \cite{chamberlain-etal-2016-phrase}\end{tabular}}& \begin{tabular}[c]{@{}c@{}}Multiple\\ (542, 100K, 400K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Crowd (gamified) +\\ 2 Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semi\\ Automatic\end{tabular} & Yes & None &  & Special Link & Special Link & Yes & Implicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}GUM\\\cite{zeldes-2017-gum}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (25, 6K, 20K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Experts \\ (Linguistics Students)\end{tabular} & Manual & Yes & None &  & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Types)  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Type)  \end{tabular} & Yes & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}PreCo \\ \cite{chen-etal-2018-preco}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple***\\ (38K, 3.58M, 12.5M)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Non-Expert, \\ Non-Native \end{tabular}& Manual** & Yes & None &  & Coref & Coref & Yes & None \\ \addlinespace[0.1cm]

\textbf{\begin{tabular}[c]{@{}l@{}}OntoNotes\\ \cite{hovy-etal-2006-ontonotes}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (1.6K, 94K, 950K)\end{tabular}  & Experts & Mixed & No & None &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}LitBank\\ \cite{bamman-etal-2020-annotated}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (100, 29K, 210K)\end{tabular}  & Experts & Manual & Yes & ACE (selected) &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}QuizBowl\\ \cite{guha-etal-2015-removing}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (400, 9.4K, 50K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Manual\\ \& CRF*\end{tabular} & Yes & \begin{tabular}[c]{@{}c@{}}Characters,\\ Books,\\  Authors*\end{tabular} &  & Coref & Coref & If Applicable & None \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}ezCoref Pilot Dataset 
\\ (this work)\end{tabular}} & Multiple & Crowd (paid) & \begin{tabular}[c]{@{}c@{}}Fully\\ Automatic\end{tabular} & Yes & None &  & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & Implicit \\ \bottomrule
\end{tabular}
\end{adjustbox}

\caption{Summary of seven datasets analyzed in this work,
which 
differ in domain, size, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. }\scriptsize{***See Footnote \ref{fn:preco}.}} 
\label{table:motivation}
\end{table*}


\ignore{
\subsubsection{bullet points}
Existing datasets differ widely in their guidelines, so we don’t know which one to employ for new data collection. 

These guidelines are often complex with many arbitrary decisions.

Complex guidelines require experts but collecting annots with experts is expensive and time consuming (small num of experts working on large num of docs)

Crowdsourcing is a non-expert alternative which was recently done by using GWAP - but that is also time consuming (development, PR); the annotators may be motivated (yay, it’s a game!) but they need simplified guidelines

Alternative is traditional crowdsourcing but just as GWAP it requires simplified guidelines - teach ppl what you want (ppl can resolve coref naturally, but need to explain them the task)

One of the proposed solutions applied also in GWAP is to use the notion of learning by progression = iterating through concepts from easy to difficult cases. But for it to be done well with minimum time from workers => it requires researchers to identify what is hard and what is easy for a better / more efficient design

In this work, we try to address this question. We collect annotations under minimal training to identify what is hard and easy for annotators. Furthermore, deviations from existing expert guidelines can help inform avenues to revisit.

\subsection{text}
\agcomment{WIP}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase, chen-2018-preco}. However, these datasets vary widely in their definition of coreference (expressed through annotation guidelines), resulting in inconsistent annotations both within and across languages and domains~\cite{universal-anaphora} (e.g., English news in Figure~\ref{figure:data_guidelines}). 

Coreference datasets vary in terms of their definition of coreference expressed via different guidelines, annotation formats and annotation platform used to collect the dataset. All these differences have impacts on the quality of collected data. These datasets not only differ in terms of what is coreference but also what is considered as a mention. Unfortunately, at the moment, there is only limited consensus on the various aspects of coreference phenomena that should be covered by any annotation guidelines~\cite{universal-anaphora}

In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.

Another complimentary dimension in which these datasets differ is how these datasets were collected. Traditionally, these datasets such as OntoNotes were collected via expert annotators trained in lengthy guidelines. More recently, impressive progress has been made towards crowdsourcing coreference annotations. Both payment based approaches and games-with-a-purpose has been proposed and impressive success has been achieved e.g., as demonstrated by the success of Phrase Detectives. However, GWAPs are often not open-sourced and require maintaining constant visibility to collect annotations, thereby significantly increasing researcher efforts to collect new datasets. 

In this work, we investigate whether it is feasible to crowdsource coreference resolution under minimal guidelines? For instance, annotations for pronoun resolution which are very useful for information extraction tasks can be obtained via minimal training, as observed in our experiments. If we can obtain good annotations via minimal training, that can speed up the process and make it easier for other researchers to collect new datasets.
}



% \agcomment{broad area of the paper, recent progress, key limitation}

% \agcomment{give an example of key limitation}

% \agcomment{why and where, addressing this challenge is useful. why addressing this challenge isn't trivial.}

% \agcomment{some existing efforts to address this issue, and one line limitation.}

% \agcomment{what do we do in this paper to address this issue.}

% \agcomment{our contributions}

==> emnlp_sections/introductionv4.tex <==
\section{Introduction}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.5\textwidth, scale=0.8,clip,trim=0 0 0 0mm]{figs/motivation_effort.pdf}
% \caption{Annotator efforts versus efforts of a researcher interested in collecting new datasets. \ezcoref explores the minimum effort scenario for both annotators and researchers. \agcomment{this diagram is rough, i still have to carefully think which dataset to place where, and beautify it.}}
% % \mkcomment{PreCo-should be a bit higher on the researcher effort and a bit further on annot effort than ezCoref (because of the need to go through and first develop simplified (less than ours) guidelines; they are the most similar but also have a bit more detailed guidelines resulting in annot/researcher efforts going up just a bit; QuizBowl and PD I would assume have similar guidelines as PreCp (can be a bit closer to us cause maybe they are simpler?); the research effort in PD is definitely sky-high; why is it so for QB? need to get experts? GUM has maybe higher researcher efforsts cause they literary spend a semester teaching ppl how to annot? (ragardless of whether that's needed of not, since it's part of the class) LB I would say maybe has less annot effort as the entities are restricted? I don't remember whether they automatically identify them}
% \label{figure:motivation_efforts}
% \end{figure}

Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated datasets~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase}. However, these datasets vary widely in their definitions of coreference and annotation guidelines, resulting in inconsistent annotations both within and across domains and languages. For instance, in a common English news sentence, while ARRAU~\cite{Uryupina2019} treats generic pronouns as non-referring, OntoNotes chooses not to mark them at all (Figure~\ref{figure:data_guidelines}). 
% ~\cite{universal-anaphora}
%(e.g., English news in Figure~\ref{figure:data_guidelines}). 


% \begin{quote}
% \small
% \textbf{OntoNotes}: Maybe we need a {\color{red}[} CIA {\color{red}\texttt{]e1}} version of the Miranda warning: You have the right to conceal your coup intentions, because we may rat on you. \vspace{0.2cm}\\
% \textbf{ARRAU}: Maybe {\color{teal}[} we {\color{teal}\texttt{]e1}} need a {\color{red}[} CIA {\color{red}\texttt{]e2}} version of the Miranda warning: {\color{blue}[} You {\color{blue}\texttt{]e1}} have the right to conceal {\color{orange}[} your {\color{orange}\texttt{]e1}} coup intentions, because {\color{brown}[} we {\color{brown}\texttt{]e1}} may rat on {\color{violet}[} you {\color{violet}\texttt{]e1}}. \vspace{0.2cm}\\
% \textbf{Crowd (this work)}: Maybe {\color{teal}[} we {\color{teal}\texttt{]e1}} need {\color{red}[} a {\color{ForestGreen}[} CIA {\color{ForestGreen}\texttt{]e2}} version of the Miranda warning {\color{red}\texttt{]e2}}: {\color{blue}[} You {\color{blue}\texttt{]e1}} have {\color{magenta}[} the right {\color{magenta}\texttt{]e1}} to conceal {\color{orange}[} {\color{blue}[} your {\color{blue}\texttt{]e1}} coup intentions {\color{orange}\texttt{]e1}} , because {\color{teal}[} we {\color{teal}\texttt{]e1}} may rat on {\color{blue}[} you {\color{blue}\texttt{]e1}}. \vspace{0.2cm}\\
% \end{quote}

% \begin{quote}
% \small
% \textbf{OntoNotes}: {\color{red} \texttt{[}} Lloyd's, once a pillar of {\color{blue} \texttt{[}} the world insurance market {\color{blue} \texttt{]e1}}, {\color{red} \texttt{]e2}} is being shaken to {\color{red} \texttt{[}} its {\color{red} \texttt{]e2}} very foundation.\vspace{0.2cm}\\
% \textbf{ARRAU}: {\color{red} \texttt{[}} Lloyd's, once {\color{violet}\texttt{[}} a pillar of {\color{blue}\texttt{[}} the world {\color{teal}\texttt{[}} insurance {\color{teal}\texttt{]e3}} market \texttt{{\color{blue}]e2} {\color{violet}]eS1} {\color{red} ]e1}}, is being shaken to \texttt{{\color{brown}[} {\color{red}[}} its {\color{red}\texttt{]e1}} very foundation {\color{brown} \texttt{]eS2}}.
% \end{quote}

% \begin{table}[t]
% \centering
% \tiny
% \begin{tabular}{ll}
% \hline
% Dataset     & Example                                                                                                              \\ \hline \addlinespace[0.1cm]
% OntoNotes   & \begin{tabular}[c]{@{}l@{}}Maybe we need a \color{teal}{[}CIA{]}\color{black}\;version of the Miranda warning : \\ You have the right to conceal your coup intentions, \\ because we may rat on you.\end{tabular}                                                                                 \\ \addlinespace[0.2cm]

% ARRAU       & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the Miranda warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have {[}the right to conceal \color{magenta}{[} \color{orange}{[}your{]} \color{magenta}{[}coup{]}\color{magenta}\; intentions{]}\color{black}, \\ because \color{violet}{[}we{]}\color{black}\; may rat on \color{red}{[}you{]}\color{black}.\end{tabular} \\ \addlinespace[0.2cm]

% Crowd (this work) & \begin{tabular}[c]{@{}l@{}}Maybe \color{brown}{[}we{]}\color{black}\; need {[}a \color{teal}{[}CIA{]}\color{black}\; version of {[}the {[}Miranda{]}eS warning{]}eS{]}eS :\\ \color{blue}{[}You{]}\color{black}\; have \color{orange}{[}the right{]}\color{black}\; to 
% \color{magenta}{[}conceal \color{blue}{[}your{]} \color{magenta} coup intentions{]}\color{black}, \\ because \color{brown}{[}we{]}\color{black}\; may rat on \color{blue}{[}you{]}.\color{black}\;\end{tabular}    \\ \hline
% \end{tabular}
% \captionof{figure}{A sentence annotated according to two different guidelines and our crowd annotators. \agcomment{WIP}}
% \label{figure:data_guidelines}
% \end{table}

\begin{figure}[t]
    \centering
  %\hspace{-3mm}
  \includegraphics[width=0.45\textwidth, scale=0.7,clip,trim=0 0 0 0mm]{emnlp2022-latex/EMNLP 2022/figs/motivation_guidelines.pdf}
  \caption{A common sentence annotated by both OntoNotes~\cite{hovy-etal-2006-ontonotes} and ARRAU~\cite{Uryupina2019}. We visualize both annotations along with the crowd annotations obtained in our study using \ezcoref\ platform. 
  While OntoNotes does not mark generic pronouns and ARRAU marks them as non-referring mentions, our crowdworkers mark all generic pronouns (e.g., ``you'' and ``we'') as coreferent.}
  \vspace{-0.1in}
%   \caption{This sentence was annotated by both OntoNotes~\cite{hovy-etal-2006-ontonotes} and ARRAU~\cite{Uryupina2019}. Each dataset's respective coreference annotations are shown above, along with annotations by crowdworkers using our \ezcoref\ platform. 
% %   OntoNotes and ARRAU themselves differ in their definitions of mentions and coreferences. cx
%   While OntoNotes does not mark generic pronouns and ARRAU marks them as non-referring mentions, our crowdworkers mark all generic pronouns (e.g., ``you'' and ``we'') as coreferent. 
% %   We do not show entity ids for most of the singletons for visual clarity.
%   }
\label{figure:data_guidelines}
\end{figure}

% \footnotetext{Entity annotations for most singletons omitted for visual clarity.}
% A common sentence drawn from two datasets, OntoNotes and ARRAU, with gold annotations as per their guidelines and re-annotated by our crowdworkers by using \ezcoref. While OntoNotes and ARRAU themselves differ in their definition of mentions and coreferences, crowdworkers with minimal guidelines have a completely different perception compared to these two datasets. OntoNotes does not mark generic pronouns, ARRAU marks generic pronouns as non-referring, however, crowdworkers naturally mark generic pronouns as coreferent.

When collecting a new coreference dataset, how should the annotation guidelines be chosen? Traditionally, these guidelines have leaned towards lengthy explanations of complex linguistic concepts, such as those in the OntoNotes guidelines~\citep{ontonotes-guidelines}, which detail what should and should not be coreferent (e.g., how to deal with head-sharing noun phrases, premodifiers, and generic mentions). 
As a result, coreference datasets have traditionally been annotated by linguists (experts) already familiar with such concepts, and this reliance on experts makes the process expensive and time-consuming. Crowdsourced coreference data collection has the potential to be significantly cheaper and faster; however, teaching an exhaustive set of linguistic guidelines to non-expert crowd workers remains a formidable challenge. As a result, there has been a growing interest among researchers in curating a unified set of guidelines~\cite{universal-anaphora} suitable for annotators with various backgrounds. 

More recently, one of the proposed solution to crowdsource large coreference datasets~\cite{chamberlain-etal-2016-phrase} is to use games-with-a-purpose (GWAPs)~\cite{von-ahn-2006-gwap}, such as Phrase Detectives~\citep{poesio-etal-2013-PDoverview}. While GWAPs make it enjoyable for crowdworkers to learn complex guidelines and perform annotations using them~\cite{madge2019progression}, they also require significant effort to attract and maintain workers (e.g., Phrase Detectives Corpus 1.0 was collected over a span of six years~\cite{chamberlain-etal-2016-phrase, poesio2013phrase}), which motivates us to instead study coreference collection on more efficient payment-based platforms.
% and are often not open-sourced, making them inaccessible to other researchers interested in collecting new datasets.


% , including payment-based microtasks and games-with-a-purpose (GWAPs)~\cite{von-ahn-2006-gwap, poesio-etal-2013-PDoverview},

% Even so, annotators may have to frequently refer to these guidelines, which results in significant annotator efforts (e.g., OntoNotes and ARRAU as shown in Figure~\ref{figure:motivation_efforts}).  

% In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.
%Because of the differences in the existing guidelines, it is difficult to know which guidelines to use when collecting datasets in a new domain or language. Furthermore, these guidelines frequently include lengthy explanations of 

% More recently, efforts have been made to crowdsource coreference annotations by utilizing non-experts to annotate large corpora~\cite{chen-2018-preco, chamberlain-etal-2016-phrase}. For instance, applying the games-with-a-purpose (GWAPs) approach~\cite{von-ahn-2006-gwap, poesio2017crowdsourcing, kicikoglu2020aggregation, madge-etal-2019-making}, which emphasizes on fun as a motivator for annotators, researchers have successfully curated coreference datasets~\cite{poesio2019crowdsourced, poesio2013phrase, chamberlain-etal-2016-phrase}. While GWAPs make it interesting and enjoyable \mkcomment{I think GWAP is a fixed term? "game-with-a-pupose" not gameS; you probably can use "GWAPs" is you really want to but I wouldn't use "games-with..."}\agcomment{great point! though, I think gameS-with-a-purpose is equally valid, for instance Poessio uses this term in \url{https://dl.acm.org/doi/pdf/10.1145/2448116.2448119}; section 2.4 and von Ahn, one of the pioneers who popularized this concept, also uses "games"} for non-expert annotators to annotate documents, these methods necessitate significant researcher efforts to build such games and keep them visible for data collection~\cite{poesio-etal-2013-PDoverview} (e.g., Phrase Detectives in Figure~2). Furthermore, even this approach %\mkcomment{this approach; it's not a system, i think} 
% is challenged by complex, lengthy guidelines, as non-expert annotators in crowdsourcing setups \mkcomment{in any setup really, and it's kind of crowdsourcing anyway in nlp when you use non-experts, this is redundant} require concise, easy-to-understand guidelines to perform well and remain engaged.

% Another alternative for crowdsourcing linguistic annotations, including coreferences, is to use traditional payment-based methods (e.g., Amazon Mechanical Turk)~\cite{snow-2008-cheap, cybulska-vossen-2014-using, roit-etal-2020-controlled, bornstein-2020-corefi}, which are much easier to setup the task \mkcomment{more like easier to recruit the annotators "which offer an easier way to recruit the annotators while offering a dirverse..." - task setup depends on your annot interface, etc.; also not sure about this "diverse" claim; there are very specific ppl on AMT; it's pretty much NOT direverse} and offer a diverse workforce, reducing the researcher's efforts. However, these systems have the same difficulties in teaching complicated linguistic tasks to crowd annotators. \mkcomment{what "systems", I don't think this is the best word choice}


% \textcolor{orange}{One of the solutions proposed in the literature is to incorporate the \textit{learning by progression} approach~\cite{kicikoglu2020aggregation, madge2019progression, miller2019expertise}, where the annotators start with simpler tasks and gradually move towards more complex problems. However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks.}

% % One of the proposed solutions, also investigated for GWAPs, is to use the notion of learning by progression~\cite{poesio-etal-2013-phrase, kicikoglu2020aggregation, madge2019progression, miller2019expertise}, whereby the annotators start with simpler tasks, and then they are progressively taught more complex tasks. \mkcomment{One of the solutions proposed in the literature is to incorporate the \textit{learning by progression approach}, where the annotators start with simpler tasks and gradual move towards more complex problems.} 
% However, with these approaches, researchers must iteratively identify or use their judgment to decide the complexity of various tasks. \mkcomment{However, in order to efficiently employ the \textit{learning by progression} approach, researchers have to identify which cases are .... }

% \mkcomment{this transition is a bit rough; you mention the need to identiry these easy vs difficult cases and then switch to another topic without saying that this is what we do... should finish that thing first, then switch to minimal guidelines as a way to coref}
\agcomment{WIP from here onwards}
Specifically, our work investigates the feasibility of crowdsourcing coreference annotations by providing \emph{minimal} guidelines to workers on the Amazon Mechanical Turk Platform (AMT). In contrast to more elaborate guidelines used in previous work, 
our minimal guidelines 
%cover the broad concept 
teach workers only the broad
concept
of coreference, focusing on basic phenomena that have similar treatment across existing guidelines,
such as pronouns. 
%pronouns in ``\textcolor{red}{{[}John{]}} doesn’t like 
%\textcolor{teal}{{[}Fred{]}}, but \textcolor{red}{{[}he{]}} still invited \textcolor{teal}{{[}him{]}} to \textcolor{violet}{{[}the party{]}}").

% \agcomment{added minimal guidelines definition}
% \micomment{need to loosely define minimal guidelines. have a sentence explaining what is covered by the guidelines here (at a high level with some specific examples in parenthetical).} 
% \textcolor{orange}{By observing agreements/disagreements among annotators under \emph{minimal} training, we aim to understand which coreference concepts are easy to annotate for crowd annotators and which concepts would require more explanations in the guidelines. Such an understanding would not only help effective crowdsourcing but also help to prioritize difficult concepts while curating annotation guidelines.} 
% We train our annotators using these \emph{minimal} guidelines in order to investigate which coreference concepts are easier to annotate for crowd annotators and which concepts require more explanations in the guidelines.
% \mkcomment{We...XYZ (teach, present, or sth) ... in order to investigate....(give justification for minimal guidelines)??? <--- maybe like this you can add it?}
% For instance, annotations for pronoun resolution which are very useful for information extraction tasks can be obtained via minimal training, as observed in our experiments. If we can obtain good annotations via minimal training, that can speed up the process and make it easier for other researchers to collect new datasets, thereby reducing both annotator and researcher efforts.
To facilitate collection of these annotations, we develop a methodology---\texttt{ezCoref}---which includes an intuitive, open-sourced annotation tool
% \footnote{Our platform's code and collected data is available in supplementary material, and will be released publicly after review.}
supported by a short crowd-oriented interactive tutorial that includes annotation guidelines.\footnote{Our tutorial received overwhelmingly positive feedback. One annotator commented that it was ``\textit{absolutely beautiful, intuitive, and helpful. Legitimately the best one I've ever seen in my 2 years on AMT! Awesome job.}" (\autoref{table:tutorial_feedback} in Appendix)} We use \texttt{ezCoref} to re-annotate 240 passages from seven existing English coreference datasets. Our results show that high-quality annotations (measured by agreement with expert annotations) are obtained from non-experts with the minimal training facilitated by our annotation platform (>90$\%$ B3~\cite{bagga-1998-algorithms} agreement with experts).
% \micomment{can you say something about the quality of annotations from ezcoref, like we get high agreement with expert-annotated datasets}
\mkcomment{make the contributions clearer}
Our annotation study uniquely allows us to identify where the behavior of our crowd annotators differs from that of experts. For example, we qualitatively observe that crowd workers mark all generic pronouns as coreferent, while existing guidelines treat them as non-referring, and we observe similar deviations from expert guidelines for appositives and copulae. Furthermore, annotators find it easier to annotate pronouns than other coreference types, and they exhibit higher agreement when annotating familiar texts (e.g., childhood stories or fiction) compared to texts rich in cataphoric expressions or those requiring world knowledge.
% \micomment{the following insights should be reordered by interestingness/impactfulness and condensed}
% We obtain a high agreement among annotators for the fiction domain, suggesting that this domain is suitable to collect crowdsourced coreference annotations. Comparing various linguistic concepts, we find that annotators struggle with cataphoras, resulting in multiple mistake when annotating QuizBowl dataset~\cite{guha-etal-2015-removing}. Finally, comparing the expert guidelines with crowd annotations, we find that appositives and copulae have been annotated similarly by existing guidelines, but annotators naturally mark them differently and would require clarification in guidelines if expected otherwise. 
% \mkcomment{<---this sentence is not the smoothest, the point of it is too far in the forest; Finally, we find that non-expert annotators tend to annotate metions in appositives and copulae as coreferent, even though most of existing guidelines connected these with another, special link. ....though that is not true either right... they don't tend to do that, they are all over the place with copula but maybe better with appos, then it's the question of major vote}
We conclude with a qualitative analysis and highlight cases with genuine ambiguity, which we hope will inform future research into guideline construction and coreference platform development.





\begin{table*}[]
\centering 
\begin{adjustbox}{max width=\textwidth}
\tiny
\begin{tabular}{lccccclcccc}
\toprule
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Domains\\ $\#$(doc, ment, tok)\end{tabular}}} & \multirow{2}{*}{\textbf{Annotators}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Mention \\ Detection\end{tabular}}} & \multicolumn{2}{c}{\textbf{Mention Types}} & \multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{Coreference Links}} &  \\ \cline{5-6} \cline{8-11} \addlinespace[0.05cm]
 &  &  &  & \textbf{Singletons} & \textbf{\begin{tabular}[c]{@{}c@{}}Entity\\ Restrictions\end{tabular}} & \multicolumn{1}{c}{} & \textbf{Copulae} & \textbf{Appositives} & \textbf{Generics} & \textbf{Ambiguity} \\\midrule
 
\textbf{\begin{tabular}[c]{@{}l@{}}ARRAU\\ \cite{Uryupina2019}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (552, 99K, 350K)\end{tabular}  & Single Expert & Manual & Yes & None &  & Special Link & No Link & Yes & Explicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}Phrase Detectives (PD)\\ \cite{chamberlain-etal-2016-phrase}\end{tabular}}& \begin{tabular}[c]{@{}c@{}}Multiple\\ (542, 100K, 400K)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Crowd (gamified) +\\ 2 Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Semi\\ Automatic\end{tabular} & Yes & None &  & Special Link & Special Link & Yes & Implicit \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}GUM\\\cite{zeldes-2017-gum}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (25, 6K, 20K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}} Experts \\ (Linguistics Students)\end{tabular} & Manual & Yes & None &  & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Types)  \end{tabular} & \begin{tabular}[c]{@{}c@{}} Coref \\ (Sub-Type)  \end{tabular} & Yes & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}PreCo \\ \cite{chen-etal-2018-preco}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple***\\ (38K, 3.58M, 12.5M)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Non-Expert, \\ Non-Native \end{tabular}& Manual** & Yes & None &  & Coref & Coref & Yes & None \\ \addlinespace[0.1cm]

\textbf{\begin{tabular}[c]{@{}l@{}}OntoNotes\\ \cite{hovy-etal-2006-ontonotes}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Multiple\\ (1.6K, 94K, 950K)\end{tabular}  & Experts & Mixed & No & None &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}LitBank\\ \cite{bamman-etal-2020-annotated}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (100, 29K, 210K)\end{tabular}  & Experts & Manual & Yes & ACE (selected) &  & Special Link & Special Link & \begin{tabular}[c]{@{}c@{}}Only with\\ Pronominals\end{tabular} & None \\ \addlinespace[0.2cm]

\textbf{\begin{tabular}[c]{@{}l@{}}QuizBowl\\ \cite{guha-etal-2015-removing}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}Single\\ (400, 9.4K, 50K)\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Domain\\ Experts\end{tabular} & \begin{tabular}[c]{@{}c@{}}Manual\\ \& CRF*\end{tabular} & Yes & \begin{tabular}[c]{@{}c@{}}Characters,\\ Books,\\  Authors*\end{tabular} &  & Coref & Coref & If Applicable & None \\ \midrule
\textbf{\begin{tabular}[c]{@{}l@{}}ezCoref Pilot Dataset 
\\ (this work)\end{tabular}} & Multiple & Crowd (paid) & \begin{tabular}[c]{@{}c@{}}Fully\\ Automatic\end{tabular} & Yes & None &  & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & \begin{tabular}[c]{@{}c@{}}Annotator`s\\ Intuition\end{tabular} & Implicit \\ \bottomrule
\end{tabular}
\end{adjustbox}

\caption{Summary of seven datasets analyzed in this work,
which 
differ in domain, size, annotator qualifications, mention detection procedures, types of mentions, and types of links considered as coreferences between these mentions.\scriptsize{*Allows other types of mention only when this mention is an answer to a question.}\scriptsize{**We interpret manual identification based on illustrations presented in the original publication~\cite{chen-2018-preco}. }\scriptsize{***See Footnote \ref{fn:preco}.}} 
\vspace{-0.1in}
\label{table:motivation}
\end{table*}


\ignore{
\subsubsection{bullet points}
Existing datasets differ widely in their guidelines, so we don’t know which one to employ for new data collection. 

These guidelines are often complex with many arbitrary decisions.

Complex guidelines require experts but collecting annots with experts is expensive and time consuming (small num of experts working on large num of docs)

Crowdsourcing is a non-expert alternative which was recently done by using GWAP - but that is also time consuming (development, PR); the annotators may be motivated (yay, it’s a game!) but they need simplified guidelines

Alternative is traditional crowdsourcing but just as GWAP it requires simplified guidelines - teach ppl what you want (ppl can resolve coref naturally, but need to explain them the task)

One of the proposed solutions applied also in GWAP is to use the notion of learning by progression = iterating through concepts from easy to difficult cases. But for it to be done well with minimum time from workers => it requires researchers to identify what is hard and what is easy for a better / more efficient design

In this work, we try to address this question. We collect annotations under minimal training to identify what is hard and easy for annotators. Furthermore, deviations from existing expert guidelines can help inform avenues to revisit.

\subsection{text}
\agcomment{WIP}
Coreference resolution is the task of identifying and clustering together all textual expressions (\emph{mentions}) that refer to the same discourse entity in a given document. Impressive progress has been made in developing coreference systems~\citep{lee-etal-2017-end, moosavi-strube-2018-using,
joshi-etal-2020-spanbert}, enabled by expert-annotated~\citep{hovy-etal-2006-ontonotes, bamman-etal-2020-annotated, uryupina2020annotating} and crowdsourced  datasets~\citep{chamberlain-etal-2016-phrase, chen-2018-preco}. However, these datasets vary widely in their definition of coreference (expressed through annotation guidelines), resulting in inconsistent annotations both within and across languages and domains~\cite{universal-anaphora} (e.g., English news in Figure~\ref{figure:data_guidelines}). 

Coreference datasets vary in terms of their definition of coreference expressed via different guidelines, annotation formats and annotation platform used to collect the dataset. All these differences have impacts on the quality of collected data. These datasets not only differ in terms of what is coreference but also what is considered as a mention. Unfortunately, at the moment, there is only limited consensus on the various aspects of coreference phenomena that should be covered by any annotation guidelines~\cite{universal-anaphora}

In order to collect new datasets, researchers often train their annotators with the objective of maximizing inter annotator agreement. This process is arduous entailing many iterations to curate guidelines and consumes lot of researcher time, efforts and money. Furthermore, it has not been proven that data curated via extensively trained annotators can only give us the best performance on downstream tasks.

Another complimentary dimension in which these datasets differ is how these datasets were collected. Traditionally, these datasets such as OntoNotes were collected via expert annotators trained in lengthy guidelines. More recently, impressive progress has been made towards crowdsourcing coreference annotations. Both payment based approaches and games-with-a-purpose has been proposed and impressive success has been achieved e.g., as demonstrated by the success of Phrase Detectives. However, GWAPs are often not open-sourced and require maintaining constant visibility to collect annotations, thereby significantly increasing researcher efforts to collect new datasets. 

In this work, we investigate whether it is feasible to crowdsource coreference resolution under minimal guidelines? For instance, annotations for pronoun resolution which are very useful for information extraction tasks can be obtained via minimal training, as observed in our experiments. If we can obtain good annotations via minimal training, that can speed up the process and make it easier for other researchers to collect new datasets.
}



% \agcomment{broad area of the paper, recent progress, key limitation}

% \agcomment{give an example of key limitation}

% \agcomment{why and where, addressing this challenge is useful. why addressing this challenge isn't trivial.}

% \agcomment{some existing efforts to address this issue, and one line limitation.}

% \agcomment{what do we do in this paper to address this issue.}

% \agcomment{our contributions}
